Minimal Solvers for Full DoF Motion Estimation from Asynchronous Tracks

We address the problem of estimating both translational and angular velocity of a camera from asynchronous point tracks, a formulation relevant to rolling shutter and event cameras. Since the original problem is non-polynomial, we propose a polynomial approximation, classify the resulting minimal problems, and determine their algebraic degrees. Furthermore, we develop minimal solvers for several problems with low degrees and evaluate them on synthetic and real datasets. The code will be made publicly available.

==> plot/appx_test_3v_t.tex <==


\begin{axis}[%
width=0.35\columnwidth,
height=0.22\columnwidth,
at={(2.4in,0.389in)},
scale only axis,
xmin=0,
xmax=40,
xlabel style={font=\color{white!15!black}, yshift=0.03in},
xlabel={Ang. vel. ($^{\circ}$ / frame)},
title={Tran err ($^{\circ}$)},
ymin=0,
ymax=25,
ymode=normal,
yminorticks=true,
axis lines = left,
axis background/.style={fill=white},
title style={font=\bfseries, yshift=-0.1in},
%ylabel style={yshift=-0.15in},
%ylabel={Success rate ($\%$)},
%legend style={at={(1,1.3)}, anchor=south, legend cell align=left, align=left, draw=white!15!black, font=\normalsize,nodes={scale=1.0, transform shape}},
%legend columns=3
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addplot [color=magenta,line width=2pt, mark options={solid, red}]
  table[row sep=crcr]{%
0.0 0.0754183 \\
1.0 1.98385 \\
2.0 3.12389 \\
3.0 3.88439 \\
4.0 5.03135 \\
5.0 5.68055 \\
6.0 6.63679 \\
7.0 7.83389 \\
8.0 8.48627 \\
9.0 8.61269 \\
10.0 9.57822 \\
11.0 10.062 \\
12.0 10.6393 \\
13.0 10.4317 \\
14.0 11.1699 \\
15.0 12.2071 \\
16.0 12.9732 \\
17.0 12.9787 \\
18.0 13.0163 \\
19.0 13.6352 \\
20.0 14.7668 \\
21.0 15.1024 \\
22.0 15.502 \\
23.0 15.2776 \\
24.0 15.5847 \\
25.0 16.2476 \\
26.0 16.559 \\
27.0 16.1505 \\
28.0 17.1729 \\
29.0 17.7646 \\
30.0 17.8187 \\
31.0 17.9756 \\
32.0 18.4674 \\
33.0 18.9158 \\
34.0 19.6416 \\
35.0 19.8163 \\
36.0 19.5328 \\
37.0 20.2527 \\
38.0 19.9859 \\
39.0 20.5231 \\
40.0 20.5732 \\
41.0 21.3242 \\
42.0 21.6336 \\
43.0 21.4596 \\
44.0 21.3453 \\
45.0 21.6496 \\
};
\addlegendentry{5 point \cite{}}



\addplot [color=orange!50!black,line width=1.5pt, mark options={solid, orange}, mark options={solid, cyan}, mark=*, mark repeat=11, mark phase=3, mark size=1pt]
  table[row sep=crcr]{%
0.0 6.73024e-07 \\
1.0 0.308339 \\
2.0 0.670033 \\
3.0 0.805764 \\
4.0 1.29288 \\
5.0 1.90713 \\
6.0 2.2217 \\
7.0 3.0481 \\
8.0 3.45885 \\
9.0 4.17642 \\
10.0 4.36681 \\
11.0 4.88351 \\
12.0 5.19607 \\
13.0 6.13489 \\
14.0 6.67373 \\
15.0 7.04574 \\
16.0 7.219 \\
17.0 7.71307 \\
18.0 8.1094 \\
19.0 8.70963 \\
20.0 9.3394 \\
21.0 8.76994 \\
22.0 9.73637 \\
23.0 10.2944 \\
24.0 10.4252 \\
25.0 10.7281 \\
26.0 10.9359 \\
27.0 10.7741 \\
28.0 11.6372 \\
29.0 11.8993 \\
30.0 11.7218 \\
31.0 12.209 \\
32.0 12.7711 \\
33.0 13.0514 \\
34.0 13.3381 \\
35.0 13.4812 \\
36.0 13.7933 \\
37.0 13.7903 \\
38.0 13.8647 \\
39.0 14.2621 \\
40.0 14.2439 \\
41.0 14.9421 \\
42.0 14.6496 \\
43.0 14.9617 \\
44.0 15.5115 \\
45.0 15.5303 \\
  };
\addlegendentry{m=3,n=2,K=1+A1,HC}


\addplot [color=orange,line width=1.5pt, mark options={solid, orange}, mark options={solid, violet}, mark=*, mark repeat=11, mark phase=6, mark size=1pt]
  table[row sep=crcr]{%
0.0 9.92198 \\
1.0 0.763473 \\
2.0 0.959114 \\
3.0 1.4822 \\
4.0 1.96686 \\
5.0 1.9547 \\
6.0 2.92635 \\
7.0 3.14848 \\
8.0 3.57084 \\
9.0 3.81413 \\
10.0 4.5899 \\
11.0 5.15746 \\
12.0 5.84067 \\
13.0 5.95554 \\
14.0 6.54955 \\
15.0 6.67831 \\
16.0 7.55743 \\
17.0 8.39495 \\
18.0 8.35834 \\
19.0 9.00937 \\
20.0 8.97051 \\
21.0 9.26063 \\
22.0 10.053 \\
23.0 9.98885 \\
24.0 10.2087 \\
25.0 11.2047 \\
26.0 11.2355 \\
27.0 11.4633 \\
28.0 12.1095 \\
29.0 11.764 \\
30.0 12.3073 \\
31.0 12.6437 \\
32.0 12.9415 \\
33.0 13.0036 \\
34.0 13.6835 \\
35.0 13.79 \\
36.0 13.4384 \\
37.0 14.1472 \\
38.0 13.8217 \\
39.0 14.4 \\
40.0 14.5845 \\
41.0 14.639 \\
42.0 14.697 \\
43.0 15.316 \\
44.0 15.978 \\
45.0 15.3507 \\
  };
\addlegendentry{m=3,n=2,K=1+A1,GB}


\addplot [color=orange!50!black,line width=1.5pt, mark options={solid, orange}, mark options={solid, cyan}, mark=triangle*, mark repeat=11, mark phase=9, mark size=1pt]
  table[row sep=crcr]{%
0.0 0.0229996 \\
1.0 0.358826 \\
2.0 0.61406 \\
3.0 1.17945 \\
4.0 1.78447 \\
5.0 2.20818 \\
6.0 2.30511 \\
7.0 3.03662 \\
8.0 3.45505 \\
9.0 4.01147 \\
10.0 5.26442 \\
11.0 5.38838 \\
12.0 5.89216 \\
13.0 6.45238 \\
14.0 7.0448 \\
15.0 7.1057 \\
16.0 8.17871 \\
17.0 8.67918 \\
18.0 9.39202 \\
19.0 9.82557 \\
20.0 9.55785 \\
21.0 10.0752 \\
22.0 10.6224 \\
23.0 10.53 \\
24.0 10.5579 \\
25.0 10.9158 \\
26.0 11.4805 \\
27.0 11.7419 \\
28.0 12.3817 \\
29.0 12.6499 \\
30.0 12.3115 \\
31.0 12.75 \\
32.0 12.3809 \\
33.0 13.1026 \\
34.0 13.3324 \\
35.0 13.5476 \\
36.0 13.8003 \\
37.0 13.9522 \\
38.0 13.4882 \\
39.0 14.5631 \\
40.0 14.7426 \\
41.0 14.5366 \\
42.0 14.9755 \\
43.0 14.8562 \\
44.0 15.4939 \\
45.0 15.2144 \\
  };
\addlegendentry{m=3,n=2,K=1+A2,HC}


\addplot [color=orange,line width=1.5pt, mark options={solid, orange}, mark options={solid, violet}, mark=triangle*, mark repeat=11, mark size=1pt]
  table[row sep=crcr]{%
0.0 20.5955 \\
1.0 2.41958 \\
2.0 2.05163 \\
3.0 2.00091 \\
4.0 2.49812 \\
5.0 2.74443 \\
6.0 3.44209 \\
7.0 3.73452 \\
8.0 4.14921 \\
9.0 4.44827 \\
10.0 5.63559 \\
11.0 5.51104 \\
12.0 6.15591 \\
13.0 6.84359 \\
14.0 6.7716 \\
15.0 7.55186 \\
16.0 7.82891 \\
17.0 9.02209 \\
18.0 8.86604 \\
19.0 9.08825 \\
20.0 9.67878 \\
21.0 10.0209 \\
22.0 10.8324 \\
23.0 10.4961 \\
24.0 10.8355 \\
25.0 11.533 \\
26.0 11.5561 \\
27.0 12.064 \\
28.0 12.1282 \\
29.0 12.2409 \\
30.0 12.7297 \\
31.0 12.602 \\
32.0 12.9885 \\
33.0 12.9793 \\
34.0 13.0172 \\
35.0 13.1323 \\
36.0 13.4692 \\
37.0 14.1155 \\
38.0 14.3594 \\
39.0 14.4699 \\
40.0 14.1158 \\
41.0 13.9531 \\
42.0 14.4224 \\
43.0 14.6915 \\
44.0 14.9325 \\
45.0 14.5862 \\
  };
\addlegendentry{m=3,n=2,K=1+A2,GB}




\addplot [color=orange!50!black,line width=1.5pt, mark options={solid, orange}, mark options={solid, black}, mark=*, mark repeat=11, mark phase = 5, mark size=1pt]
  table[row sep=crcr]{%
0.0 7.68351e-07 \\
1.0 0.0168213 \\
2.0 0.0568557 \\
3.0 0.0502121 \\
4.0 0.297186 \\
5.0 0.224735 \\
6.0 0.443325 \\
7.0 0.758757 \\
8.0 0.71217 \\
9.0 0.826171 \\
10.0 1.07566 \\
11.0 1.30774 \\
12.0 1.73267 \\
13.0 1.87626 \\
14.0 2.06965 \\
15.0 2.23907 \\
16.0 2.23527 \\
17.0 2.68746 \\
18.0 2.86435 \\
19.0 2.95856 \\
20.0 3.58984 \\
21.0 3.74054 \\
22.0 3.70891 \\
23.0 4.07004 \\
24.0 4.54428 \\
25.0 4.45505 \\
26.0 4.6022 \\
27.0 4.93592 \\
28.0 5.11944 \\
29.0 5.09617 \\
30.0 5.57685 \\
31.0 5.87944 \\
32.0 5.6748 \\
33.0 5.83087 \\
34.0 5.81499 \\
35.0 6.55494 \\
36.0 6.66037 \\
37.0 6.64477 \\
38.0 6.75254 \\
39.0 6.69845 \\
40.0 7.12801 \\
41.0 7.39201 \\
42.0 7.14401 \\
43.0 7.44146 \\
44.0 7.59466 \\
45.0 7.95833 \\
  };
\addlegendentry{m=3,n=2,K=2+A1,HC}

\addplot [color=orange!50!black,line width=1.5pt, mark options={solid, orange}, mark options={solid, black}, mark=triangle*, mark repeat=11, mark size=1pt]
  table[row sep=crcr]{%
0.0 6.40171e-07 \\
1.0 0.0179258 \\
2.0 0.0226558 \\
3.0 0.106925 \\
4.0 0.178818 \\
5.0 0.212656 \\
6.0 0.391668 \\
7.0 0.424364 \\
8.0 0.686211 \\
9.0 0.69008 \\
10.0 1.1878 \\
11.0 1.35059 \\
12.0 1.54157 \\
13.0 1.65711 \\
14.0 1.93582 \\
15.0 2.10299 \\
16.0 2.32787 \\
17.0 2.27267 \\
18.0 2.99512 \\
19.0 3.3052 \\
20.0 3.18998 \\
21.0 3.54452 \\
22.0 3.98603 \\
23.0 4.07344 \\
24.0 4.35293 \\
25.0 4.34505 \\
26.0 4.52876 \\
27.0 4.70502 \\
28.0 4.79187 \\
29.0 5.30233 \\
30.0 5.338 \\
31.0 6.00075 \\
32.0 5.59689 \\
33.0 5.62653 \\
34.0 6.08409 \\
35.0 6.25285 \\
36.0 6.41479 \\
37.0 6.58908 \\
38.0 6.95646 \\
39.0 7.25313 \\
40.0 7.07673 \\
41.0 7.11935 \\
42.0 7.40656 \\
43.0 7.76167 \\
44.0 7.5334 \\
45.0 8.27428 \\
  };
\addlegendentry{m=3,n=2,K=2+A2,GB}






\legend{}

\end{axis}

==> plot/appx_test_4v_t.tex <==


\begin{axis}[%
width=0.35\columnwidth,
height=0.22\columnwidth,
at={(2.4in,0.389in)},
scale only axis,
xmin=0,
xmax=40,
xlabel style={font=\color{white!15!black}, yshift=0.03in},
xlabel={Ang. vel. ($^{\circ}$ / frame)},
title={Tran err ($^{\circ}$)},
ymin=0,
ymax=30,
ymode=normal,
yminorticks=true,
axis lines = left,
axis background/.style={fill=white},
title style={font=\bfseries, yshift=-0.1in},
%ylabel style={yshift=-0.15in},
%ylabel={Success rate ($\%$)},
%legend style={at={(1,1.3)}, anchor=south, legend cell align=left, align=left, draw=white!15!black, font=\normalsize,nodes={scale=1.0, transform shape}},
%legend columns=3
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\addplot [color=magenta,line width=2pt, mark options={solid, red}]
  table[row sep=crcr]{%
0.0 0.0754183 \\
1.0 1.98385 \\
2.0 3.12389 \\
3.0 3.88439 \\
4.0 5.03135 \\
5.0 5.68055 \\
6.0 6.63679 \\
7.0 7.83389 \\
8.0 8.48627 \\
9.0 8.61269 \\
10.0 9.57822 \\
11.0 10.062 \\
12.0 10.6393 \\
13.0 10.4317 \\
14.0 11.1699 \\
15.0 12.2071 \\
16.0 12.9732 \\
17.0 12.9787 \\
18.0 13.0163 \\
19.0 13.6352 \\
20.0 14.7668 \\
21.0 15.1024 \\
22.0 15.502 \\
23.0 15.2776 \\
24.0 15.5847 \\
25.0 16.2476 \\
26.0 16.559 \\
27.0 16.1505 \\
28.0 17.1729 \\
29.0 17.7646 \\
30.0 17.8187 \\
31.0 17.9756 \\
32.0 18.4674 \\
33.0 18.9158 \\
34.0 19.6416 \\
35.0 19.8163 \\
36.0 19.5328 \\
37.0 20.2527 \\
38.0 19.9859 \\
39.0 20.5231 \\
40.0 20.5732 \\
41.0 21.3242 \\
42.0 21.6336 \\
43.0 21.4596 \\
44.0 21.3453 \\
45.0 21.6496 \\
};
\addlegendentry{5 point \cite{}}


\addplot [color=cyan!40!black,line width=1.5pt, mark options={solid, orange}, mark options={solid, violet}, mark=*, mark repeat=11, mark size=1pt]
  table[row sep=crcr]{%
0.0 180.0 \\
1.0 11.4429 \\
2.0 11.2827 \\
3.0 11.9388 \\
4.0 12.754 \\
5.0 13.0252 \\
6.0 14.3017 \\
7.0 14.3095 \\
8.0 14.0038 \\
9.0 15.7665 \\
10.0 17.4475 \\
11.0 17.3807 \\
12.0 18.491 \\
13.0 20.6544 \\
14.0 20.7491 \\
15.0 21.3851 \\
16.0 20.4043 \\
17.0 22.3974 \\
18.0 22.8896 \\
19.0 23.359 \\
20.0 23.7829 \\
21.0 23.567 \\
22.0 24.842 \\
23.0 24.8747 \\
24.0 25.827 \\
25.0 25.4132 \\
26.0 26.0427 \\
27.0 26.6732 \\
28.0 26.3007 \\
29.0 27.6503 \\
30.0 26.6448 \\
31.0 27.9731 \\
32.0 27.8487 \\
33.0 28.3551 \\
34.0 28.8544 \\
35.0 28.4544 \\
36.0 27.0001 \\
37.0 27.964 \\
38.0 27.3436 \\
39.0 29.6296 \\
40.0 29.2162 \\
41.0 28.8216 \\
42.0 29.7358 \\
43.0 29.9795 \\
44.0 29.4795 \\
45.0 29.0481 \\
  };
\addlegendentry{m=4,n=1,K=1+A1,HC}


\addplot [color=cyan,line width=1.5pt, mark options={solid, orange}, mark options={solid, violet!50!magenta}, mark=*, mark repeat=11, mark phase=3, mark size=1pt]
  table[row sep=crcr]{%
0.0 19.0068 \\
1.0 7.00479 \\
2.0 7.21054 \\
3.0 7.90683 \\
4.0 8.03865 \\
5.0 9.06642 \\
6.0 9.348 \\
7.0 10.9141 \\
8.0 11.0374 \\
9.0 12.1011 \\
10.0 12.1033 \\
11.0 13.4475 \\
12.0 13.7199 \\
13.0 14.2028 \\
14.0 15.1784 \\
15.0 15.5274 \\
16.0 16.2233 \\
17.0 15.7892 \\
18.0 16.6 \\
19.0 17.3378 \\
20.0 17.77 \\
21.0 18.677 \\
22.0 19.013 \\
23.0 19.2047 \\
24.0 19.8589 \\
25.0 20.8363 \\
26.0 19.7984 \\
27.0 19.7303 \\
28.0 20.4409 \\
29.0 21.2452 \\
30.0 20.2227 \\
31.0 20.7072 \\
32.0 21.7682 \\
33.0 21.2794 \\
34.0 21.9569 \\
35.0 21.2019 \\
36.0 21.6311 \\
37.0 20.2657 \\
38.0 21.5436 \\
39.0 22.5662 \\
40.0 23.5211 \\
41.0 21.7663 \\
42.0 21.716 \\
43.0 21.7414 \\
44.0 22.8252 \\
45.0 21.931 \\
};
\addlegendentry{m=4,n=1,K=1+A1,GB}


\addplot [color=cyan!40!black,line width=1.5pt, mark options={solid, orange}, mark options={solid, violet}, mark=triangle*, mark repeat=11, mark phase=6, mark size=1pt]
  table[row sep=crcr]{%
0.0 27.3654 \\
1.0 1.04182 \\
2.0 1.32853 \\
3.0 1.46703 \\
4.0 1.85446 \\
5.0 2.50757 \\
6.0 3.09307 \\
7.0 3.97205 \\
8.0 4.75217 \\
9.0 5.45326 \\
10.0 6.10813 \\
11.0 7.78926 \\
12.0 8.44604 \\
13.0 9.5339 \\
14.0 10.2141 \\
15.0 10.92 \\
16.0 12.1673 \\
17.0 13.6392 \\
18.0 14.9298 \\
19.0 14.457 \\
20.0 15.9569 \\
21.0 16.1626 \\
22.0 17.0764 \\
23.0 17.1202 \\
24.0 17.6735 \\
25.0 18.2432 \\
26.0 18.3032 \\
27.0 18.8514 \\
28.0 18.5949 \\
29.0 19.3837 \\
30.0 19.0031 \\
31.0 18.7498 \\
32.0 19.8522 \\
33.0 20.2916 \\
34.0 20.9439 \\
35.0 20.6697 \\
36.0 20.3473 \\
37.0 19.8139 \\
38.0 20.9304 \\
39.0 19.6313 \\
40.0 20.0022 \\
41.0 19.6803 \\
42.0 20.9807 \\
43.0 20.4856 \\
44.0 20.5355 \\
45.0 21.2269 \\
  };
\addlegendentry{m=4,n=1,K=1+A2,HC}


\addplot [color=cyan,line width=1.5pt, mark options={solid, orange}, mark options={solid, violet!50!magenta}, mark=triangle*, mark repeat=11, mark phase=9, mark size=1pt]
  table[row sep=crcr]{%
0.0 26.6582 \\
1.0 1.40692 \\
2.0 1.20974 \\
3.0 1.4216 \\
4.0 1.72582 \\
5.0 2.2596 \\
6.0 2.92778 \\
7.0 3.96514 \\
8.0 5.7015 \\
9.0 5.60633 \\
10.0 6.96678 \\
11.0 7.17045 \\
12.0 8.99638 \\
13.0 9.93288 \\
14.0 10.9054 \\
15.0 12.5317 \\
16.0 12.5686 \\
17.0 12.822 \\
18.0 12.8978 \\
19.0 15.3371 \\
20.0 15.1903 \\
21.0 15.7151 \\
22.0 17.0534 \\
23.0 16.6295 \\
24.0 17.281 \\
25.0 18.0712 \\
26.0 17.4505 \\
27.0 19.0692 \\
28.0 18.5322 \\
29.0 19.5359 \\
30.0 19.517 \\
31.0 19.3567 \\
32.0 19.4592 \\
33.0 19.7305 \\
34.0 20.3023 \\
35.0 19.5301 \\
36.0 20.2507 \\
37.0 20.5769 \\
38.0 20.4326 \\
39.0 20.9975 \\
40.0 20.2768 \\
41.0 20.1786 \\
42.0 21.3342 \\
43.0 20.4807 \\
44.0 20.6708 \\
45.0 19.6969 \\
  };
\addlegendentry{m=4,n=1,K=1+A2,GB}




\addplot [color=cyan!40!black,line width=1.5pt, mark options={solid, orange}, mark options={solid, black}, mark=*, mark repeat=11, mark size=1pt]
  table[row sep=crcr]{%
0.0 9.58585 \\
1.0 0.30203 \\
2.0 0.776408 \\
3.0 1.19241 \\
4.0 1.78699 \\
5.0 2.35885 \\
6.0 3.36944 \\
7.0 3.37037 \\
8.0 3.99447 \\
9.0 4.48064 \\
10.0 4.82859 \\
11.0 5.59257 \\
12.0 6.37422 \\
13.0 6.66237 \\
14.0 7.03725 \\
15.0 7.0418 \\
16.0 7.97909 \\
17.0 8.71374 \\
18.0 8.26298 \\
19.0 8.44528 \\
20.0 8.8477 \\
21.0 9.26436 \\
22.0 9.38549 \\
23.0 9.77423 \\
24.0 9.79597 \\
25.0 10.4528 \\
26.0 10.5916 \\
27.0 11.1467 \\
28.0 11.1317 \\
29.0 11.3534 \\
30.0 11.5279 \\
31.0 11.587 \\
32.0 11.2696 \\
33.0 12.4354 \\
34.0 12.46 \\
35.0 12.3039 \\
36.0 12.5005 \\
37.0 12.8964 \\
38.0 13.0773 \\
39.0 13.0208 \\
40.0 13.9576 \\
41.0 13.3928 \\
42.0 14.3006 \\
43.0 13.3589 \\
44.0 14.158 \\
45.0 13.9986 \\
  };
\addlegendentry{m=4,n=1,K=2+A1,HC}

\addplot [color=cyan!40!black,line width=1.5pt, mark options={solid, orange}, mark options={solid, black}, mark=triangle*, mark repeat=11, mark phase=7, mark size=1pt]
  table[row sep=crcr]{%
0.0 27.4541 \\
1.0 0.976246 \\
2.0 1.34519 \\
3.0 1.59163 \\
4.0 2.06703 \\
5.0 2.29512 \\
6.0 2.82371 \\
7.0 3.89588 \\
8.0 4.74447 \\
9.0 5.65407 \\
10.0 7.01303 \\
11.0 8.01776 \\
12.0 9.10936 \\
13.0 9.63089 \\
14.0 10.4935 \\
15.0 13.0081 \\
16.0 12.6579 \\
17.0 13.4757 \\
18.0 13.2624 \\
19.0 14.5582 \\
20.0 16.0724 \\
21.0 16.4384 \\
22.0 16.1032 \\
23.0 16.1497 \\
24.0 16.7934 \\
25.0 17.405 \\
26.0 18.5366 \\
27.0 19.5729 \\
28.0 18.8627 \\
29.0 20.0547 \\
30.0 19.9768 \\
31.0 18.9201 \\
32.0 20.2336 \\
33.0 20.326 \\
34.0 20.3763 \\
35.0 19.9868 \\
36.0 20.1661 \\
37.0 20.4236 \\
38.0 20.9167 \\
39.0 20.2427 \\
40.0 19.7455 \\
41.0 20.6914 \\
42.0 20.7698 \\
43.0 20.6618 \\
44.0 20.3707 \\
45.0 19.6996 \\
  };
\addlegendentry{m=4,n=1,K=2+A2,HC}

\addplot [color=cyan,line width=1.5pt, mark options={solid, orange}, mark options={solid, yellow}, mark=triangle*, mark repeat=11, mark phase=3, mark size=1pt]
  table[row sep=crcr]{%
0.0 27.6892 \\
1.0 1.38113 \\
2.0 1.20477 \\
3.0 1.3333 \\
4.0 1.953 \\
5.0 2.62311 \\
6.0 3.15187 \\
7.0 3.74491 \\
8.0 4.76633 \\
9.0 5.58684 \\
10.0 6.92482 \\
11.0 7.28509 \\
12.0 9.31915 \\
13.0 10.0672 \\
14.0 10.6791 \\
15.0 12.0137 \\
16.0 12.6007 \\
17.0 12.9421 \\
18.0 13.3845 \\
19.0 14.1144 \\
20.0 15.3669 \\
21.0 15.4559 \\
22.0 17.0347 \\
23.0 16.7076 \\
24.0 17.8154 \\
25.0 17.6203 \\
26.0 18.0998 \\
27.0 18.3603 \\
28.0 18.9533 \\
29.0 19.0331 \\
30.0 19.672 \\
31.0 19.6463 \\
32.0 20.9747 \\
33.0 20.1378 \\
34.0 19.2839 \\
35.0 20.232 \\
36.0 20.3105 \\
37.0 20.1418 \\
38.0 19.877 \\
39.0 20.3372 \\
40.0 20.8142 \\
41.0 20.498 \\
42.0 19.9027 \\
43.0 19.9785 \\
44.0 19.7768 \\
45.0 20.4352 \\
  };
\addlegendentry{m=4,n=1,K=2+A2,GB}

\legend{}

\end{axis}

==> plot/appx_test_event_3v_t.tex <==


\begin{axis}[%
width=0.35\columnwidth,
height=0.22\columnwidth,
at={(2.4in,0.389in)},
scale only axis,
xmin=0,
xmax=40,
xlabel style={font=\color{white!15!black}, yshift=0.03in},
xlabel={Ang. vel. ($^{\circ}$ / frame)},
title={Tran err ($^{\circ}$)},
ymin=0,
ymax=30,
ymode=normal,
yminorticks=true,
axis lines = left,
axis background/.style={fill=white},
title style={font=\bfseries, yshift=-0.1in},
%ylabel style={yshift=-0.15in},
%ylabel={Success rate ($\%$)},
%legend style={at={(1,1.3)}, anchor=south, legend cell align=left, align=left, draw=white!15!black, font=\normalsize,nodes={scale=1.0, transform shape}},
%legend columns=3
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addplot [color=magenta,line width=2pt, mark options={solid, red}]
  table[row sep=crcr]{%
0.0 0.0295238 \\
1.0 5.40393 \\
2.0 7.78743 \\
3.0 9.61086 \\
4.0 10.8405 \\
5.0 12.0025 \\
6.0 13.2969 \\
7.0 14.0259 \\
8.0 15.4061 \\
9.0 15.7173 \\
10.0 16.4864 \\
11.0 17.3546 \\
12.0 17.6014 \\
13.0 17.5699 \\
14.0 18.3201 \\
15.0 18.2636 \\
16.0 19.085 \\
17.0 20.1345 \\
18.0 19.9439 \\
19.0 20.5993 \\
20.0 20.2852 \\
21.0 20.1148 \\
22.0 21.1968 \\
23.0 21.275 \\
24.0 21.9623 \\
25.0 22.0935 \\
26.0 22.4699 \\
27.0 22.5022 \\
28.0 23.2747 \\
29.0 22.4835 \\
30.0 22.4285 \\
31.0 23.4644 \\
32.0 23.4076 \\
33.0 23.2753 \\
34.0 23.5566 \\
35.0 23.0511 \\
36.0 24.4182 \\
37.0 24.5082 \\
38.0 24.4673 \\
39.0 24.2551 \\
40.0 24.5867 \\
41.0 24.9884 \\
42.0 25.2501 \\
43.0 24.8187 \\
44.0 25.2996 \\
45.0 25.9283 \\
};
\addlegendentry{5 point \cite{}}



\addplot [color=orange!50!black,line width=1.5pt, mark options={solid, orange}, mark options={solid, cyan}, mark=*, mark repeat=11, mark phase=3, mark size=1pt]
  table[row sep=crcr]{%
0.0 0.0205394 \\
1.0 0.411362 \\
2.0 0.764316 \\
3.0 1.40189 \\
4.0 1.77715 \\
5.0 2.88994 \\
6.0 3.79444 \\
7.0 4.4359 \\
8.0 5.21948 \\
9.0 6.08897 \\
10.0 7.20891 \\
11.0 8.3381 \\
12.0 8.60246 \\
13.0 9.84853 \\
14.0 10.5282 \\
15.0 10.8676 \\
16.0 11.5479 \\
17.0 12.0121 \\
18.0 12.9451 \\
19.0 12.72 \\
20.0 13.9065 \\
21.0 14.4363 \\
22.0 14.1979 \\
23.0 15.1683 \\
24.0 15.0107 \\
25.0 15.1672 \\
26.0 15.8433 \\
27.0 16.1508 \\
28.0 16.3458 \\
29.0 16.0016 \\
30.0 16.774 \\
31.0 16.9203 \\
32.0 17.2533 \\
33.0 17.4297 \\
34.0 17.9931 \\
35.0 17.0057 \\
36.0 17.1376 \\
37.0 18.0011 \\
38.0 17.9122 \\
39.0 18.1139 \\
40.0 17.6169 \\
41.0 18.247 \\
42.0 17.8356 \\
43.0 17.3095 \\
44.0 18.0131 \\
45.0 17.7787 \\
  };
\addlegendentry{m=3,n=2,K=1+A1,HC}


\addplot [color=orange,line width=1.5pt, mark options={solid, orange}, mark options={solid, violet}, mark=*, mark repeat=11, mark phase=6, mark size=1pt]
  table[row sep=crcr]{%
0.0 9.52978 \\
1.0 0.905071 \\
2.0 1.3093 \\
3.0 1.80302 \\
4.0 2.21501 \\
5.0 3.12415 \\
6.0 4.06433 \\
7.0 4.41583 \\
8.0 5.77906 \\
9.0 6.75345 \\
10.0 7.52406 \\
11.0 8.34475 \\
12.0 8.33545 \\
13.0 9.41743 \\
14.0 10.5011 \\
15.0 11.1549 \\
16.0 11.4771 \\
17.0 12.303 \\
18.0 12.2286 \\
19.0 12.7197 \\
20.0 13.1001 \\
21.0 13.9467 \\
22.0 15.1466 \\
23.0 14.6345 \\
24.0 15.0444 \\
25.0 15.1686 \\
26.0 15.3397 \\
27.0 15.8999 \\
28.0 17.3913 \\
29.0 15.9424 \\
30.0 16.6816 \\
31.0 16.7881 \\
32.0 16.5068 \\
33.0 16.9198 \\
34.0 17.1614 \\
35.0 17.6848 \\
36.0 17.1712 \\
37.0 17.1996 \\
38.0 18.3916 \\
39.0 18.0397 \\
40.0 18.1027 \\
41.0 18.2727 \\
42.0 17.8032 \\
43.0 17.814 \\
44.0 18.7696 \\
45.0 18.7234 \\
  };
\addlegendentry{m=3,n=2,K=1+A1,GB}


\addplot [color=orange!50!black,line width=1.5pt, mark options={solid, orange}, mark options={solid, cyan}, mark=triangle*, mark repeat=11, mark phase=9, mark size=1pt]
  table[row sep=crcr]{%
0.0 0.0410393 \\
1.0 0.578568 \\
2.0 0.982817 \\
3.0 1.45343 \\
4.0 2.17933 \\
5.0 3.03706 \\
6.0 3.85097 \\
7.0 4.60927 \\
8.0 5.84075 \\
9.0 6.26584 \\
10.0 7.45796 \\
11.0 8.07269 \\
12.0 9.42402 \\
13.0 9.77234 \\
14.0 10.7905 \\
15.0 11.097 \\
16.0 11.757 \\
17.0 12.6454 \\
18.0 13.4627 \\
19.0 13.1009 \\
20.0 14.0766 \\
21.0 14.5544 \\
22.0 14.8706 \\
23.0 16.2186 \\
24.0 15.3749 \\
25.0 15.3192 \\
26.0 16.2008 \\
27.0 16.5056 \\
28.0 16.8694 \\
29.0 16.7847 \\
30.0 17.4145 \\
31.0 16.5187 \\
32.0 17.3902 \\
33.0 17.0137 \\
34.0 16.9543 \\
35.0 17.0487 \\
36.0 17.3228 \\
37.0 18.3345 \\
38.0 17.7901 \\
39.0 17.7333 \\
40.0 17.9421 \\
41.0 18.2364 \\
42.0 17.9216 \\
43.0 17.7317 \\
44.0 18.1013 \\
45.0 18.0466 \\
  };
\addlegendentry{m=3,n=2,K=1+A2,HC}


\addplot [color=orange,line width=1.5pt, mark options={solid, orange}, mark options={solid, violet}, mark=triangle*, mark repeat=11, mark size=1pt]
  table[row sep=crcr]{%
0.0 21.1766 \\
1.0 1.28761 \\
2.0 1.68076 \\
3.0 1.83133 \\
4.0 2.40213 \\
5.0 3.03747 \\
6.0 4.24722 \\
7.0 4.84674 \\
8.0 5.43797 \\
9.0 6.38401 \\
10.0 8.00457 \\
11.0 9.20992 \\
12.0 9.10259 \\
13.0 10.1543 \\
14.0 10.6611 \\
15.0 11.3429 \\
16.0 12.5165 \\
17.0 13.0789 \\
18.0 13.2318 \\
19.0 13.5879 \\
20.0 14.076 \\
21.0 14.9806 \\
22.0 15.5973 \\
23.0 14.8116 \\
24.0 15.7011 \\
25.0 16.1777 \\
26.0 16.2064 \\
27.0 15.8651 \\
28.0 16.4366 \\
29.0 16.8244 \\
30.0 16.755 \\
31.0 17.1126 \\
32.0 17.1216 \\
33.0 16.9271 \\
34.0 17.3908 \\
35.0 17.6734 \\
36.0 17.2888 \\
37.0 17.723 \\
38.0 17.4984 \\
39.0 17.5309 \\
40.0 18.4489 \\
41.0 17.5137 \\
42.0 18.3559 \\
43.0 17.5107 \\
44.0 17.8088 \\
45.0 17.6289 \\
  };
\addlegendentry{m=3,n=2,K=1+A2,GB}




\addplot [color=orange!50!black,line width=1.5pt, mark options={solid, orange}, mark options={solid, black}, mark=*, mark repeat=11, mark phase = 5, mark size=1pt]
  table[row sep=crcr]{%
0.0 7.68351e-07 \\
  };
\addlegendentry{m=3,n=2,K=2+A1,HC}

\addplot [color=orange!50!black,line width=1.5pt, mark options={solid, orange}, mark options={solid, black}, mark=triangle*, mark repeat=11, mark size=1pt]
  table[row sep=crcr]{%
0.0 2.73023e-06 \\
1.0 0.0232339 \\
2.0 0.133281 \\
3.0 0.180174 \\
4.0 0.445429 \\
5.0 0.779802 \\
6.0 0.964762 \\
7.0 1.38416 \\
8.0 1.60972 \\
9.0 1.84125 \\
10.0 2.63089 \\
11.0 2.71384 \\
12.0 3.01009 \\
13.0 3.49445 \\
14.0 3.97579 \\
15.0 4.68122 \\
16.0 4.44518 \\
17.0 4.83879 \\
18.0 5.20396 \\
19.0 5.69007 \\
20.0 5.65334 \\
21.0 5.81308 \\
22.0 6.02594 \\
23.0 6.45628 \\
24.0 7.17601 \\
25.0 6.80613 \\
26.0 7.5479 \\
27.0 7.93679 \\
28.0 7.78479 \\
29.0 8.40484 \\
30.0 8.13693 \\
31.0 8.30537 \\
32.0 8.64755 \\
33.0 8.59411 \\
34.0 9.00186 \\
35.0 9.55989 \\
36.0 9.58495 \\
37.0 9.68602 \\
38.0 9.89967 \\
39.0 10.1876 \\
40.0 10.1 \\
41.0 10.1999 \\
42.0 10.5467 \\
43.0 10.6931 \\
44.0 10.6867 \\
45.0 10.9966 \\
  };
\addlegendentry{m=3,n=2,K=2+A2,GB}






\legend{}

\end{axis}

==> plot/appx_test_event_4v_t.tex <==


\begin{axis}[%
width=0.35\columnwidth,
height=0.22\columnwidth,
at={(2.4in,0.389in)},
scale only axis,
xmin=0,
xmax=40,
xlabel style={font=\color{white!15!black}, yshift=0.03in},
xlabel={Ang. vel. ($^{\circ}$ / frame)},
title={Tran err ($^{\circ}$)},
ymin=0,
ymax=30,
ymode=normal,
yminorticks=true,
axis lines = left,
axis background/.style={fill=white},
title style={font=\bfseries, yshift=-0.1in},
%ylabel style={yshift=-0.15in},
%ylabel={Success rate ($\%$)},
%legend style={at={(1,1.3)}, anchor=south, legend cell align=left, align=left, draw=white!15!black, font=\normalsize,nodes={scale=1.0, transform shape}},
%legend columns=3
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\addplot [color=magenta,line width=2pt, mark options={solid, red}]
  table[row sep=crcr]{%
0.0 0.0295238 \\
1.0 5.40393 \\
2.0 7.78743 \\
3.0 9.61086 \\
4.0 10.8405 \\
5.0 12.0025 \\
6.0 13.2969 \\
7.0 14.0259 \\
8.0 15.4061 \\
9.0 15.7173 \\
10.0 16.4864 \\
11.0 17.3546 \\
12.0 17.6014 \\
13.0 17.5699 \\
14.0 18.3201 \\
15.0 18.2636 \\
16.0 19.085 \\
17.0 20.1345 \\
18.0 19.9439 \\
19.0 20.5993 \\
20.0 20.2852 \\
21.0 20.1148 \\
22.0 21.1968 \\
23.0 21.275 \\
24.0 21.9623 \\
25.0 22.0935 \\
26.0 22.4699 \\
27.0 22.5022 \\
28.0 23.2747 \\
29.0 22.4835 \\
30.0 22.4285 \\
31.0 23.4644 \\
32.0 23.4076 \\
33.0 23.2753 \\
34.0 23.5566 \\
35.0 23.0511 \\
36.0 24.4182 \\
37.0 24.5082 \\
38.0 24.4673 \\
39.0 24.2551 \\
40.0 24.5867 \\
41.0 24.9884 \\
42.0 25.2501 \\
43.0 24.8187 \\
44.0 25.2996 \\
45.0 25.9283 \\
};
\addlegendentry{5 point \cite{}}


\addplot [color=cyan!40!black,line width=1.5pt, mark options={solid, orange}, mark options={solid, violet}, mark=*, mark repeat=11, mark size=1pt]
  table[row sep=crcr]{%
0.0 180.0 \\
1.0 11.5344 \\
2.0 11.4599 \\
3.0 11.3528 \\
4.0 11.5655 \\
5.0 12.6848 \\
6.0 12.854 \\
7.0 13.9595 \\
8.0 13.1175 \\
9.0 14.5418 \\
10.0 14.2047 \\
11.0 15.6198 \\
12.0 15.6068 \\
13.0 16.6443 \\
14.0 17.3162 \\
15.0 17.8821 \\
16.0 18.0874 \\
17.0 19.1382 \\
18.0 19.5709 \\
19.0 19.3989 \\
20.0 20.1019 \\
21.0 20.7047 \\
22.0 20.8209 \\
23.0 20.9402 \\
24.0 20.3068 \\
25.0 21.0258 \\
26.0 22.5173 \\
27.0 22.8889 \\
28.0 23.3887 \\
29.0 22.6715 \\
30.0 23.5748 \\
31.0 24.632 \\
32.0 23.7302 \\
33.0 24.1963 \\
34.0 24.4358 \\
35.0 25.2245 \\
36.0 25.0431 \\
37.0 24.6398 \\
38.0 25.8154 \\
39.0 25.1999 \\
40.0 25.6378 \\
41.0 26.8636 \\
42.0 25.4582 \\
43.0 26.7382 \\
44.0 26.033 \\
45.0 26.0466 \\
  };
\addlegendentry{m=4,n=1,K=1+A1,HC}


\addplot [color=cyan,line width=1.5pt, mark options={solid, orange}, mark options={solid, violet!50!magenta}, mark=*, mark repeat=11, mark phase=3, mark size=1pt]
  table[row sep=crcr]{%
0.0 19.9041 \\
1.0 7.30644 \\
2.0 6.64288 \\
3.0 6.70171 \\
4.0 6.77908 \\
5.0 7.49006 \\
6.0 8.67532 \\
7.0 8.36965 \\
8.0 9.42795 \\
9.0 10.0792 \\
10.0 10.3866 \\
11.0 10.8104 \\
12.0 11.3499 \\
13.0 12.3042 \\
14.0 12.3212 \\
15.0 12.6327 \\
16.0 12.8322 \\
17.0 13.6626 \\
18.0 14.2326 \\
19.0 14.831 \\
20.0 15.5109 \\
21.0 14.8481 \\
22.0 15.3322 \\
23.0 16.6761 \\
24.0 16.1668 \\
25.0 16.3932 \\
26.0 15.711 \\
27.0 16.8377 \\
28.0 16.6311 \\
29.0 18.4897 \\
30.0 17.4796 \\
31.0 16.8529 \\
32.0 18.0364 \\
33.0 18.1445 \\
34.0 18.6256 \\
35.0 18.4114 \\
36.0 18.3668 \\
37.0 19.0253 \\
38.0 18.992 \\
39.0 20.8654 \\
40.0 19.8163 \\
41.0 19.6268 \\
42.0 20.2705 \\
43.0 18.7645 \\
44.0 19.2518 \\
45.0 18.9208 \\
};
\addlegendentry{m=4,n=1,K=1+A1,GB}


\addplot [color=cyan!40!black,line width=1.5pt, mark options={solid, orange}, mark options={solid, violet}, mark=triangle*, mark repeat=11, mark phase=6, mark size=1pt]
  table[row sep=crcr]{%
0.0 40.0 \\
1.0 0.484264 \\
2.0 1.09819 \\
3.0 1.52502 \\
4.0 2.19258 \\
5.0 3.52974 \\
6.0 3.77516 \\
7.0 5.58648 \\
8.0 6.80835 \\
9.0 8.44117 \\
10.0 9.31998 \\
11.0 10.8441 \\
12.0 11.7804 \\
13.0 12.6766 \\
14.0 13.3693 \\
15.0 13.9604 \\
16.0 14.7396 \\
17.0 16.394 \\
18.0 16.2096 \\
19.0 17.631 \\
20.0 17.8144 \\
21.0 17.537 \\
22.0 17.6555 \\
23.0 18.7072 \\
24.0 18.4693 \\
25.0 18.1765 \\
26.0 18.6179 \\
27.0 19.0563 \\
28.0 19.6852 \\
29.0 19.1355 \\
30.0 19.7136 \\
31.0 18.4205 \\
32.0 19.2944 \\
33.0 18.2811 \\
34.0 19.5173 \\
35.0 18.6095 \\
36.0 19.388 \\
37.0 18.431 \\
38.0 18.9899 \\
39.0 18.0064 \\
40.0 18.2589 \\
41.0 17.4057 \\
42.0 18.6724 \\
43.0 18.5771 \\
44.0 17.0643 \\
45.0 18.0438 \\
  };
\addlegendentry{m=4,n=1,K=1+A2,HC}


\addplot [color=cyan,line width=1.5pt, mark options={solid, orange}, mark options={solid, violet!50!magenta}, mark=triangle*, mark repeat=11, mark phase=9, mark size=1pt]
  table[row sep=crcr]{%
0.0 25.9355 \\
1.0 0.787151 \\
2.0 0.879307 \\
3.0 1.29818 \\
4.0 2.05244 \\
5.0 2.91271 \\
6.0 3.73871 \\
7.0 5.69642 \\
8.0 7.21763 \\
9.0 8.71094 \\
10.0 9.68457 \\
11.0 10.5599 \\
12.0 11.0934 \\
13.0 12.4872 \\
14.0 13.5795 \\
15.0 14.1056 \\
16.0 14.5406 \\
17.0 16.2099 \\
18.0 16.7617 \\
19.0 16.3883 \\
20.0 17.2251 \\
21.0 17.4443 \\
22.0 17.2904 \\
23.0 18.0597 \\
24.0 17.7082 \\
25.0 18.0207 \\
26.0 17.9739 \\
27.0 18.5017 \\
28.0 18.905 \\
29.0 18.6829 \\
30.0 18.691 \\
31.0 19.067 \\
32.0 19.3642 \\
33.0 17.6402 \\
34.0 18.0685 \\
35.0 17.889 \\
36.0 19.485 \\
37.0 18.8303 \\
38.0 17.207 \\
39.0 18.0624 \\
40.0 17.7693 \\
41.0 17.7628 \\
42.0 18.5448 \\
43.0 17.9531 \\
44.0 17.8535 \\
45.0 17.6471 \\
  };
\addlegendentry{m=4,n=1,K=1+A2,GB}




\addplot [color=cyan!40!black,line width=1.5pt, mark options={solid, orange}, mark options={solid, black}, mark=*, mark repeat=11, mark size=1pt]
  table[row sep=crcr]{%
0.0 10.3088 \\
1.0 0.271321 \\
2.0 0.976929 \\
3.0 2.23312 \\
4.0 2.68476 \\
5.0 3.55822 \\
6.0 4.50096 \\
7.0 5.60106 \\
8.0 6.08816 \\
9.0 6.70698 \\
10.0 7.77006 \\
11.0 8.06121 \\
12.0 8.74328 \\
13.0 9.25784 \\
14.0 10.1572 \\
15.0 10.3985 \\
16.0 9.82386 \\
17.0 10.8689 \\
18.0 11.5651 \\
19.0 11.8955 \\
20.0 12.2675 \\
21.0 12.6843 \\
22.0 12.4386 \\
23.0 13.0344 \\
24.0 12.7822 \\
25.0 13.4108 \\
26.0 13.2267 \\
27.0 14.1568 \\
28.0 14.2052 \\
29.0 14.5222 \\
30.0 14.1124 \\
31.0 14.2007 \\
32.0 14.825 \\
33.0 15.6132 \\
34.0 14.825 \\
35.0 15.6248 \\
36.0 14.2759 \\
37.0 15.3764 \\
38.0 15.3176 \\
39.0 16.1525 \\
40.0 15.5502 \\
41.0 15.5031 \\
42.0 15.9942 \\
43.0 16.3893 \\
44.0 16.3481 \\
45.0 16.6098 \\
  };
\addlegendentry{m=4,n=1,K=2+A1,HC}

\addplot [color=cyan!40!black,line width=1.5pt, mark options={solid, orange}, mark options={solid, black}, mark=triangle*, mark repeat=11, mark phase=7, mark size=1pt]
  table[row sep=crcr]{%
0.0 11.9812 \\
1.0 0.248715 \\
2.0 0.650257 \\
3.0 1.2048 \\
4.0 1.69779 \\
5.0 2.75447 \\
6.0 3.35815 \\
7.0 3.84269 \\
8.0 3.93309 \\
9.0 4.90235 \\
10.0 5.28489 \\
11.0 5.99719 \\
12.0 7.10233 \\
13.0 7.06605 \\
14.0 7.16235 \\
15.0 7.62713 \\
16.0 8.67077 \\
17.0 8.25965 \\
18.0 9.07364 \\
19.0 9.6271 \\
20.0 9.7329 \\
21.0 10.1406 \\
22.0 10.8483 \\
23.0 10.8483 \\
24.0 10.6846 \\
25.0 10.8489 \\
26.0 11.36 \\
27.0 11.5643 \\
28.0 11.9751 \\
29.0 11.7263 \\
30.0 12.5845 \\
31.0 12.3552 \\
32.0 12.9129 \\
33.0 13.0238 \\
34.0 12.9809 \\
35.0 12.843 \\
36.0 13.812 \\
37.0 13.9637 \\
38.0 13.7027 \\
39.0 14.6209 \\
40.0 14.5523 \\
41.0 14.4336 \\
42.0 14.6586 \\
43.0 14.5314 \\
44.0 14.8808 \\
45.0 14.4263 \\
  };
\addlegendentry{m=4,n=1,K=2+A2,HC}

\addplot [color=cyan,line width=1.5pt, mark options={solid, orange}, mark options={solid, yellow}, mark=triangle*, mark repeat=11, mark phase=3, mark size=1pt]
  table[row sep=crcr]{%
0.0 0.0580188 \\
1.0 0.325863 \\
2.0 0.839748 \\
3.0 1.4315 \\
4.0 1.77721 \\
5.0 2.98979 \\
6.0 3.51212 \\
7.0 3.95683 \\
8.0 4.83111 \\
9.0 5.77778 \\
10.0 5.42215 \\
11.0 5.92159 \\
12.0 6.59239 \\
13.0 7.86358 \\
14.0 8.16592 \\
15.0 8.37757 \\
16.0 8.05863 \\
17.0 9.0665 \\
18.0 9.2721 \\
19.0 10.2872 \\
20.0 9.54462 \\
21.0 10.1443 \\
22.0 10.5171 \\
23.0 11.5166 \\
24.0 10.9174 \\
25.0 11.2673 \\
26.0 11.1151 \\
27.0 11.2702 \\
28.0 11.3417 \\
29.0 11.2164 \\
30.0 12.0144 \\
31.0 12.8601 \\
32.0 12.4737 \\
33.0 13.1811 \\
34.0 12.6169 \\
35.0 12.4474 \\
36.0 13.0733 \\
37.0 13.6353 \\
38.0 14.0458 \\
39.0 13.4964 \\
40.0 13.4943 \\
41.0 13.7345 \\
42.0 13.7546 \\
43.0 13.5142 \\
44.0 13.9767 \\
45.0 14.421 \\
  };
\addlegendentry{m=4,n=1,K=2+A2,GB}

\legend{}

\end{axis}

==> plot/appx_test_event_t.tex <==


\begin{axis}[%
width=0.35\columnwidth,
height=0.22\columnwidth,
at={(2.4in,0.389in)},
scale only axis,
xmin=0,
xmax=40,
xlabel style={font=\color{white!15!black}, yshift=0.03in},
xlabel={Ang. vel. ($^{\circ}$ / frame)},
title={Tran err ($^{\circ}$)},
ymin=0,
ymax=30,
ymode=normal,
yminorticks=true,
axis lines = left,
axis background/.style={fill=white},
title style={font=\bfseries, yshift=-0.1in},
%ylabel style={yshift=-0.15in},
%ylabel={Success rate ($\%$)},
%legend style={at={(1,1.3)}, anchor=south, legend cell align=left, align=left, draw=white!15!black, font=\normalsize,nodes={scale=1.0, transform shape}},
%legend columns=3
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addplot [color=magenta,line width=2pt, mark options={solid, red}]
  table[row sep=crcr]{%
0.0 0.0295238 \\
1.0 5.40393 \\
2.0 7.78743 \\
3.0 9.61086 \\
4.0 10.8405 \\
5.0 12.0025 \\
6.0 13.2969 \\
7.0 14.0259 \\
8.0 15.4061 \\
9.0 15.7173 \\
10.0 16.4864 \\
11.0 17.3546 \\
12.0 17.6014 \\
13.0 17.5699 \\
14.0 18.3201 \\
15.0 18.2636 \\
16.0 19.085 \\
17.0 20.1345 \\
18.0 19.9439 \\
19.0 20.5993 \\
20.0 20.2852 \\
21.0 20.1148 \\
22.0 21.1968 \\
23.0 21.275 \\
24.0 21.9623 \\
25.0 22.0935 \\
26.0 22.4699 \\
27.0 22.5022 \\
28.0 23.2747 \\
29.0 22.4835 \\
30.0 22.4285 \\
31.0 23.4644 \\
32.0 23.4076 \\
33.0 23.2753 \\
34.0 23.5566 \\
35.0 23.0511 \\
36.0 24.4182 \\
37.0 24.5082 \\
38.0 24.4673 \\
39.0 24.2551 \\
40.0 24.5867 \\
41.0 24.9884 \\
42.0 25.2501 \\
43.0 24.8187 \\
44.0 25.2996 \\
45.0 25.9283 \\
};
\addlegendentry{5 point \cite{}}

\addplot [color=green!20!yellow,line width=2pt, mark options={solid, red}]
  table[row sep=crcr]{%
0.0 0.888304 \\
1.0 0.39835 \\
2.0 0.919814 \\
3.0 1.25658 \\
4.0 1.60588 \\
5.0 2.13746 \\
6.0 2.86429 \\
7.0 3.71739 \\
8.0 4.66432 \\
9.0 5.08846 \\
10.0 5.36084 \\
11.0 6.69121 \\
12.0 7.12057 \\
13.0 7.61857 \\
14.0 8.61587 \\
15.0 9.81239 \\
16.0 9.90343 \\
17.0 10.6948 \\
18.0 10.8267 \\
19.0 10.8263 \\
20.0 12.3808 \\
21.0 12.7238 \\
22.0 12.7584 \\
23.0 13.2521 \\
24.0 13.402 \\
25.0 14.1605 \\
26.0 14.0782 \\
27.0 14.3572 \\
28.0 15.051 \\
29.0 14.9014 \\
30.0 15.5146 \\
31.0 15.6073 \\
32.0 16.0392 \\
33.0 15.1833 \\
34.0 15.8992 \\
35.0 15.4078 \\
36.0 16.3375 \\
37.0 15.9543 \\
38.0 16.4651 \\
39.0 16.525 \\
40.0 17.1497 \\
41.0 16.8509 \\
42.0 16.2565 \\
43.0 16.8761 \\
44.0 17.0387 \\
45.0 17.1538 \\
};
\addlegendentry{m=2,n=5,K=1+A2,GB3}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addplot [color=green!50!black,line width=1.5pt, mark options={solid, violet!50!magenta}, mark=triangle*, mark repeat=11, mark phase=3, mark size=0.5pt]
  table[row sep=crcr]{%
0.0 0.0680085 \\
1.0 0.468565 \\
2.0 0.826134 \\
3.0 1.19689 \\
4.0 1.87782 \\
5.0 2.54145 \\
6.0 3.33613 \\
7.0 4.01512 \\
8.0 4.08448 \\
9.0 5.50641 \\
10.0 6.14811 \\
11.0 6.2219 \\
12.0 7.29282 \\
13.0 7.5986 \\
14.0 9.028 \\
15.0 9.38085 \\
16.0 9.66067 \\
17.0 10.5784 \\
18.0 10.9666 \\
19.0 11.7027 \\
20.0 12.4025 \\
21.0 12.2158 \\
22.0 12.733 \\
23.0 12.6673 \\
24.0 13.1314 \\
25.0 13.6622 \\
26.0 13.9474 \\
27.0 14.1689 \\
28.0 14.1415 \\
29.0 15.1108 \\
30.0 15.169 \\
31.0 15.1588 \\
32.0 15.8789 \\
33.0 15.9817 \\
34.0 15.8393 \\
35.0 16.0375 \\
36.0 16.8081 \\
37.0 15.8212 \\
38.0 16.9261 \\
39.0 16.4061 \\
40.0 17.0015 \\
41.0 16.7214 \\
42.0 17.5377 \\
43.0 16.8372 \\
44.0 16.7842 \\
45.0 16.8085 \\
};
\addlegendentry{m=2,n=5,K=1,A2,HC}


\addplot [color=green!90!black,line width=1.5pt, mark options={solid, violet}, mark=triangle*, mark repeat=11, mark phase=7, mark size=0.5pt]
  table[row sep=crcr]{%
0.0 19.5712 \\
1.0 0.450075 \\
2.0 0.715022 \\
3.0 1.10829 \\
4.0 2.09965 \\
5.0 2.35336 \\
6.0 2.96093 \\
7.0 3.42486 \\
8.0 4.14373 \\
9.0 4.88621 \\
10.0 5.67953 \\
11.0 6.4525 \\
12.0 7.05306 \\
13.0 7.79551 \\
14.0 8.20732 \\
15.0 9.37248 \\
16.0 9.69866 \\
17.0 10.2173 \\
18.0 10.4468 \\
19.0 10.7764 \\
20.0 11.8426 \\
21.0 11.9242 \\
22.0 12.636 \\
23.0 12.8215 \\
24.0 13.5211 \\
25.0 13.6385 \\
26.0 13.5368 \\
27.0 14.1037 \\
28.0 15.0047 \\
29.0 14.7527 \\
30.0 15.031 \\
31.0 15.7795 \\
32.0 14.9906 \\
33.0 15.8313 \\
34.0 15.5189 \\
35.0 16.7381 \\
36.0 16.5718 \\
37.0 16.6795 \\
38.0 16.2408 \\
39.0 16.5093 \\
40.0 16.0766 \\
41.0 17.3691 \\
42.0 17.4648 \\
43.0 16.7806 \\
44.0 17.2999 \\
45.0 18.1325 \\
   }; 
\addlegendentry{m=2,n=5,K=1,A2,GB5}


%\addplot [color=green!20!yellow,line width=1.5pt, mark options={solid, orange}]
%  table[row sep=crcr]{%
%  1.3340502686000278e-20 0 \\
%   }; 
%\addlegendentry{m=2,n=5,K=1,A2,GB5}

\addplot [color=green!50!black,line width=1.5pt, mark options={solid, violet!50!magenta}, mark=*, mark repeat=11, mark size=1pt]
  table[row sep=crcr]{%
0.0 0.00565589 \\
1.0 0.248956 \\
2.0 0.387675 \\
3.0 0.687467 \\
4.0 1.25101 \\
5.0 1.56909 \\
6.0 2.03988 \\
7.0 2.29278 \\
8.0 3.05995 \\
9.0 3.17405 \\
10.0 3.96465 \\
11.0 4.32642 \\
12.0 5.19985 \\
13.0 5.55154 \\
14.0 5.91054 \\
15.0 6.291 \\
16.0 6.73996 \\
17.0 7.26452 \\
18.0 7.43652 \\
19.0 8.64017 \\
20.0 8.42627 \\
21.0 8.90608 \\
22.0 9.60014 \\
23.0 9.5668 \\
24.0 10.2674 \\
25.0 10.5882 \\
26.0 11.042 \\
27.0 10.9875 \\
28.0 10.6041 \\
29.0 11.4942 \\
30.0 11.5936 \\
31.0 12.0513 \\
32.0 11.9049 \\
33.0 11.8846 \\
34.0 12.7914 \\
35.0 12.7631 \\
36.0 12.6459 \\
37.0 12.8998 \\
38.0 12.9424 \\
39.0 13.3527 \\
40.0 13.9433 \\
41.0 13.1388 \\
42.0 13.9104 \\
43.0 13.351 \\
44.0 13.7324 \\
45.0 14.4969 \\
   }; 
\addlegendentry{m=2,n=5,K=1,A1,HC}

\addplot [color=green!50!black,line width=1.5pt, mark options={solid,violet, draw=black,fill=violet}, mark=triangle*, mark repeat=11, mark size=0.4pt, mark phase=3]
  table[row sep=crcr]{%
0.0 0.0712007 \\
1.0 0.0282025 \\
2.0 0.102561 \\
3.0 0.182324 \\
4.0 0.317151 \\
5.0 0.547334 \\
6.0 0.544799 \\
7.0 0.964559 \\
8.0 1.14227 \\
9.0 1.37981 \\
10.0 2.04475 \\
11.0 2.08049 \\
12.0 2.44061 \\
13.0 2.56781 \\
14.0 2.75565 \\
15.0 3.14398 \\
16.0 3.1681 \\
17.0 3.60146 \\
18.0 3.81367 \\
19.0 4.32211 \\
20.0 4.58418 \\
21.0 4.80082 \\
22.0 4.90011 \\
23.0 5.26036 \\
24.0 5.3747 \\
25.0 5.71672 \\
26.0 5.95655 \\
27.0 6.20765 \\
28.0 6.62395 \\
29.0 6.61303 \\
30.0 6.7897 \\
31.0 7.07693 \\
32.0 7.15826 \\
33.0 7.54138 \\
34.0 7.88044 \\
35.0 8.05797 \\
36.0 7.91742 \\
37.0 7.92804 \\
38.0 8.60932 \\
39.0 7.75499 \\
40.0 8.70647 \\
41.0 9.0286 \\
42.0 8.8474 \\
43.0 9.43489 \\
44.0 9.59362 \\
45.0 9.5614 \\
   }; 
\addlegendentry{m=2,n=5,K=2,A2,HC}



\legend{}

\end{axis}

==> plot/appx_test_t.tex <==


\begin{axis}[%
width=0.35\columnwidth,
height=0.22\columnwidth,
at={(2.4in,0.389in)},
scale only axis,
xmin=0,
xmax=40,
xlabel style={font=\color{white!15!black}, yshift=0.03in},
xlabel={Ang. vel. ($^{\circ}$ / frame)},
title={Tran err ($^{\circ}$)},
ymin=0,
ymax=25,
ymode=normal,
yminorticks=true,
axis lines = left,
axis background/.style={fill=white},
title style={font=\bfseries, yshift=-0.1in},
%ylabel style={yshift=-0.15in},
%ylabel={Success rate ($\%$)},
%legend style={at={(1,1.3)}, anchor=south, legend cell align=left, align=left, draw=white!15!black, font=\normalsize,nodes={scale=1.0, transform shape}},
%legend columns=3
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addplot [color=magenta,line width=2pt, mark options={solid, red}]
  table[row sep=crcr]{%
0.0 0.0754183 \\
1.0 1.98385 \\
2.0 3.12389 \\
3.0 3.88439 \\
4.0 5.03135 \\
5.0 5.68055 \\
6.0 6.63679 \\
7.0 7.83389 \\
8.0 8.48627 \\
9.0 8.61269 \\
10.0 9.57822 \\
11.0 10.062 \\
12.0 10.6393 \\
13.0 10.4317 \\
14.0 11.1699 \\
15.0 12.2071 \\
16.0 12.9732 \\
17.0 12.9787 \\
18.0 13.0163 \\
19.0 13.6352 \\
20.0 14.7668 \\
21.0 15.1024 \\
22.0 15.502 \\
23.0 15.2776 \\
24.0 15.5847 \\
25.0 16.2476 \\
26.0 16.559 \\
27.0 16.1505 \\
28.0 17.1729 \\
29.0 17.7646 \\
30.0 17.8187 \\
31.0 17.9756 \\
32.0 18.4674 \\
33.0 18.9158 \\
34.0 19.6416 \\
35.0 19.8163 \\
36.0 19.5328 \\
37.0 20.2527 \\
38.0 19.9859 \\
39.0 20.5231 \\
40.0 20.5732 \\
41.0 21.3242 \\
42.0 21.6336 \\
43.0 21.4596 \\
44.0 21.3453 \\
45.0 21.6496 \\
};
\addlegendentry{5 point \cite{}}

\addplot [color=green!20!yellow,line width=2pt, mark options={solid, red}]
  table[row sep=crcr]{%
0.0 2.03654 \\
1.0 0.28479 \\
2.0 0.344499 \\
3.0 0.808347 \\
4.0 1.11722 \\
5.0 1.72236 \\
6.0 1.78495 \\
7.0 2.04359 \\
8.0 2.75591 \\
9.0 2.99381 \\
10.0 3.29988 \\
11.0 3.65562 \\
12.0 4.10759 \\
13.0 4.30394 \\
14.0 4.81624 \\
15.0 5.65019 \\
16.0 5.67737 \\
17.0 6.80344 \\
18.0 6.74345 \\
19.0 6.81016 \\
20.0 7.71882 \\
21.0 7.88935 \\
22.0 8.63112 \\
23.0 8.86291 \\
24.0 9.71148 \\
25.0 9.90786 \\
26.0 10.341 \\
27.0 10.7497 \\
28.0 11.2126 \\
29.0 10.6676 \\
30.0 11.913 \\
31.0 12.1631 \\
32.0 12.6458 \\
33.0 12.6283 \\
34.0 13.2181 \\
35.0 13.5529 \\
36.0 13.7201 \\
37.0 14.1795 \\
38.0 13.516 \\
39.0 14.0745 \\
40.0 14.7425 \\
41.0 15.091 \\
42.0 14.8136 \\
43.0 15.7803 \\
44.0 14.6686 \\
45.0 15.4265 \\
};
\addlegendentry{m=2,n=5,K=1+A2,GB3}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addplot [color=green!50!black,line width=1.5pt, mark options={solid, violet!50!magenta}, mark=triangle*, mark repeat=11, mark phase=3, mark size=0.5pt]
  table[row sep=crcr]{%
0.0 0.0649043 \\
1.0 0.137694 \\
2.0 0.40846 \\
3.0 0.746185 \\
4.0 1.21239 \\
5.0 1.60141 \\
6.0 1.78061 \\
7.0 1.92056 \\
8.0 2.06002 \\
9.0 2.68262 \\
10.0 3.40499 \\
11.0 3.81994 \\
12.0 3.93293 \\
13.0 4.77633 \\
14.0 4.95503 \\
15.0 5.36032 \\
16.0 5.64635 \\
17.0 6.21562 \\
18.0 6.55125 \\
19.0 7.41033 \\
20.0 7.93223 \\
21.0 8.41288 \\
22.0 8.39496 \\
23.0 9.29366 \\
24.0 9.94255 \\
25.0 10.385 \\
26.0 11.2094 \\
27.0 10.719 \\
28.0 12.0479 \\
29.0 11.7929 \\
30.0 12.1468 \\
31.0 12.3059 \\
32.0 12.7401 \\
33.0 12.7879 \\
34.0 13.2953 \\
35.0 13.5744 \\
36.0 14.0223 \\
37.0 13.918 \\
38.0 14.0894 \\
39.0 14.2658 \\
40.0 14.0855 \\
41.0 14.6188 \\
42.0 14.6033 \\
43.0 15.4433 \\
44.0 15.5314 \\
45.0 15.2754 \\
};
\addlegendentry{m=2,n=5,K=1,A2,HC}


\addplot [color=green!90!black,line width=1.5pt, mark options={solid, violet}, mark=triangle*, mark repeat=11, mark phase=7, mark size=0.5pt]
  table[row sep=crcr]{%
0.0 17.9635 \\
1.0 0.200164 \\
2.0 0.388281 \\
3.0 0.674539 \\
4.0 0.809545 \\
5.0 1.11609 \\
6.0 1.44991 \\
7.0 2.06558 \\
8.0 2.58811 \\
9.0 2.87061 \\
10.0 3.4871 \\
11.0 3.70748 \\
12.0 3.98159 \\
13.0 4.66411 \\
14.0 4.65531 \\
15.0 4.9703 \\
16.0 5.92295 \\
17.0 6.2096 \\
18.0 6.80792 \\
19.0 7.17662 \\
20.0 7.58284 \\
21.0 8.03358 \\
22.0 8.88474 \\
23.0 8.80992 \\
24.0 9.56936 \\
25.0 10.0014 \\
26.0 10.0858 \\
27.0 10.9526 \\
28.0 11.3379 \\
29.0 10.9686 \\
30.0 11.7125 \\
31.0 11.734 \\
32.0 12.7615 \\
33.0 12.519 \\
34.0 13.4493 \\
35.0 13.6531 \\
36.0 14.0161 \\
37.0 14.2295 \\
38.0 14.8674 \\
39.0 14.2631 \\
40.0 14.9929 \\
41.0 15.4994 \\
42.0 15.1299 \\
43.0 16.0908 \\
44.0 16.5179 \\
45.0 16.545 \\
   }; 
\addlegendentry{m=2,n=5,K=1,A2,GB5}


%\addplot [color=green!20!yellow,line width=1.5pt, mark options={solid, orange}]
%  table[row sep=crcr]{%
%  1.3340502686000278e-20 0 \\
%   }; 
%\addlegendentry{m=2,n=5,K=1,A2,GB5}

\addplot [color=green!50!black,line width=1.5pt, mark options={solid, violet!50!magenta}, mark=*, mark repeat=11, mark size=1pt]
  table[row sep=crcr]{%
0.0 0.0390187 \\
1.0 0.130982 \\
2.0 0.377602 \\
3.0 0.609749 \\
4.0 0.643912 \\
5.0 0.932389 \\
6.0 1.27132 \\
7.0 1.46429 \\
8.0 1.89292 \\
9.0 2.00179 \\
10.0 2.47113 \\
11.0 2.95188 \\
12.0 3.17832 \\
13.0 3.61713 \\
14.0 3.9728 \\
15.0 4.2419 \\
16.0 4.84071 \\
17.0 5.03692 \\
18.0 5.3953 \\
19.0 5.82678 \\
20.0 6.09927 \\
21.0 6.19267 \\
22.0 6.85813 \\
23.0 7.08603 \\
24.0 6.98464 \\
25.0 7.58535 \\
26.0 7.87985 \\
27.0 8.6056 \\
28.0 8.55317 \\
29.0 8.79898 \\
30.0 9.01737 \\
31.0 9.20355 \\
32.0 10.2314 \\
33.0 10.3813 \\
34.0 10.1025 \\
35.0 10.3995 \\
36.0 10.3094 \\
37.0 10.9559 \\
38.0 10.9395 \\
39.0 10.9846 \\
40.0 11.0998 \\
41.0 12.1452 \\
42.0 11.944 \\
43.0 11.7539 \\
44.0 12.1153 \\
45.0 12.1515 \\
   }; 
\addlegendentry{m=2,n=5,K=1,A1,HC}

\addplot [color=green!50!black,line width=1.5pt, mark options={solid,violet, draw=black,fill=violet}, mark=triangle*, mark repeat=11, mark size=0.4pt, mark phase=3]
  table[row sep=crcr]{%
0.0 0.0253505 \\
1.0 0.0957173 \\
2.0 0.094639 \\
3.0 0.122277 \\
4.0 0.190873 \\
5.0 0.290176 \\
6.0 0.292274 \\
7.0 0.52553 \\
8.0 0.526289 \\
9.0 0.607581 \\
10.0 0.78599 \\
11.0 1.19481 \\
12.0 1.10794 \\
13.0 1.41683 \\
14.0 1.30512 \\
15.0 1.76209 \\
16.0 1.54488 \\
17.0 2.03979 \\
18.0 2.15368 \\
19.0 2.39609 \\
20.0 2.50203 \\
21.0 3.08071 \\
22.0 3.27019 \\
23.0 3.30295 \\
24.0 3.53848 \\
25.0 3.67174 \\
26.0 4.01383 \\
27.0 4.3184 \\
28.0 4.29224 \\
29.0 4.64861 \\
30.0 4.70933 \\
31.0 4.90339 \\
32.0 5.07798 \\
33.0 5.30382 \\
34.0 5.38126 \\
35.0 6.19191 \\
36.0 5.87337 \\
37.0 6.35895 \\
38.0 6.35433 \\
39.0 6.91603 \\
40.0 7.0981 \\
41.0 6.94717 \\
42.0 7.1209 \\
43.0 7.25585 \\
44.0 7.3294 \\
45.0 7.74752 \\
   }; 
\addlegendentry{m=2,n=5,K=2,A2,HC}



\legend{}

\end{axis}

==> plot/noise_test_event_t.tex <==


\begin{axis}[%
width=0.35\columnwidth,
height=0.2\columnwidth,
at={(2.4in,0.389in)},
scale only axis,
xmin=0,
xmax=40,
xlabel style={font=\color{white!15!black}, yshift=0.03in},
xlabel={Ang. vel. ($^{\circ}$ / frame)},
title={Tran err ($^{\circ}$)},
ymin=0,
ymax=30,
ymode=normal,
yminorticks=true,
axis lines = left,
axis background/.style={fill=white},
title style={font=\bfseries, yshift=-0.1in},
%ylabel style={yshift=-0.15in},
%ylabel={Success rate ($\%$)},
%legend style={at={(1,1.3)}, anchor=south, legend cell align=left, align=left, draw=white!15!black, font=\normalsize,nodes={scale=1.0, transform shape}},
%legend columns=3
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addplot [color=magenta,line width=2pt, mark options={solid, red}]
  table[row sep=crcr]{%
0.0 2.55691 \\
1.0 5.29081 \\
2.0 8.08509 \\
3.0 10.0311 \\
4.0 10.8145 \\
5.0 12.2644 \\
6.0 13.7649 \\
7.0 14.3361 \\
8.0 15.0758 \\
9.0 15.942 \\
10.0 16.0862 \\
11.0 17.0274 \\
12.0 18.1551 \\
13.0 17.5772 \\
14.0 17.8022 \\
15.0 19.151 \\
16.0 19.5058 \\
17.0 20.0089 \\
18.0 18.8891 \\
19.0 19.9996 \\
20.0 20.434 \\
21.0 20.4443 \\
22.0 20.5908 \\
23.0 21.0238 \\
24.0 22.2578 \\
25.0 21.3952 \\
26.0 22.0817 \\
27.0 22.7676 \\
28.0 22.5996 \\
29.0 22.7545 \\
30.0 23.3283 \\
31.0 22.9134 \\
32.0 22.8835 \\
33.0 23.6536 \\
34.0 24.0964 \\
35.0 23.8326 \\
36.0 23.9643 \\
37.0 24.8487 \\
38.0 23.9295 \\
39.0 23.8897 \\
40.0 24.6958 \\
41.0 25.3846 \\
42.0 25.4832 \\
43.0 24.2851 \\
44.0 25.5781 \\
45.0 25.8743 \\
};
\addlegendentry{5 point \cite{DBLP:journals/pami/Nister04}}

\addplot [color=green!20!yellow,line width=2pt, mark options={solid, red}]
  table[row sep=crcr]{%
0.0 4.44624 \\
1.0 4.69802 \\
2.0 4.79111 \\
3.0 4.46066 \\
4.0 4.25987 \\
5.0 4.45934 \\
6.0 5.09795 \\
7.0 4.8904 \\
8.0 5.64351 \\
9.0 6.17426 \\
10.0 6.23683 \\
11.0 7.69632 \\
12.0 8.2866 \\
13.0 9.26862 \\
14.0 9.43752 \\
15.0 9.43505 \\
16.0 10.2058 \\
17.0 11.2406 \\
18.0 10.7707 \\
19.0 11.494 \\
20.0 12.1039 \\
21.0 12.1486 \\
22.0 13.0823 \\
23.0 13.116 \\
24.0 13.4377 \\
25.0 14.3841 \\
26.0 14.1324 \\
27.0 14.4922 \\
28.0 14.491 \\
29.0 15.0069 \\
30.0 15.162 \\
31.0 15.5158 \\
32.0 15.3947 \\
33.0 15.4927 \\
34.0 16.0684 \\
35.0 15.761 \\
36.0 16.7135 \\
37.0 16.6611 \\
38.0 16.4628 \\
39.0 15.453 \\
40.0 16.1744 \\
41.0 17.1134 \\
42.0 17.5022 \\
43.0 16.4375 \\
44.0 17.6202 \\
45.0 16.9478 \\
};
\addlegendentry{m=2,n=5,K=1+A2,GB3}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addplot [color=green!50!black,line width=1.5pt, mark options={solid, violet!50!magenta}, mark=triangle*, mark repeat=11, mark phase=3, mark size=0.5pt]
  table[row sep=crcr]{%
0.0 4.12736 \\
1.0 4.64434 \\
2.0 4.48736 \\
3.0 4.27492 \\
4.0 4.06448 \\
5.0 4.73131 \\
6.0 4.90358 \\
7.0 5.373 \\
8.0 5.36999 \\
9.0 6.19056 \\
10.0 7.29864 \\
11.0 7.51409 \\
12.0 7.94757 \\
13.0 8.87455 \\
14.0 9.25648 \\
15.0 9.76317 \\
16.0 9.80051 \\
17.0 10.6191 \\
18.0 11.1016 \\
19.0 11.6323 \\
20.0 11.7827 \\
21.0 12.1882 \\
22.0 13.7933 \\
23.0 13.87 \\
24.0 13.484 \\
25.0 14.4986 \\
26.0 14.2152 \\
27.0 14.3111 \\
28.0 15.162 \\
29.0 14.6678 \\
30.0 15.3667 \\
31.0 15.3363 \\
32.0 15.4978 \\
33.0 16.3786 \\
34.0 15.1769 \\
35.0 16.0747 \\
36.0 16.5664 \\
37.0 16.4963 \\
38.0 16.927 \\
39.0 16.685 \\
40.0 17.054 \\
41.0 17.1911 \\
42.0 17.3377 \\
43.0 16.9755 \\
44.0 17.3475 \\
45.0 17.0317 \\
};
\addlegendentry{m=2,n=5,K=1,A2,HC}


\addplot [color=green!90!black,line width=1.5pt, mark options={solid, violet}, mark=triangle*, mark repeat=11, mark phase=7, mark size=0.5pt]
  table[row sep=crcr]{%
0.0 4.17134 \\
1.0 3.77529 \\
2.0 4.19062 \\
3.0 4.58346 \\
4.0 4.42642 \\
5.0 4.60888 \\
6.0 4.37652 \\
7.0 5.45731 \\
8.0 6.05292 \\
9.0 6.02462 \\
10.0 6.81304 \\
11.0 6.77447 \\
12.0 7.64944 \\
13.0 8.07206 \\
14.0 8.63404 \\
15.0 8.92646 \\
16.0 9.85755 \\
17.0 10.5787 \\
18.0 11.0902 \\
19.0 11.2695 \\
20.0 11.1373 \\
21.0 12.2098 \\
22.0 12.8104 \\
23.0 13.5511 \\
24.0 13.6245 \\
25.0 13.6822 \\
26.0 14.143 \\
27.0 13.8514 \\
28.0 14.7015 \\
29.0 14.9722 \\
30.0 15.5789 \\
31.0 15.034 \\
32.0 15.7137 \\
33.0 15.6437 \\
34.0 16.2516 \\
35.0 16.4343 \\
36.0 16.033 \\
37.0 15.8996 \\
38.0 16.4031 \\
39.0 17.0645 \\
40.0 17.0068 \\
41.0 17.0663 \\
42.0 17.7474 \\
43.0 16.8419 \\
44.0 17.3443 \\
45.0 17.9746 \\
   }; 
\addlegendentry{m=2,n=5,K=1,A2,GB5}


%\addplot [color=green!20!yellow,line width=1.5pt, mark options={solid, orange}]
%  table[row sep=crcr]{%
%  1.3340502686000278e-20 0 \\
%   }; 
%\addlegendentry{m=2,n=5,K=1,A2,GB5}

\addplot [color=green!50!black,line width=1.5pt, mark options={solid, violet!50!magenta}, mark=*, mark repeat=11, mark size=1pt]
  table[row sep=crcr]{%
0.0 2.27512 \\
1.0 2.35913 \\
2.0 2.45346 \\
3.0 2.56059 \\
4.0 2.50166 \\
5.0 2.7583 \\
6.0 3.00035 \\
7.0 3.4994 \\
8.0 4.01573 \\
9.0 4.23368 \\
10.0 4.63117 \\
11.0 4.6429 \\
12.0 5.4091 \\
13.0 5.75349 \\
14.0 6.10375 \\
15.0 6.74148 \\
16.0 7.36518 \\
17.0 7.9644 \\
18.0 8.02729 \\
19.0 8.57684 \\
20.0 8.47935 \\
21.0 9.52912 \\
22.0 10.0978 \\
23.0 9.81981 \\
24.0 9.77264 \\
25.0 9.90049 \\
26.0 10.0729 \\
27.0 10.8783 \\
28.0 11.3465 \\
29.0 10.9245 \\
30.0 11.1053 \\
31.0 11.9389 \\
32.0 12.1831 \\
33.0 12.093 \\
34.0 12.4503 \\
35.0 12.6684 \\
36.0 12.3066 \\
37.0 12.4462 \\
38.0 13.2132 \\
39.0 13.1778 \\
40.0 13.3261 \\
41.0 13.2053 \\
42.0 13.9251 \\
43.0 13.8041 \\
44.0 14.1137 \\
45.0 14.3915 \\
   }; 
\addlegendentry{m=2,n=5,K=1,A1,HC}

\addplot [color=green!50!black,line width=1.5pt, mark options={solid,violet, draw=black,fill=violet}, mark=triangle*, mark repeat=11, mark size=0.4pt, mark phase=3]
  table[row sep=crcr]{%
0.0 2.71561 \\
1.0 2.86339 \\
2.0 3.03414 \\
3.0 2.87033 \\
4.0 2.85517 \\
5.0 2.66032 \\
6.0 2.69355 \\
7.0 2.99424 \\
8.0 3.30912 \\
9.0 3.14361 \\
10.0 3.43352 \\
11.0 3.45525 \\
12.0 3.6783 \\
13.0 3.83152 \\
14.0 4.17814 \\
15.0 4.17721 \\
16.0 4.28438 \\
17.0 4.76633 \\
18.0 4.73558 \\
19.0 4.5852 \\
20.0 5.02741 \\
21.0 5.67357 \\
22.0 5.36467 \\
23.0 5.67176 \\
24.0 6.00504 \\
25.0 6.03542 \\
26.0 6.15665 \\
27.0 6.54635 \\
28.0 6.78141 \\
29.0 7.12968 \\
30.0 7.30029 \\
31.0 7.66012 \\
32.0 7.55877 \\
33.0 7.94984 \\
34.0 8.45911 \\
35.0 8.17242 \\
36.0 7.93061 \\
37.0 8.36942 \\
38.0 8.31813 \\
39.0 8.47686 \\
40.0 8.69353 \\
41.0 8.86337 \\
42.0 9.05162 \\
43.0 9.2339 \\
44.0 9.31422 \\
45.0 9.4371 \\
   }; 
\addlegendentry{m=2,n=5,K=2,A2,HC}




\legend{}

\end{axis}

==> plot/noise_test_event_t_3v.tex <==


\begin{axis}[%
width=0.35\columnwidth,
height=0.2\columnwidth,
at={(2.4in,0.389in)},
scale only axis,
xmin=0,
xmax=40,
xlabel style={font=\color{white!15!black}, yshift=0.03in},
xlabel={Ang. vel. ($^{\circ}$ / frame)},
title={Tran err ($^{\circ}$)},
ymin=0,
ymax=30,
ymode=normal,
yminorticks=true,
axis lines = left,
axis background/.style={fill=white},
title style={font=\bfseries, yshift=-0.1in},
%ylabel style={yshift=-0.15in},
%ylabel={Success rate ($\%$)},
%legend style={at={(1,1.3)}, anchor=south, legend cell align=left, align=left, draw=white!15!black, font=\normalsize,nodes={scale=1.0, transform shape}},
%legend columns=3
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addplot [color=magenta,line width=2pt, mark options={solid, red}]
  table[row sep=crcr]{%
0.0 2.55691 \\
1.0 5.29081 \\
2.0 8.08509 \\
3.0 10.0311 \\
4.0 10.8145 \\
5.0 12.2644 \\
6.0 13.7649 \\
7.0 14.3361 \\
8.0 15.0758 \\
9.0 15.942 \\
10.0 16.0862 \\
11.0 17.0274 \\
12.0 18.1551 \\
13.0 17.5772 \\
14.0 17.8022 \\
15.0 19.151 \\
16.0 19.5058 \\
17.0 20.0089 \\
18.0 18.8891 \\
19.0 19.9996 \\
20.0 20.434 \\
21.0 20.4443 \\
22.0 20.5908 \\
23.0 21.0238 \\
24.0 22.2578 \\
25.0 21.3952 \\
26.0 22.0817 \\
27.0 22.7676 \\
28.0 22.5996 \\
29.0 22.7545 \\
30.0 23.3283 \\
31.0 22.9134 \\
32.0 22.8835 \\
33.0 23.6536 \\
34.0 24.0964 \\
35.0 23.8326 \\
36.0 23.9643 \\
37.0 24.8487 \\
38.0 23.9295 \\
39.0 23.8897 \\
40.0 24.6958 \\
41.0 25.3846 \\
42.0 25.4832 \\
43.0 24.2851 \\
44.0 25.5781 \\
45.0 25.8743 \\
};
\addlegendentry{5 point \cite{DBLP:journals/pami/Nister04}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\addplot [color=orange!50!black,line width=1.5pt, mark options={solid, orange}, mark options={solid, cyan}, mark=*, mark repeat=11, mark phase = 3, mark size=1pt]
  table[row sep=crcr]{%
0.0 6.01393 \\
1.0 5.87833 \\
2.0 5.64267 \\
3.0 5.57762 \\
4.0 5.8727 \\
5.0 6.17798 \\
6.0 6.08312 \\
7.0 6.91296 \\
8.0 7.17257 \\
9.0 7.8374 \\
10.0 8.40181 \\
11.0 9.00969 \\
12.0 9.5965 \\
13.0 10.718 \\
14.0 10.5846 \\
15.0 11.0109 \\
16.0 11.9661 \\
17.0 12.9544 \\
18.0 13.4163 \\
19.0 13.4694 \\
20.0 14.2861 \\
21.0 14.1582 \\
22.0 14.4304 \\
23.0 15.3762 \\
24.0 14.9746 \\
25.0 15.4153 \\
26.0 15.6276 \\
27.0 16.0248 \\
28.0 16.7065 \\
29.0 16.5208 \\
30.0 16.8892 \\
31.0 16.7247 \\
32.0 17.2393 \\
33.0 17.0022 \\
34.0 17.0169 \\
35.0 18.1015 \\
36.0 17.9838 \\
37.0 17.8576 \\
38.0 17.5527 \\
39.0 17.9417 \\
40.0 17.5086 \\
41.0 18.1148 \\
42.0 18.0259 \\
43.0 17.6086 \\
44.0 17.7359 \\
45.0 18.6533 \\
  };
\addlegendentry{m=3,n=2,K=1+A1,HC}


\addplot [color=orange,line width=1.5pt, mark options={solid, orange}, mark options={solid, violet}, mark=*, mark repeat=11, mark phase = 5, mark size=1pt]
  table[row sep=crcr]{%
0.0 5.12512 \\
1.0 5.71835 \\
2.0 5.76868 \\
3.0 5.74292 \\
4.0 6.03484 \\
5.0 6.57589 \\
6.0 6.36493 \\
7.0 6.8369 \\
8.0 7.0473 \\
9.0 8.02502 \\
10.0 8.54733 \\
11.0 9.18031 \\
12.0 9.57884 \\
13.0 10.3519 \\
14.0 10.7898 \\
15.0 11.1298 \\
16.0 11.8696 \\
17.0 12.9287 \\
18.0 12.4289 \\
19.0 13.3926 \\
20.0 14.1932 \\
21.0 14.5459 \\
22.0 14.5406 \\
23.0 15.378 \\
24.0 15.1006 \\
25.0 15.847 \\
26.0 15.9139 \\
27.0 16.0379 \\
28.0 16.8552 \\
29.0 16.3227 \\
30.0 15.9227 \\
31.0 16.774 \\
32.0 17.2907 \\
33.0 16.7552 \\
34.0 17.4646 \\
35.0 16.9681 \\
36.0 17.4611 \\
37.0 17.5125 \\
38.0 17.6404 \\
39.0 17.9056 \\
40.0 17.9769 \\
41.0 17.9932 \\
42.0 17.8711 \\
43.0 17.6015 \\
44.0 18.6976 \\
45.0 18.4232 \\
  };
\addlegendentry{m=3,n=2,K=1+A1,GB}


\addplot [color=orange!50!black,line width=1.5pt, mark options={solid, orange}, mark options={solid, cyan}, mark=triangle*, mark repeat=11, mark phase = 7, mark size=1pt]
  table[row sep=crcr]{%
0.0 6.26213 \\
1.0 5.82458 \\
2.0 6.34161 \\
3.0 6.33413 \\
4.0 6.44948 \\
5.0 6.88065 \\
6.0 6.51017 \\
7.0 7.18947 \\
8.0 7.92506 \\
9.0 8.26297 \\
10.0 8.38141 \\
11.0 9.37548 \\
12.0 10.4014 \\
13.0 10.7449 \\
14.0 11.9982 \\
15.0 11.9992 \\
16.0 12.9626 \\
17.0 13.0828 \\
18.0 13.9759 \\
19.0 14.131 \\
20.0 14.6692 \\
21.0 14.9023 \\
22.0 15.571 \\
23.0 15.593 \\
24.0 16.4872 \\
25.0 15.8504 \\
26.0 16.4289 \\
27.0 16.9448 \\
28.0 16.1429 \\
29.0 17.1917 \\
30.0 16.8229 \\
31.0 17.7819 \\
32.0 16.9543 \\
33.0 16.8652 \\
34.0 16.7222 \\
35.0 17.2698 \\
36.0 18.6597 \\
37.0 17.233 \\
38.0 16.9429 \\
39.0 17.4538 \\
40.0 17.9114 \\
41.0 18.1757 \\
42.0 17.9522 \\
43.0 18.3315 \\
44.0 17.8936 \\
45.0 18.2131 \\
  };
\addlegendentry{m=3,n=2,K=1+A2,HC}


\addplot [color=orange,line width=1.5pt, mark options={solid, orange}, mark options={solid, violet}, mark=triangle*, mark repeat=11, mark size=1pt]
  table[row sep=crcr]{%
0.0 6.85341 \\
1.0 6.97485 \\
2.0 6.55225 \\
3.0 6.88598 \\
4.0 6.60238 \\
5.0 6.55896 \\
6.0 6.9479 \\
7.0 7.746 \\
8.0 7.33197 \\
9.0 7.90672 \\
10.0 9.24229 \\
11.0 9.1568 \\
12.0 9.85381 \\
13.0 11.3298 \\
14.0 11.6518 \\
15.0 11.5602 \\
16.0 12.3991 \\
17.0 13.6664 \\
18.0 14.2669 \\
19.0 14.222 \\
20.0 15.1141 \\
21.0 14.9783 \\
22.0 15.1017 \\
23.0 15.1164 \\
24.0 15.7984 \\
25.0 15.7122 \\
26.0 16.2185 \\
27.0 17.06 \\
28.0 16.5386 \\
29.0 16.5628 \\
30.0 16.8521 \\
31.0 16.6386 \\
32.0 16.8476 \\
33.0 17.2983 \\
34.0 17.4213 \\
35.0 18.2659 \\
36.0 17.5214 \\
37.0 17.1389 \\
38.0 17.6452 \\
39.0 17.6921 \\
40.0 17.5837 \\
41.0 18.0932 \\
42.0 17.7879 \\
43.0 18.1624 \\
44.0 17.9241 \\
45.0 17.9802 \\
  };
\addlegendentry{m=3,n=2,K=1+A2,GB}




\addplot [color=orange!50!black,line width=1.5pt, mark options={solid, orange}, mark options={solid, black}, mark=*, mark repeat=11, mark size=1pt]
  table[row sep=crcr]{%
0.0 3.35116 \\
  };
\addlegendentry{m=3,n=2,K=2+A1,HC}

\addplot [color=orange!50!black,line width=1.5pt, mark options={solid, orange}, mark options={solid, black}, mark=triangle*, mark repeat=11, mark size=1pt]
  table[row sep=crcr]{%
0.0 3.35116 \\
1.0 3.50206 \\
2.0 3.50109 \\
3.0 3.59316 \\
4.0 3.95622 \\
5.0 3.94814 \\
6.0 3.61068 \\
7.0 3.97417 \\
8.0 4.32538 \\
9.0 4.21185 \\
10.0 4.55192 \\
11.0 4.35496 \\
12.0 4.78152 \\
13.0 4.75762 \\
14.0 5.38918 \\
15.0 5.4319 \\
16.0 5.65845 \\
17.0 6.14617 \\
18.0 6.39859 \\
19.0 6.64534 \\
20.0 6.60941 \\
21.0 6.91793 \\
22.0 7.05679 \\
23.0 7.34075 \\
24.0 7.67204 \\
25.0 7.72236 \\
26.0 7.70093 \\
27.0 8.32095 \\
28.0 8.43273 \\
29.0 8.58592 \\
30.0 8.39171 \\
31.0 9.27632 \\
32.0 9.11454 \\
33.0 9.10379 \\
34.0 9.60949 \\
35.0 9.02604 \\
36.0 9.75639 \\
37.0 10.1934 \\
38.0 10.0669 \\
39.0 10.0977 \\
40.0 10.0016 \\
41.0 10.6494 \\
42.0 10.8908 \\
43.0 10.8118 \\
44.0 10.7967 \\
45.0 10.6807 \\
  };
\addlegendentry{m=3,n=2,K=2+A2,GB}







\legend{}

\end{axis}

==> plot/noise_test_event_t_4v.tex <==


\begin{axis}[%
width=0.35\columnwidth,
height=0.2\columnwidth,
at={(2.4in,0.389in)},
scale only axis,
xmin=0,
xmax=40,
xlabel style={font=\color{white!15!black}, yshift=0.03in},
xlabel={Ang. vel. ($^{\circ}$ / frame)},
title={Tran err ($^{\circ}$)},
ymin=0,
ymax=30,
ymode=normal,
yminorticks=true,
axis lines = left,
axis background/.style={fill=white},
title style={font=\bfseries, yshift=-0.1in},
%ylabel style={yshift=-0.15in},
%ylabel={Success rate ($\%$)},
%legend style={at={(1,1.3)}, anchor=south, legend cell align=left, align=left, draw=white!15!black, font=\normalsize,nodes={scale=1.0, transform shape}},
%legend columns=3
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addplot [color=magenta,line width=2pt, mark options={solid, red}]
  table[row sep=crcr]{%
0.0 2.55691 \\
1.0 5.29081 \\
2.0 8.08509 \\
3.0 10.0311 \\
4.0 10.8145 \\
5.0 12.2644 \\
6.0 13.7649 \\
7.0 14.3361 \\
8.0 15.0758 \\
9.0 15.942 \\
10.0 16.0862 \\
11.0 17.0274 \\
12.0 18.1551 \\
13.0 17.5772 \\
14.0 17.8022 \\
15.0 19.151 \\
16.0 19.5058 \\
17.0 20.0089 \\
18.0 18.8891 \\
19.0 19.9996 \\
20.0 20.434 \\
21.0 20.4443 \\
22.0 20.5908 \\
23.0 21.0238 \\
24.0 22.2578 \\
25.0 21.3952 \\
26.0 22.0817 \\
27.0 22.7676 \\
28.0 22.5996 \\
29.0 22.7545 \\
30.0 23.3283 \\
31.0 22.9134 \\
32.0 22.8835 \\
33.0 23.6536 \\
34.0 24.0964 \\
35.0 23.8326 \\
36.0 23.9643 \\
37.0 24.8487 \\
38.0 23.9295 \\
39.0 23.8897 \\
40.0 24.6958 \\
41.0 25.3846 \\
42.0 25.4832 \\
43.0 24.2851 \\
44.0 25.5781 \\
45.0 25.8743 \\
};
\addlegendentry{5 point \cite{DBLP:journals/pami/Nister04}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%






\addplot [color=cyan!50!black,line width=1.5pt, mark options={solid, orange}, mark options={solid, violet}, mark=*, mark repeat=11, mark size=1pt]
  table[row sep=crcr]{%
0.0 56.8391 \\
1.0 38.0821 \\
2.0 32.6522 \\
3.0 26.6904 \\
4.0 22.2943 \\
5.0 20.2198 \\
6.0 19.0072 \\
7.0 16.8383 \\
8.0 16.5342 \\
9.0 15.7747 \\
10.0 16.3949 \\
11.0 16.885 \\
12.0 18.4151 \\
13.0 16.9933 \\
14.0 16.7143 \\
15.0 17.9639 \\
16.0 18.3972 \\
17.0 19.1106 \\
18.0 19.6986 \\
19.0 19.9319 \\
20.0 19.8276 \\
21.0 20.1816 \\
22.0 21.7958 \\
23.0 21.242 \\
24.0 22.2559 \\
25.0 21.6069 \\
26.0 22.1164 \\
27.0 22.5811 \\
28.0 23.7551 \\
29.0 22.3673 \\
30.0 23.6601 \\
31.0 24.1246 \\
32.0 24.6729 \\
33.0 24.2066 \\
34.0 22.856 \\
35.0 24.5278 \\
36.0 24.45 \\
37.0 25.2875 \\
38.0 24.9506 \\
39.0 24.823 \\
40.0 25.615 \\
41.0 25.5712 \\
42.0 26.3188 \\
43.0 26.2687 \\
44.0 24.226 \\
45.0 26.2943 \\
  };
\addlegendentry{m=4,n=1,K=1+A1,HC}


\addplot [color=cyan,line width=1.5pt, mark options={solid, orange}, mark options={solid, violet}, mark=*, mark repeat=11, mark size=1pt]
  table[row sep=crcr]{%
0.0 28.5546 \\
1.0 14.7771 \\
2.0 12.288 \\
3.0 11.5566 \\
4.0 11.3186 \\
5.0 9.83856 \\
6.0 9.76867 \\
7.0 9.94043 \\
8.0 9.81682 \\
9.0 10.7906 \\
10.0 10.6205 \\
11.0 10.9981 \\
12.0 10.9098 \\
13.0 10.5901 \\
14.0 12.0031 \\
15.0 11.2328 \\
16.0 12.2959 \\
17.0 12.3342 \\
18.0 12.2547 \\
19.0 12.9326 \\
20.0 13.3689 \\
21.0 13.9997 \\
22.0 13.9016 \\
23.0 13.6185 \\
24.0 14.0898 \\
25.0 12.7663 \\
26.0 14.5684 \\
27.0 15.1138 \\
28.0 14.8448 \\
29.0 14.6004 \\
30.0 16.2864 \\
31.0 15.3337 \\
32.0 14.7923 \\
33.0 15.4015 \\
34.0 15.6629 \\
35.0 15.9882 \\
36.0 16.1436 \\
37.0 15.8018 \\
38.0 16.3041 \\
39.0 15.9235 \\
40.0 17.205 \\
41.0 15.9501 \\
42.0 16.4565 \\
43.0 17.477 \\
44.0 17.869 \\
45.0 17.0915 \\
};
\addlegendentry{m=4,n=1,K=1+A1,GB}


\addplot [color=cyan!50!black,line width=1.5pt, mark options={solid, orange}, mark options={solid, violet}, mark=triangle*, mark repeat=11, mark size=1pt]
  table[row sep=crcr]{%
0.0 17.6855 \\
1.0 12.9355 \\
2.0 10.7637 \\
3.0 8.82434 \\
4.0 8.15057 \\
5.0 7.70199 \\
6.0 7.8363 \\
7.0 8.77978 \\
8.0 9.39956 \\
9.0 10.7923 \\
10.0 10.7613 \\
11.0 11.6464 \\
12.0 12.9469 \\
13.0 12.3253 \\
14.0 13.4224 \\
15.0 14.9537 \\
16.0 14.9826 \\
17.0 15.4787 \\
18.0 17.0065 \\
19.0 17.9416 \\
20.0 16.4525 \\
21.0 17.9601 \\
22.0 17.6217 \\
23.0 17.6553 \\
24.0 17.4976 \\
25.0 17.6697 \\
26.0 18.5619 \\
27.0 18.8954 \\
28.0 18.3784 \\
29.0 19.0767 \\
30.0 19.2539 \\
31.0 18.4603 \\
32.0 18.5967 \\
33.0 18.8424 \\
34.0 18.8264 \\
35.0 18.4688 \\
36.0 18.4358 \\
37.0 19.1707 \\
38.0 18.1055 \\
39.0 18.8991 \\
40.0 18.0872 \\
41.0 18.6536 \\
42.0 18.039 \\
43.0 18.0986 \\
44.0 16.9187 \\
45.0 17.766 \\
  };
\addlegendentry{m=4,n=1,K=1+A2,HC}


\addplot [color=cyan,line width=1.5pt, mark options={solid, orange}, mark options={solid, violet}, mark=triangle*, mark repeat=11, mark size=1pt]
  table[row sep=crcr]{%
0.0 19.7475 \\
1.0 13.0639 \\
2.0 10.8772 \\
3.0 9.46208 \\
4.0 8.389 \\
5.0 7.68719 \\
6.0 8.61568 \\
7.0 8.54854 \\
8.0 9.23397 \\
9.0 9.95287 \\
10.0 10.4791 \\
11.0 12.1718 \\
12.0 12.0658 \\
13.0 13.3747 \\
14.0 14.0649 \\
15.0 14.6907 \\
16.0 15.2654 \\
17.0 15.4418 \\
18.0 15.6418 \\
19.0 16.287 \\
20.0 16.6939 \\
21.0 17.0399 \\
22.0 17.3363 \\
23.0 17.5726 \\
24.0 18.3788 \\
25.0 18.4083 \\
26.0 17.3804 \\
27.0 18.0871 \\
28.0 18.5348 \\
29.0 19.078 \\
30.0 19.4439 \\
31.0 17.1448 \\
32.0 17.8401 \\
33.0 18.4358 \\
34.0 18.373 \\
35.0 18.0642 \\
36.0 16.8276 \\
37.0 18.8694 \\
38.0 17.7207 \\
39.0 17.167 \\
40.0 18.2615 \\
41.0 17.8713 \\
42.0 17.0919 \\
43.0 17.4043 \\
44.0 16.7261 \\
45.0 18.4473 \\
  };
\addlegendentry{m=4,n=1,K=1+A2,GB}




\addplot [color=cyan!50!black,line width=1.5pt, mark options={solid, orange}, mark options={solid, black}, mark=*, mark repeat=11, mark size=1pt]
  table[row sep=crcr]{%
0.0 9.57877 \\
1.0 8.8041 \\
2.0 9.11313 \\
3.0 9.14505 \\
4.0 8.80527 \\
5.0 8.89178 \\
6.0 8.94761 \\
7.0 8.8717 \\
8.0 9.74035 \\
9.0 8.95123 \\
10.0 9.43711 \\
11.0 9.39401 \\
12.0 10.5003 \\
13.0 10.8759 \\
14.0 10.8105 \\
15.0 12.0987 \\
16.0 11.2427 \\
17.0 12.1718 \\
18.0 12.5637 \\
19.0 12.2636 \\
20.0 12.4788 \\
21.0 12.8394 \\
22.0 12.9896 \\
23.0 13.2162 \\
24.0 13.6148 \\
25.0 13.9533 \\
26.0 13.7248 \\
27.0 13.8082 \\
28.0 14.1449 \\
29.0 14.2774 \\
30.0 14.5169 \\
31.0 14.5942 \\
32.0 14.9137 \\
33.0 15.255 \\
34.0 15.7237 \\
35.0 14.8857 \\
36.0 15.3291 \\
37.0 16.375 \\
38.0 15.953 \\
39.0 15.5989 \\
40.0 16.1341 \\
41.0 15.033 \\
42.0 15.9837 \\
43.0 15.2882 \\
44.0 16.5626 \\
45.0 16.2507 \\
  };
\addlegendentry{m=4,n=1,K=2+A1,HC}

\addplot [color=cyan!50!black,line width=1.5pt, mark options={solid, orange}, mark options={solid, black}, mark=triangle*, mark repeat=11, mark phase=3, mark size=1pt]
  table[row sep=crcr]{%
0.0 5.62992 \\
1.0 5.23851 \\
2.0 5.73977 \\
3.0 6.24707 \\
4.0 6.16703 \\
5.0 6.57099 \\
6.0 6.61925 \\
7.0 6.79521 \\
8.0 7.20554 \\
9.0 6.56128 \\
10.0 7.12225 \\
11.0 7.54827 \\
12.0 7.96951 \\
13.0 8.79189 \\
14.0 8.54937 \\
15.0 8.72894 \\
16.0 8.79224 \\
17.0 9.69272 \\
18.0 9.41309 \\
19.0 10.1739 \\
20.0 10.0961 \\
21.0 10.3335 \\
22.0 10.8687 \\
23.0 11.3445 \\
24.0 11.5736 \\
25.0 11.473 \\
26.0 12.036 \\
27.0 11.6732 \\
28.0 12.1087 \\
29.0 12.2693 \\
30.0 12.849 \\
31.0 12.8417 \\
32.0 12.2173 \\
33.0 13.7295 \\
34.0 13.2346 \\
35.0 13.465 \\
36.0 13.3699 \\
37.0 13.6414 \\
38.0 14.0424 \\
39.0 13.8386 \\
40.0 14.6203 \\
41.0 15.0349 \\
42.0 14.6431 \\
43.0 14.7641 \\
44.0 14.9329 \\
45.0 15.6601 \\
  };
\addlegendentry{m=4,n=1,K=2+A2,HC}

\addplot [color=cyan,line width=1.5pt, mark options={solid, orange}, mark options={solid, yellow}, mark=triangle*, mark repeat=11, mark phase=7, mark size=1pt]
  table[row sep=crcr]{%
0.0 9.23617 \\
1.0 8.95577 \\
2.0 8.98701 \\
3.0 8.72722 \\
4.0 8.49641 \\
5.0 8.57502 \\
6.0 8.71076 \\
7.0 8.15013 \\
8.0 7.81917 \\
9.0 8.1612 \\
10.0 8.52589 \\
11.0 9.16307 \\
12.0 8.52626 \\
13.0 9.29752 \\
14.0 8.67424 \\
15.0 9.73097 \\
16.0 9.86984 \\
17.0 10.0726 \\
18.0 10.011 \\
19.0 10.4027 \\
20.0 10.8986 \\
21.0 10.5104 \\
22.0 10.7352 \\
23.0 11.3305 \\
24.0 11.7955 \\
25.0 11.5051 \\
26.0 11.5705 \\
27.0 11.6101 \\
28.0 12.4219 \\
29.0 12.3755 \\
30.0 12.2991 \\
31.0 12.4277 \\
32.0 12.02 \\
33.0 12.3961 \\
34.0 12.9013 \\
35.0 12.9844 \\
36.0 13.2036 \\
37.0 13.3361 \\
38.0 13.3908 \\
39.0 13.3905 \\
40.0 13.1304 \\
41.0 13.65 \\
42.0 13.8454 \\
43.0 14.1808 \\
44.0 14.3149 \\
45.0 14.3169 \\
  };
\addlegendentry{m=4,n=1,K=2+A2,GB}

\legend{}

\end{axis}

==> plot/noise_test_t.tex <==


\begin{axis}[%
width=0.35\columnwidth,
height=0.20\columnwidth,
at={(2.4in,0.389in)},
scale only axis,
xmin=0,
xmax=40,
xlabel style={font=\color{white!15!black}, yshift=0.03in},
xlabel={Ang. vel. ($^{\circ}$ / frame)},
title={Tran err ($^{\circ}$)},
ymin=0,
ymax=25,
ymode=normal,
yminorticks=true,
axis lines = left,
axis background/.style={fill=white},
title style={font=\bfseries, yshift=-0.1in},
%ylabel style={yshift=-0.15in},
%ylabel={Success rate ($\%$)},
%legend style={at={(1,1.3)}, anchor=south, legend cell align=left, align=left, draw=white!15!black, font=\normalsize,nodes={scale=1.0, transform shape}},
%legend columns=3
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addplot [color=magenta,line width=2pt, mark options={solid, red}]
  table[row sep=crcr]{%
0.0 5.46365 \\
1.0 5.59261 \\
2.0 5.82918 \\
3.0 5.87567 \\
4.0 7.00883 \\
5.0 7.74415 \\
6.0 7.68287 \\
7.0 8.63747 \\
8.0 9.29517 \\
9.0 9.50292 \\
10.0 9.78742 \\
11.0 10.9589 \\
12.0 10.9359 \\
13.0 11.5838 \\
14.0 12.4155 \\
15.0 12.5927 \\
16.0 13.5557 \\
17.0 14.5062 \\
18.0 14.8155 \\
19.0 13.5581 \\
20.0 14.9004 \\
21.0 15.0003 \\
22.0 16.0294 \\
23.0 16.0375 \\
24.0 16.3335 \\
25.0 16.5643 \\
26.0 16.6159 \\
27.0 17.6459 \\
28.0 17.2628 \\
29.0 17.7897 \\
30.0 17.6869 \\
31.0 19.1384 \\
32.0 18.617 \\
33.0 18.9231 \\
34.0 19.657 \\
35.0 19.5009 \\
36.0 20.3382 \\
37.0 20.3662 \\
38.0 20.5738 \\
39.0 19.9006 \\
40.0 20.3003 \\
41.0 21.0816 \\
42.0 21.3033 \\
43.0 21.0552 \\
44.0 21.8458 \\
45.0 21.3037 \\
};
\addlegendentry{5 point \cite{}}

\addplot [color=green!20!yellow,line width=2pt, mark options={solid, red}]
  table[row sep=crcr]{%
0.0 4.75967 \\
1.0 4.48746 \\
2.0 5.16458 \\
3.0 5.02304 \\
4.0 4.89903 \\
5.0 4.87093 \\
6.0 4.73377 \\
7.0 4.62409 \\
8.0 5.39827 \\
9.0 5.50234 \\
10.0 5.33382 \\
11.0 5.78023 \\
12.0 5.95655 \\
13.0 6.70416 \\
14.0 6.17423 \\
15.0 7.19735 \\
16.0 7.5096 \\
17.0 7.92453 \\
18.0 8.28772 \\
19.0 8.33106 \\
20.0 8.51601 \\
21.0 8.79294 \\
22.0 9.92955 \\
23.0 9.98337 \\
24.0 9.9161 \\
25.0 10.778 \\
26.0 11.2432 \\
27.0 10.9942 \\
28.0 11.7649 \\
29.0 11.3639 \\
30.0 12.9688 \\
31.0 12.5908 \\
32.0 12.2352 \\
33.0 13.6073 \\
34.0 13.06 \\
35.0 13.5343 \\
36.0 13.709 \\
37.0 14.5838 \\
38.0 14.0471 \\
39.0 14.1511 \\
40.0 14.8468 \\
41.0 14.7189 \\
42.0 14.8386 \\
43.0 15.0137 \\
44.0 14.8509 \\
45.0 15.3587 \\
};
\addlegendentry{m=2,n=5,K=1+A2,GB3}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addplot [color=green!50!black,line width=1.5pt, mark options={solid, violet!50!magenta}, mark=triangle*, mark repeat=11, mark phase=3, mark size=0.5pt]
  table[row sep=crcr]{%
0.0 4.47831 \\
1.0 5.19288 \\
2.0 4.66138 \\
3.0 4.73623 \\
4.0 4.37517 \\
5.0 4.92408 \\
6.0 4.83314 \\
7.0 4.963 \\
8.0 5.27228 \\
9.0 5.35453 \\
10.0 5.47667 \\
11.0 5.66193 \\
12.0 6.10498 \\
13.0 6.43116 \\
14.0 6.5967 \\
15.0 7.12981 \\
16.0 7.35621 \\
17.0 7.18223 \\
18.0 7.58689 \\
19.0 8.60284 \\
20.0 8.89958 \\
21.0 9.02006 \\
22.0 9.55155 \\
23.0 10.1719 \\
24.0 10.1641 \\
25.0 11.2277 \\
26.0 11.1221 \\
27.0 11.3164 \\
28.0 11.5613 \\
29.0 12.725 \\
30.0 12.5201 \\
31.0 12.9225 \\
32.0 13.3187 \\
33.0 12.9658 \\
34.0 13.2374 \\
35.0 13.7226 \\
36.0 14.3454 \\
37.0 14.0222 \\
38.0 14.6949 \\
39.0 14.5332 \\
40.0 14.2682 \\
41.0 14.3842 \\
42.0 14.7155 \\
43.0 15.5551 \\
44.0 15.8975 \\
45.0 15.3734 \\
};
\addlegendentry{m=2,n=5,K=1,A2,HC}


\addplot [color=green!90!black,line width=1.5pt, mark options={solid, violet}, mark=triangle*, mark repeat=11, mark phase=7, mark size=0.5pt]
  table[row sep=crcr]{%
0.0 4.63309 \\
1.0 4.82279 \\
2.0 4.54777 \\
3.0 4.77508 \\
4.0 5.18919 \\
5.0 4.383 \\
6.0 4.37206 \\
7.0 4.91078 \\
8.0 5.13627 \\
9.0 4.9737 \\
10.0 5.25764 \\
11.0 5.4107 \\
12.0 5.66279 \\
13.0 6.10444 \\
14.0 6.2541 \\
15.0 6.25697 \\
16.0 7.30177 \\
17.0 7.10322 \\
18.0 7.60052 \\
19.0 7.96899 \\
20.0 8.15708 \\
21.0 8.87552 \\
22.0 9.22131 \\
23.0 9.89154 \\
24.0 9.92678 \\
25.0 10.26 \\
26.0 11.0079 \\
27.0 11.3556 \\
28.0 11.5195 \\
29.0 12.4738 \\
30.0 12.7114 \\
31.0 12.0185 \\
32.0 12.6747 \\
33.0 12.9266 \\
34.0 13.2752 \\
35.0 13.6384 \\
36.0 14.3874 \\
37.0 14.5032 \\
38.0 15.178 \\
39.0 14.7955 \\
40.0 15.2208 \\
41.0 14.8965 \\
42.0 15.8788 \\
43.0 16.1829 \\
44.0 16.2864 \\
45.0 16.4697 \\
   }; 
\addlegendentry{m=2,n=5,K=1,A2,GB5}


%\addplot [color=green!20!yellow,line width=1.5pt, mark options={solid, orange}]
%  table[row sep=crcr]{%
%  1.3340502686000278e-20 0 \\
%   }; 
%\addlegendentry{m=2,n=5,K=1,A2,GB5}

\addplot [color=green!50!black,line width=1.5pt, mark options={solid, violet!50!magenta}, mark=*, mark repeat=11, mark size=1pt]
  table[row sep=crcr]{%
0.0 2.95077 \\
1.0 2.9793 \\
2.0 2.91474 \\
3.0 3.2306 \\
4.0 3.31353 \\
5.0 3.5883 \\
6.0 3.57829 \\
7.0 3.8033 \\
8.0 3.73719 \\
9.0 4.13053 \\
10.0 3.8861 \\
11.0 4.06685 \\
12.0 4.62239 \\
13.0 4.6657 \\
14.0 5.13302 \\
15.0 5.04563 \\
16.0 5.52181 \\
17.0 5.82993 \\
18.0 6.02297 \\
19.0 6.07749 \\
20.0 7.20076 \\
21.0 6.85328 \\
22.0 7.13825 \\
23.0 7.83133 \\
24.0 7.87835 \\
25.0 8.11541 \\
26.0 8.38038 \\
27.0 8.4632 \\
28.0 8.83526 \\
29.0 9.16823 \\
30.0 9.54578 \\
31.0 9.15547 \\
32.0 9.95211 \\
33.0 9.75175 \\
34.0 10.2302 \\
35.0 10.6166 \\
36.0 10.757 \\
37.0 10.9299 \\
38.0 11.5091 \\
39.0 11.7209 \\
40.0 12.0099 \\
41.0 11.8217 \\
42.0 11.8227 \\
43.0 12.6588 \\
44.0 12.3257 \\
45.0 12.2267 \\
   }; 
\addlegendentry{m=2,n=5,K=1,A1,HC}

\addplot [color=green!50!black,line width=1.5pt, mark options={solid,violet, draw=black,fill=violet}, mark=triangle*, mark repeat=11, mark size=0.4pt, mark phase=3]
  table[row sep=crcr]{%
0.0 3.91875 \\
1.0 3.86954 \\
2.0 3.89852 \\
3.0 3.37434 \\
4.0 3.68936 \\
5.0 3.66347 \\
6.0 3.99086 \\
7.0 3.74851 \\
8.0 3.77112 \\
9.0 3.97026 \\
10.0 3.66091 \\
11.0 4.10504 \\
12.0 3.92902 \\
13.0 4.09975 \\
14.0 4.30926 \\
15.0 3.85512 \\
16.0 4.18445 \\
17.0 4.08521 \\
18.0 4.30942 \\
19.0 4.3164 \\
20.0 4.9398 \\
21.0 4.62899 \\
22.0 4.61273 \\
23.0 5.03563 \\
24.0 5.23127 \\
25.0 5.27083 \\
26.0 5.42507 \\
27.0 5.42673 \\
28.0 5.90936 \\
29.0 5.80168 \\
30.0 6.24564 \\
31.0 5.98778 \\
32.0 6.04251 \\
33.0 6.86896 \\
34.0 7.05147 \\
35.0 6.70076 \\
36.0 7.3516 \\
37.0 6.78068 \\
38.0 7.26082 \\
39.0 7.38343 \\
40.0 7.7175 \\
41.0 7.7225 \\
42.0 7.9249 \\
43.0 8.15902 \\
44.0 8.15506 \\
45.0 8.84508 \\
   }; 
\addlegendentry{m=2,n=5,K=2,A2,HC}



\legend{}

\end{axis}

==> plot/noise_test_t_3v.tex <==


\begin{axis}[%
width=0.35\columnwidth,
height=0.20\columnwidth,
at={(2.4in,0.389in)},
scale only axis,
xmin=0,
xmax=40,
xlabel style={font=\color{white!15!black}, yshift=0.03in},
xlabel={Ang. vel. ($^{\circ}$ / frame)},
title={Tran err ($^{\circ}$)},
ymin=0,
ymax=25,
ymode=normal,
yminorticks=true,
axis lines = left,
axis background/.style={fill=white},
title style={font=\bfseries, yshift=-0.1in},
%ylabel style={yshift=-0.15in},
%ylabel={Success rate ($\%$)},
%legend style={at={(1,1.3)}, anchor=south, legend cell align=left, align=left, draw=white!15!black, font=\normalsize,nodes={scale=1.0, transform shape}},
%legend columns=3
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addplot [color=magenta,line width=2pt, mark options={solid, red}]
  table[row sep=crcr]{%
0.0 5.46365 \\
1.0 5.59261 \\
2.0 5.82918 \\
3.0 5.87567 \\
4.0 7.00883 \\
5.0 7.74415 \\
6.0 7.68287 \\
7.0 8.63747 \\
8.0 9.29517 \\
9.0 9.50292 \\
10.0 9.78742 \\
11.0 10.9589 \\
12.0 10.9359 \\
13.0 11.5838 \\
14.0 12.4155 \\
15.0 12.5927 \\
16.0 13.5557 \\
17.0 14.5062 \\
18.0 14.8155 \\
19.0 13.5581 \\
20.0 14.9004 \\
21.0 15.0003 \\
22.0 16.0294 \\
23.0 16.0375 \\
24.0 16.3335 \\
25.0 16.5643 \\
26.0 16.6159 \\
27.0 17.6459 \\
28.0 17.2628 \\
29.0 17.7897 \\
30.0 17.6869 \\
31.0 19.1384 \\
32.0 18.617 \\
33.0 18.9231 \\
34.0 19.657 \\
35.0 19.5009 \\
36.0 20.3382 \\
37.0 20.3662 \\
38.0 20.5738 \\
39.0 19.9006 \\
40.0 20.3003 \\
41.0 21.0816 \\
42.0 21.3033 \\
43.0 21.0552 \\
44.0 21.8458 \\
45.0 21.3037 \\
};
\addlegendentry{5 point \cite{}}



\addplot [color=orange!50!black,line width=1.5pt, mark options={solid, orange}, mark options={solid, cyan}, mark=*, mark repeat=11, mark phase=3, mark size=1pt]
  table[row sep=crcr]{%
0.0 5.83408 \\
1.0 5.57956 \\
2.0 5.80445 \\
3.0 5.42556 \\
4.0 6.01306 \\
5.0 6.3284 \\
6.0 6.05954 \\
7.0 6.91859 \\
8.0 7.93764 \\
9.0 7.49117 \\
10.0 8.37721 \\
11.0 8.73463 \\
12.0 10.0457 \\
13.0 10.3794 \\
14.0 11.4626 \\
15.0 11.9245 \\
16.0 12.037 \\
17.0 12.6512 \\
18.0 13.648 \\
19.0 13.3239 \\
20.0 14.1745 \\
21.0 14.4899 \\
22.0 14.6331 \\
23.0 15.2476 \\
24.0 15.3872 \\
25.0 15.9014 \\
26.0 16.7071 \\
27.0 15.8532 \\
28.0 15.9589 \\
29.0 16.4141 \\
30.0 16.9476 \\
31.0 16.638 \\
32.0 16.9775 \\
33.0 16.6611 \\
34.0 17.6768 \\
35.0 17.4102 \\
36.0 18.0809 \\
37.0 17.8217 \\
38.0 17.5841 \\
39.0 18.147 \\
40.0 18.6323 \\
41.0 18.634 \\
42.0 18.008 \\
43.0 18.0483 \\
44.0 18.1606 \\
45.0 18.5825 \\
  };
\addlegendentry{m=3,n=2,K=1+A1,HC}


\addplot [color=orange,line width=1.5pt, mark options={solid, orange}, mark options={solid, violet}, mark=*, mark repeat=11, mark phase=6, mark size=1pt]
  table[row sep=crcr]{%
0.0 5.63727 \\
1.0 5.48888 \\
2.0 5.32852 \\
3.0 5.85695 \\
4.0 6.56298 \\
5.0 6.18407 \\
6.0 6.04247 \\
7.0 7.09192 \\
8.0 7.40563 \\
9.0 8.44629 \\
10.0 8.29166 \\
11.0 8.92253 \\
12.0 9.59242 \\
13.0 10.3809 \\
14.0 11.1439 \\
15.0 11.4185 \\
16.0 12.5491 \\
17.0 12.7503 \\
18.0 13.6036 \\
19.0 13.5572 \\
20.0 14.0014 \\
21.0 14.0954 \\
22.0 15.0411 \\
23.0 15.3163 \\
24.0 15.077 \\
25.0 15.1705 \\
26.0 15.1941 \\
27.0 15.3742 \\
28.0 16.0295 \\
29.0 15.9605 \\
30.0 16.0483 \\
31.0 16.5659 \\
32.0 17.2475 \\
33.0 17.1957 \\
34.0 17.1422 \\
35.0 17.5632 \\
36.0 17.887 \\
37.0 17.931 \\
38.0 17.0538 \\
39.0 18.2122 \\
40.0 17.4055 \\
41.0 17.8295 \\
42.0 18.1036 \\
43.0 17.9034 \\
44.0 17.4249 \\
45.0 18.2057 \\
  };
\addlegendentry{m=3,n=2,K=1+A1,GB}


\addplot [color=orange!50!black,line width=1.5pt, mark options={solid, orange}, mark options={solid, cyan}, mark=triangle*, mark repeat=11, mark phase=9, mark size=1pt]
  table[row sep=crcr]{%
0.0 6.57099 \\
1.0 5.88827 \\
2.0 6.2312 \\
3.0 6.2706 \\
4.0 6.65713 \\
5.0 7.03098 \\
6.0 6.76043 \\
7.0 7.40046 \\
8.0 7.71723 \\
9.0 8.2227 \\
10.0 8.53032 \\
11.0 10.018 \\
12.0 10.3593 \\
13.0 10.4407 \\
14.0 12.0081 \\
15.0 11.6343 \\
16.0 13.4552 \\
17.0 12.7549 \\
18.0 13.649 \\
19.0 14.6438 \\
20.0 14.4418 \\
21.0 14.5889 \\
22.0 15.5646 \\
23.0 15.0573 \\
24.0 16.0442 \\
25.0 16.3824 \\
26.0 16.213 \\
27.0 16.6416 \\
28.0 17.1538 \\
29.0 16.7935 \\
30.0 16.816 \\
31.0 17.0842 \\
32.0 17.5122 \\
33.0 17.36 \\
34.0 17.476 \\
35.0 17.6404 \\
36.0 18.367 \\
37.0 17.6249 \\
38.0 17.5995 \\
39.0 17.9845 \\
40.0 18.2376 \\
41.0 17.4871 \\
42.0 17.5794 \\
43.0 17.6543 \\
44.0 17.3359 \\
45.0 18.129 \\
  };
\addlegendentry{m=3,n=2,K=1+A2,HC}


\addplot [color=orange,line width=1.5pt, mark options={solid, orange}, mark options={solid, violet}, mark=triangle*, mark repeat=11, mark size=1pt]
  table[row sep=crcr]{%
0.0 7.16115 \\
1.0 6.25556 \\
2.0 5.98725 \\
3.0 6.34369 \\
4.0 5.43488 \\
5.0 5.86969 \\
6.0 6.34466 \\
7.0 6.23331 \\
8.0 6.54451 \\
9.0 6.8305 \\
10.0 7.52081 \\
11.0 7.69074 \\
12.0 7.39267 \\
13.0 8.52709 \\
14.0 8.30125 \\
15.0 8.45401 \\
16.0 9.58798 \\
17.0 9.52764 \\
18.0 9.3796 \\
19.0 10.1724 \\
20.0 9.80605 \\
21.0 10.7698 \\
22.0 11.193 \\
23.0 11.1923 \\
24.0 11.6474 \\
25.0 12.0324 \\
26.0 11.9522 \\
27.0 12.2129 \\
28.0 13.0689 \\
29.0 12.1355 \\
30.0 13.081 \\
31.0 13.1198 \\
32.0 13.9125 \\
33.0 13.4261 \\
34.0 13.9552 \\
35.0 14.6507 \\
36.0 14.498 \\
37.0 14.4509 \\
38.0 14.4924 \\
39.0 14.7911 \\
40.0 15.0351 \\
41.0 14.3109 \\
42.0 15.4483 \\
43.0 15.6034 \\
44.0 15.2384 \\
45.0 15.6051 \\
  };
\addlegendentry{m=3,n=2,K=1+A2,GB}




\addplot [color=orange!50!black,line width=1.5pt, mark options={solid, orange}, mark options={solid, black}, mark=*, mark repeat=11, mark phase = 5, mark size=1pt]
  table[row sep=crcr]{%
0.0 4.58135 \\
1.0 4.20066 \\
2.0 4.42715 \\
3.0 4.5794 \\
4.0 4.20181 \\
5.0 4.67749 \\
6.0 4.10066 \\
7.0 4.73638 \\
8.0 4.77006 \\
9.0 4.66423 \\
10.0 4.73019 \\
11.0 5.07508 \\
12.0 5.28184 \\
13.0 5.20416 \\
14.0 5.72202 \\
15.0 6.0416 \\
16.0 5.99894 \\
17.0 6.44257 \\
18.0 6.62133 \\
19.0 6.72724 \\
20.0 6.54876 \\
21.0 7.09144 \\
22.0 7.47873 \\
23.0 8.03396 \\
24.0 7.65244 \\
25.0 8.03791 \\
26.0 8.20515 \\
27.0 8.40474 \\
28.0 8.20354 \\
29.0 8.79431 \\
30.0 8.87033 \\
31.0 8.92264 \\
32.0 9.39805 \\
33.0 9.11826 \\
34.0 9.37144 \\
35.0 9.73153 \\
36.0 9.68764 \\
37.0 9.60674 \\
38.0 9.98011 \\
39.0 10.3321 \\
40.0 10.4412 \\
41.0 10.8792 \\
42.0 10.6785 \\
43.0 11.0045 \\
44.0 10.7506 \\
45.0 11.0518 \\
  };
\addlegendentry{m=3,n=2,K=2+A1,HC}

\addplot [color=orange!50!black,line width=1.5pt, mark options={solid, orange}, mark options={solid, black}, mark=triangle*, mark repeat=11, mark size=1pt]
  table[row sep=crcr]{%
0.0 3.40215 \\
1.0 3.69342 \\
2.0 3.69576 \\
3.0 3.64491 \\
4.0 3.93712 \\
5.0 3.84557 \\
6.0 3.63894 \\
7.0 4.56033 \\
8.0 4.24262 \\
9.0 4.32549 \\
10.0 4.35417 \\
11.0 4.74017 \\
12.0 4.85892 \\
13.0 4.94137 \\
14.0 5.02743 \\
15.0 5.66437 \\
16.0 6.147 \\
17.0 6.15364 \\
18.0 6.19985 \\
19.0 6.19124 \\
20.0 7.02382 \\
21.0 6.37582 \\
22.0 7.33205 \\
23.0 7.56408 \\
24.0 7.22187 \\
25.0 7.7932 \\
26.0 8.04882 \\
27.0 8.64796 \\
28.0 8.37653 \\
29.0 8.39023 \\
30.0 8.52737 \\
31.0 8.89498 \\
32.0 8.93426 \\
33.0 9.52732 \\
34.0 9.58636 \\
35.0 9.3617 \\
36.0 9.5647 \\
37.0 9.98448 \\
38.0 9.90761 \\
39.0 9.7325 \\
40.0 10.4562 \\
41.0 10.1692 \\
42.0 10.5886 \\
43.0 10.703 \\
44.0 10.7798 \\
45.0 10.8349 \\
  };
\addlegendentry{m=3,n=2,K=2+A2,GB}






\legend{}

\end{axis}

==> plot/noise_test_t_4v.tex <==


\begin{axis}[%
width=0.35\columnwidth,
height=0.20\columnwidth,
at={(2.4in,0.389in)},
scale only axis,
xmin=0,
xmax=40,
xlabel style={font=\color{white!15!black}, yshift=0.03in},
xlabel={Ang. vel. ($^{\circ}$ / frame)},
title={Tran err ($^{\circ}$)},
ymin=0,
ymax=25,
ymode=normal,
yminorticks=true,
axis lines = left,
axis background/.style={fill=white},
title style={font=\bfseries, yshift=-0.1in},
%ylabel style={yshift=-0.15in},
%ylabel={Success rate ($\%$)},
%legend style={at={(1,1.3)}, anchor=south, legend cell align=left, align=left, draw=white!15!black, font=\normalsize,nodes={scale=1.0, transform shape}},
%legend columns=3
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\addplot [color=magenta,line width=2pt, mark options={solid, red}]
  table[row sep=crcr]{%
0.0 5.46365 \\
1.0 5.59261 \\
2.0 5.82918 \\
3.0 5.87567 \\
4.0 7.00883 \\
5.0 7.74415 \\
6.0 7.68287 \\
7.0 8.63747 \\
8.0 9.29517 \\
9.0 9.50292 \\
10.0 9.78742 \\
11.0 10.9589 \\
12.0 10.9359 \\
13.0 11.5838 \\
14.0 12.4155 \\
15.0 12.5927 \\
16.0 13.5557 \\
17.0 14.5062 \\
18.0 14.8155 \\
19.0 13.5581 \\
20.0 14.9004 \\
21.0 15.0003 \\
22.0 16.0294 \\
23.0 16.0375 \\
24.0 16.3335 \\
25.0 16.5643 \\
26.0 16.6159 \\
27.0 17.6459 \\
28.0 17.2628 \\
29.0 17.7897 \\
30.0 17.6869 \\
31.0 19.1384 \\
32.0 18.617 \\
33.0 18.9231 \\
34.0 19.657 \\
35.0 19.5009 \\
36.0 20.3382 \\
37.0 20.3662 \\
38.0 20.5738 \\
39.0 19.9006 \\
40.0 20.3003 \\
41.0 21.0816 \\
42.0 21.3033 \\
43.0 21.0552 \\
44.0 21.8458 \\
45.0 21.3037 \\
};
\addlegendentry{5 point \cite{}}


\addplot [color=cyan!40!black,line width=1.5pt, mark options={solid, orange}, mark options={solid, violet}, mark=*, mark repeat=11, mark size=1pt]
  table[row sep=crcr]{%
0.0 55.1899 \\
1.0 30.834 \\
2.0 24.8525 \\
3.0 19.6672 \\
4.0 18.2319 \\
5.0 16.6675 \\
6.0 16.8317 \\
7.0 15.6726 \\
8.0 14.8146 \\
9.0 15.5533 \\
10.0 15.4045 \\
11.0 16.1314 \\
12.0 16.2602 \\
13.0 16.9352 \\
14.0 15.9929 \\
15.0 16.5232 \\
16.0 17.724 \\
17.0 17.3171 \\
18.0 16.8757 \\
19.0 17.8237 \\
20.0 17.4626 \\
21.0 17.8829 \\
22.0 18.2233 \\
23.0 19.6604 \\
24.0 18.4492 \\
25.0 18.9956 \\
26.0 20.3031 \\
27.0 19.5194 \\
28.0 19.4287 \\
29.0 19.4826 \\
30.0 19.7354 \\
31.0 20.6918 \\
32.0 21.8383 \\
33.0 22.4697 \\
34.0 20.6505 \\
35.0 20.6609 \\
36.0 21.1978 \\
37.0 22.3763 \\
38.0 20.3035 \\
39.0 22.4841 \\
40.0 20.9747 \\
41.0 22.318 \\
42.0 23.6927 \\
43.0 22.7708 \\
44.0 22.933 \\
45.0 23.2297 \\
  };
\addlegendentry{m=4,n=1,K=1+A1,HC}


\addplot [color=cyan,line width=1.5pt, mark options={solid, orange}, mark options={solid, violet!50!magenta}, mark=*, mark repeat=11, mark phase=3, mark size=1pt]
  table[row sep=crcr]{%
0.0 28.5546 \\
1.0 14.7771 \\
2.0 12.288 \\
3.0 11.5566 \\
4.0 11.3186 \\
5.0 9.83856 \\
6.0 9.76867 \\
7.0 9.94043 \\
8.0 9.81682 \\
9.0 10.7906 \\
10.0 10.6205 \\
11.0 10.9981 \\
12.0 10.9098 \\
13.0 10.5901 \\
14.0 12.0031 \\
15.0 11.2328 \\
16.0 12.2959 \\
17.0 12.3342 \\
18.0 12.2547 \\
19.0 12.9326 \\
20.0 13.3689 \\
21.0 13.9997 \\
22.0 13.9016 \\
23.0 13.6185 \\
24.0 14.0898 \\
25.0 12.7663 \\
26.0 14.5684 \\
27.0 15.1138 \\
28.0 14.8448 \\
29.0 14.6004 \\
30.0 16.2864 \\
31.0 15.3337 \\
32.0 14.7923 \\
33.0 15.4015 \\
34.0 15.6629 \\
35.0 15.9882 \\
36.0 16.1436 \\
37.0 15.8018 \\
38.0 16.3041 \\
39.0 15.9235 \\
40.0 17.205 \\
41.0 15.9501 \\
42.0 16.4565 \\
43.0 17.477 \\
44.0 17.869 \\
45.0 17.0915 \\
};
\addlegendentry{m=4,n=1,K=1+A1,GB}


\addplot [color=cyan!40!black,line width=1.5pt, mark options={solid, orange}, mark options={solid, violet}, mark=triangle*, mark repeat=11, mark phase=6, mark size=1pt]
  table[row sep=crcr]{%
0.0 18.5749 \\
1.0 11.3181 \\
2.0 9.84484 \\
3.0 9.06886 \\
4.0 8.38928 \\
5.0 8.16445 \\
6.0 8.1389 \\
7.0 8.02536 \\
8.0 8.49682 \\
9.0 8.66201 \\
10.0 10.1556 \\
11.0 10.3478 \\
12.0 10.9388 \\
13.0 12.3805 \\
14.0 11.0739 \\
15.0 12.3211 \\
16.0 14.0132 \\
17.0 14.9855 \\
18.0 14.824 \\
19.0 15.7728 \\
20.0 15.7955 \\
21.0 16.3116 \\
22.0 18.0261 \\
23.0 17.3661 \\
24.0 17.2453 \\
25.0 18.2856 \\
26.0 18.601 \\
27.0 18.6148 \\
28.0 19.3724 \\
29.0 19.621 \\
30.0 20.0778 \\
31.0 20.4051 \\
32.0 19.6654 \\
33.0 20.2138 \\
34.0 20.0003 \\
35.0 19.4311 \\
36.0 20.751 \\
37.0 19.9846 \\
38.0 19.9506 \\
39.0 20.0595 \\
40.0 20.7679 \\
41.0 20.8841 \\
42.0 21.058 \\
43.0 20.7783 \\
44.0 20.2405 \\
45.0 19.6514 \\
  };
\addlegendentry{m=4,n=1,K=1+A2,HC}


\addplot [color=cyan,line width=1.5pt, mark options={solid, orange}, mark options={solid, violet!50!magenta}, mark=triangle*, mark repeat=11, mark phase=9, mark size=1pt]
  table[row sep=crcr]{%
0.0 21.5172 \\
1.0 13.7116 \\
2.0 10.7998 \\
3.0 9.10993 \\
4.0 9.3685 \\
5.0 8.64493 \\
6.0 8.83774 \\
7.0 8.82765 \\
8.0 8.92217 \\
9.0 9.44975 \\
10.0 9.8913 \\
11.0 10.1386 \\
12.0 11.82 \\
13.0 11.974 \\
14.0 13.3526 \\
15.0 13.3018 \\
16.0 13.6836 \\
17.0 14.7174 \\
18.0 15.0251 \\
19.0 15.7351 \\
20.0 16.3517 \\
21.0 16.8821 \\
22.0 16.6332 \\
23.0 17.336 \\
24.0 16.8981 \\
25.0 18.5614 \\
26.0 18.0001 \\
27.0 18.1105 \\
28.0 18.7414 \\
29.0 18.9703 \\
30.0 19.8993 \\
31.0 19.7672 \\
32.0 20.5077 \\
33.0 20.6122 \\
34.0 20.6635 \\
35.0 20.2928 \\
36.0 19.8353 \\
37.0 20.295 \\
38.0 20.2808 \\
39.0 21.3202 \\
40.0 21.6453 \\
41.0 20.5926 \\
42.0 20.4913 \\
43.0 19.9498 \\
44.0 19.8673 \\
45.0 20.5858 \\
  };
\addlegendentry{m=4,n=1,K=1+A2,GB}




\addplot [color=cyan!40!black,line width=1.5pt, mark options={solid, orange}, mark options={solid, black}, mark=*, mark repeat=11, mark size=1pt]
  table[row sep=crcr]{%
0.0 8.60341 \\
1.0 8.63893 \\
2.0 8.12839 \\
3.0 7.62863 \\
4.0 7.90682 \\
5.0 7.69324 \\
6.0 7.49117 \\
7.0 7.96245 \\
8.0 7.70975 \\
9.0 8.3218 \\
10.0 8.1948 \\
11.0 8.43768 \\
12.0 8.58897 \\
13.0 8.45337 \\
14.0 9.05232 \\
15.0 9.27783 \\
16.0 9.69355 \\
17.0 10.1844 \\
18.0 10.221 \\
19.0 9.93735 \\
20.0 10.4102 \\
21.0 9.91413 \\
22.0 10.7629 \\
23.0 10.9899 \\
24.0 11.4558 \\
25.0 11.3912 \\
26.0 11.1946 \\
27.0 11.7446 \\
28.0 11.9972 \\
29.0 12.3332 \\
30.0 12.3245 \\
31.0 12.4529 \\
32.0 12.7606 \\
33.0 13.1925 \\
34.0 12.7225 \\
35.0 13.3789 \\
36.0 12.9132 \\
37.0 13.5243 \\
38.0 13.6682 \\
39.0 14.0029 \\
40.0 13.8307 \\
41.0 13.2025 \\
42.0 14.2515 \\
43.0 14.4276 \\
44.0 14.2228 \\
45.0 14.7391 \\
  };
\addlegendentry{m=4,n=1,K=2+A1,HC}

\addplot [color=cyan!40!black,line width=1.5pt, mark options={solid, orange}, mark options={solid, black}, mark=triangle*, mark repeat=11, mark phase=7, mark size=1pt]
  table[row sep=crcr]{%
0.0 6.53629 \\
1.0 6.15395 \\
2.0 5.77655 \\
3.0 5.73516 \\
4.0 5.89959 \\
5.0 6.33647 \\
6.0 6.67475 \\
7.0 6.26627 \\
8.0 6.33178 \\
9.0 6.69438 \\
10.0 7.2849 \\
11.0 7.33753 \\
12.0 7.93399 \\
13.0 7.84917 \\
14.0 8.34089 \\
15.0 8.43724 \\
16.0 8.86788 \\
17.0 9.03389 \\
18.0 9.20385 \\
19.0 9.11464 \\
20.0 9.42771 \\
21.0 10.1012 \\
22.0 10.0725 \\
23.0 10.169 \\
24.0 10.3814 \\
25.0 10.6821 \\
26.0 10.6257 \\
27.0 10.8538 \\
28.0 10.9056 \\
29.0 11.1789 \\
30.0 11.4745 \\
31.0 11.5519 \\
32.0 11.9212 \\
33.0 11.6907 \\
34.0 11.6298 \\
35.0 12.682 \\
36.0 12.4689 \\
37.0 12.5856 \\
38.0 12.3987 \\
39.0 13.327 \\
40.0 12.9965 \\
41.0 12.9567 \\
42.0 12.6263 \\
43.0 13.6657 \\
44.0 13.1194 \\
45.0 13.5028 \\
  };
\addlegendentry{m=4,n=1,K=2+A2,HC}

\addplot [color=cyan,line width=1.5pt, mark options={solid, orange}, mark options={solid, yellow}, mark=triangle*, mark repeat=11, mark phase=3, mark size=1pt]
  table[row sep=crcr]{%
0.0 9.05904 \\
1.0 9.40843 \\
2.0 8.83316 \\
3.0 8.86148 \\
4.0 8.50671 \\
5.0 8.64557 \\
6.0 8.35134 \\
7.0 8.19087 \\
8.0 8.15663 \\
9.0 8.29164 \\
10.0 8.79448 \\
11.0 8.64131 \\
12.0 9.08791 \\
13.0 9.10114 \\
14.0 8.72582 \\
15.0 9.66263 \\
16.0 9.28196 \\
17.0 9.71171 \\
18.0 10.0116 \\
19.0 9.60112 \\
20.0 9.61699 \\
21.0 10.1127 \\
22.0 10.6007 \\
23.0 10.3676 \\
24.0 10.5093 \\
25.0 10.6473 \\
26.0 11.089 \\
27.0 10.8629 \\
28.0 11.3059 \\
29.0 11.5894 \\
30.0 12.1024 \\
31.0 11.4664 \\
32.0 12.026 \\
33.0 12.1607 \\
34.0 12.2353 \\
35.0 12.4431 \\
36.0 12.3319 \\
37.0 12.0838 \\
38.0 12.7356 \\
39.0 11.7947 \\
40.0 12.2696 \\
41.0 12.337 \\
42.0 12.4054 \\
43.0 12.9285 \\
44.0 13.1917 \\
45.0 12.9751 \\
  };
\addlegendentry{m=4,n=1,K=2+A2,GB}

\legend{}

\end{axis}

==> plot/rotation_stability.tex <==
\begin{axis}[%
xmode=log,
width=0.35\columnwidth,
height=0.22\columnwidth,
at={(0in,0.389in)},
scale only axis,
xmin=1e-18,
xmax=1e+2,
xlabel style={font=\color{white!15!black},yshift=0.05in},
xlabel={rotation error (rad)},
label style={font=\small},
title={Rotation stability},
ymin=0,
ymax=1000,
ymode=normal,
yminorticks=true,
axis lines = left,
axis background/.style={fill=white},
title style={font=\bfseries, yshift=0.03in},
ylabel style={yshift=-0.10in},
ylabel={Frequency},
grid=both,
legend style={at={(1.1,1.4)}, anchor=south, legend cell align=left, align=left, draw=white!15!black, font=\footnotesize,nodes={scale=1.0, transform shape}},
legend columns=3,
scaled y ticks=base 10:-3,
yticklabel style={/pgf/number format/fixed}
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addplot [color=green!50!black,line width=1.5pt, mark options={solid, violet!50!magenta}, mark=triangle*, mark repeat=11, mark phase=3, mark size=0.5pt]
  table[row sep=crcr]{%
1.334050268600027769e-20 0.000000000000000000e+00 \\
2.225329969703585113e-20 0.000000000000000000e+00 \\
3.712074117909952463e-20 0.000000000000000000e+00 \\
6.192112830212035034e-20 0.000000000000000000e+00 \\
1.032906673848005283e-19 0.000000000000000000e+00 \\
1.722992177523380382e-19 0.000000000000000000e+00 \\
2.874124176918259319e-19 0.000000000000000000e+00 \\
4.794328083497031032e-19 0.000000000000000000e+00 \\
7.997421251594711528e-19 0.000000000000000000e+00 \\
1.334050268600027926e-18 0.000000000000000000e+00 \\
2.225329969703585089e-18 0.000000000000000000e+00 \\
3.712074117909952560e-18 0.000000000000000000e+00 \\
6.192112830212034649e-18 0.000000000000000000e+00 \\
1.032906673848005355e-17 0.000000000000000000e+00 \\
1.722992177523380305e-17 0.000000000000000000e+00 \\
2.874124176918259049e-17 0.000000000000000000e+00 \\
4.794328083497030300e-17 3.000000000000000000e+00 \\
7.997421251594709602e-17 4.000000000000000000e+00 \\
1.334050268600027833e-16 1.100000000000000000e+01 \\
2.225329969703590759e-16 3.400000000000000000e+01 \\
3.712074117909949355e-16 7.800000000000000000e+01 \\
6.192112830212025928e-16 1.370000000000000000e+02 \\
1.032906673848005379e-15 1.810000000000000000e+02 \\
1.722992177523380280e-15 2.200000000000000000e+02 \\
2.874124176918252048e-15 2.230000000000000000e+02 \\
4.794328083497023053e-15 2.730000000000000000e+02 \\
7.997421251594710194e-15 2.590000000000000000e+02 \\
1.334050268600027883e-14 2.960000000000000000e+02 \\
2.225329969703585099e-14 2.610000000000000000e+02 \\
3.712074117909943596e-14 2.580000000000000000e+02 \\
6.192112830212024824e-14 2.810000000000000000e+02 \\
1.032906673848005253e-13 2.480000000000000000e+02 \\
1.722992177523380249e-13 2.520000000000000000e+02 \\
2.874124176918251795e-13 2.380000000000000000e+02 \\
4.794328083497023747e-13 2.710000000000000000e+02 \\
7.997421251594709689e-13 2.690000000000000000e+02 \\
1.334050268600027782e-12 2.880000000000000000e+02 \\
2.225329969703590564e-12 2.880000000000000000e+02 \\
3.712074117909949327e-12 3.020000000000000000e+02 \\
6.192112830212025429e-12 2.900000000000000000e+02 \\
1.032906673848005339e-11 3.090000000000000000e+02 \\
1.722992177523380047e-11 3.180000000000000000e+02 \\
2.874124176918251573e-11 3.080000000000000000e+02 \\
4.794328083497010580e-11 3.790000000000000000e+02 \\
7.997421251594699026e-11 3.330000000000000000e+02 \\
1.334050268600027960e-10 3.920000000000000000e+02 \\
2.225329969703590920e-10 3.530000000000000000e+02 \\
3.712074117909949650e-10 3.970000000000000000e+02 \\
6.192112830212009726e-10 4.040000000000000000e+02 \\
1.032906673848003633e-09 3.830000000000000000e+02 \\
1.722992177523380150e-09 3.370000000000000000e+02 \\
2.874124176918251780e-09 2.900000000000000000e+02 \\
4.794328083497010735e-09 2.630000000000000000e+02 \\
7.997421251594698199e-09 1.910000000000000000e+02 \\
1.334050268600027794e-08 9.900000000000000000e+01 \\
2.225329969703584995e-08 9.000000000000000000e+01 \\
3.712074117909943777e-08 5.200000000000000000e+01 \\
6.192112830212008568e-08 3.800000000000000000e+01 \\
1.032906673848003625e-07 2.100000000000000000e+01 \\
1.722992177523380448e-07 1.400000000000000000e+01 \\
2.874124176918251548e-07 9.000000000000000000e+00 \\
4.794328083497010669e-07 3.000000000000000000e+00 \\
7.997421251594698001e-07 4.000000000000000000e+00 \\
1.334050268600027847e-06 6.000000000000000000e+00 \\
2.225329969703585246e-06 1.000000000000000000e+00 \\
3.712074117909943380e-06 1.000000000000000000e+00 \\
6.192112830212009521e-06 0.000000000000000000e+00 \\
1.032906673848003662e-05 0.000000000000000000e+00 \\
1.722992177523380300e-05 1.000000000000000000e+00 \\
2.874124176918251570e-05 0.000000000000000000e+00 \\
4.794328083497011135e-05 0.000000000000000000e+00 \\
7.997421251594698255e-05 0.000000000000000000e+00 \\
1.334050268600027889e-04 0.000000000000000000e+00 \\
2.225329969703584857e-04 0.000000000000000000e+00 \\
3.712074117909933656e-04 0.000000000000000000e+00 \\
6.192112830212015721e-04 0.000000000000000000e+00 \\
1.032906673848005275e-03 0.000000000000000000e+00 \\
1.722992177523380124e-03 0.000000000000000000e+00 \\
2.874124176918244414e-03 1.000000000000000000e+00 \\
4.794328083497016203e-03 0.000000000000000000e+00 \\
7.997421251594711428e-03 0.000000000000000000e+00 \\
1.334050268600027803e-02 0.000000000000000000e+00 \\
2.225329969703584987e-02 1.000000000000000000e+00 \\
3.712074117909934523e-02 1.000000000000000000e+00 \\
6.192112830212015417e-02 1.000000000000000000e+00 \\
1.032906673848005275e-01 4.000000000000000000e+00 \\
1.722992177523380297e-01 3.000000000000000000e+00 \\
2.874124176918244622e-01 4.000000000000000000e+00 \\
4.794328083496991466e-01 1.200000000000000000e+01 \\
7.997421251594685199e-01 2.000000000000000000e+00 \\
1.334050268600027955e+00 8.000000000000000000e+00 \\
2.225329969703584876e+00 2.000000000000000000e+00 \\
3.712074117909933690e+00 0.000000000000000000e+00 \\
6.192112830212015417e+00 0.000000000000000000e+00 \\
1.032906673848005141e+01 0.000000000000000000e+00 \\
1.722992177523380164e+01 0.000000000000000000e+00 \\
2.874124176918244444e+01 0.000000000000000000e+00 \\
4.794328083496991155e+01 0.000000000000000000e+00 \\
7.997421251594685998e+01 0.000000000000000000e+00 \\
};
\addlegendentry{K1,A2,HC}


\addplot [color=green!90!black,line width=1.5pt, mark options={solid, violet}, mark=triangle*, mark repeat=9, mark phase = 5, mark size=1pt]
  table[row sep=crcr]{%
1.3340502686000278e-20 0 \\
2.225329969703585e-20 0 \\
3.7120741179099525e-20 0 \\
6.192112830212035e-20 0 \\
1.0329066738480053e-19 0 \\
1.7229921775233804e-19 0 \\
2.8741241769182593e-19 0 \\
4.794328083497031e-19 0 \\
7.997421251594712e-19 0 \\
1.334050268600028e-18 0 \\
2.225329969703585e-18 0 \\
3.7120741179099526e-18 0 \\
6.192112830212035e-18 0 \\
1.0329066738480054e-17 0 \\
1.7229921775233803e-17 0 \\
2.874124176918259e-17 0 \\
4.79432808349703e-17 0 \\
7.99742125159471e-17 0 \\
1.3340502686000278e-16 0 \\
2.225329969703591e-16 0 \\
3.7120741179099494e-16 0 \\
6.192112830212026e-16 1 \\
1.0329066738480054e-15 0 \\
1.7229921775233803e-15 1 \\
2.874124176918252e-15 9 \\
4.794328083497023e-15 11 \\
7.99742125159471e-15 35 \\
1.3340502686000279e-14 27 \\
2.225329969703585e-14 76 \\
3.7120741179099436e-14 86 \\
6.192112830212025e-14 135 \\
1.0329066738480053e-13 172 \\
1.7229921775233802e-13 211 \\
2.874124176918252e-13 279 \\
4.794328083497024e-13 339 \\
7.99742125159471e-13 387 \\
1.3340502686000278e-12 391 \\
2.2253299697035906e-12 441 \\
3.712074117909949e-12 448 \\
6.1921128302120254e-12 459 \\
1.0329066738480053e-11 475 \\
1.72299217752338e-11 443 \\
2.8741241769182516e-11 486 \\
4.7943280834970106e-11 406 \\
7.997421251594699e-11 425 \\
1.334050268600028e-10 461 \\
2.225329969703591e-10 376 \\
3.7120741179099496e-10 388 \\
6.19211283021201e-10 349 \\
1.0329066738480036e-09 290 \\
1.7229921775233802e-09 263 \\
2.8741241769182518e-09 237 \\
4.794328083497011e-09 228 \\
7.997421251594698e-09 211 \\
1.3340502686000278e-08 181 \\
2.225329969703585e-08 166 \\
3.712074117909944e-08 133 \\
6.192112830212009e-08 118 \\
1.0329066738480036e-07 116 \\
1.7229921775233804e-07 110 \\
2.8741241769182515e-07 96 \\
4.794328083497011e-07 68 \\
7.997421251594698e-07 68 \\
1.3340502686000278e-06 68 \\
2.2253299697035852e-06 36 \\
3.7120741179099434e-06 42 \\
6.1921128302120095e-06 42 \\
1.0329066738480037e-05 29 \\
1.7229921775233803e-05 26 \\
2.8741241769182516e-05 23 \\
4.794328083497011e-05 19 \\
7.997421251594698e-05 15 \\
0.0001334050268600028 14 \\
0.00022253299697035849 11 \\
0.00037120741179099337 11 \\
0.0006192112830212016 7 \\
0.0010329066738480053 7 \\
0.0017229921775233801 9 \\
0.0028741241769182444 8 \\
0.004794328083497016 5 \\
0.007997421251594711 4 \\
0.013340502686000278 2 \\
0.02225329969703585 2 \\
0.037120741179099345 2 \\
0.061921128302120154 2 \\
0.10329066738480053 3 \\
0.17229921775233803 8 \\
0.28741241769182446 2 \\
0.47943280834969915 1 \\
0.7997421251594685 0 \\
1.334050268600028 0 \\
2.225329969703585 0 \\
3.7120741179099337 0 \\
6.192112830212015 0 \\
10.329066738480051 0 \\
17.2299217752338 0 \\
28.741241769182444 0 \\
47.94328083496991 0 \\
79.97421251594686 0 \\
  };
\addlegendentry{K1,A2,GB5}


\addplot [color=green!20!yellow,line width=1.5pt, mark options={solid, orange}]
  table[row sep=crcr]{%
  1.3340502686000278e-20 0 \\
2.225329969703585e-20 0 \\
3.7120741179099525e-20 0 \\
6.192112830212035e-20 0 \\
1.0329066738480053e-19 0 \\
1.7229921775233804e-19 0 \\
2.8741241769182593e-19 0 \\
4.794328083497031e-19 0 \\
7.997421251594712e-19 0 \\
1.334050268600028e-18 0 \\
2.225329969703585e-18 0 \\
3.7120741179099526e-18 0 \\
6.192112830212035e-18 0 \\
1.0329066738480054e-17 0 \\
1.7229921775233803e-17 0 \\
2.874124176918259e-17 0 \\
4.79432808349703e-17 0 \\
7.99742125159471e-17 0 \\
1.3340502686000278e-16 0 \\
2.225329969703591e-16 0 \\
3.7120741179099494e-16 3 \\
6.192112830212026e-16 6 \\
1.0329066738480054e-15 37 \\
1.7229921775233803e-15 81 \\
2.874124176918252e-15 198 \\
4.794328083497023e-15 349 \\
7.99742125159471e-15 498 \\
1.3340502686000279e-14 606 \\
2.225329969703585e-14 740 \\
3.7120741179099436e-14 837 \\
6.192112830212025e-14 870 \\
1.0329066738480053e-13 846 \\
1.7229921775233802e-13 831 \\
2.874124176918252e-13 751 \\
4.794328083497024e-13 652 \\
7.99742125159471e-13 581 \\
1.3340502686000278e-12 433 \\
2.2253299697035906e-12 357 \\
3.712074117909949e-12 317 \\
6.1921128302120254e-12 254 \\
1.0329066738480053e-11 207 \\
1.72299217752338e-11 151 \\
2.8741241769182516e-11 113 \\
4.7943280834970106e-11 71 \\
7.997421251594699e-11 53 \\
1.334050268600028e-10 40 \\
2.225329969703591e-10 39 \\
3.7120741179099496e-10 23 \\
6.19211283021201e-10 22 \\
1.0329066738480036e-09 15 \\
1.7229921775233802e-09 6 \\
2.8741241769182518e-09 3 \\
4.794328083497011e-09 5 \\
7.997421251594698e-09 2 \\
1.3340502686000278e-08 3 \\
2.225329969703585e-08 0 \\
3.712074117909944e-08 0 \\
6.192112830212009e-08 0 \\
1.0329066738480036e-07 0 \\
1.7229921775233804e-07 0 \\
2.8741241769182515e-07 0 \\
4.794328083497011e-07 0 \\
7.997421251594698e-07 0 \\
1.3340502686000278e-06 0 \\
2.2253299697035852e-06 0 \\
3.7120741179099434e-06 0 \\
6.1921128302120095e-06 0 \\
1.0329066738480037e-05 0 \\
1.7229921775233803e-05 0 \\
2.8741241769182516e-05 0 \\
4.794328083497011e-05 0 \\
7.997421251594698e-05 0 \\
0.0001334050268600028 0 \\
0.00022253299697035849 0 \\
0.00037120741179099337 0 \\
0.0006192112830212016 0 \\
0.0010329066738480053 0 \\
0.0017229921775233801 0 \\
0.0028741241769182444 0 \\
0.004794328083497016 0 \\
0.007997421251594711 0 \\
0.013340502686000278 0 \\
0.02225329969703585 0 \\
0.037120741179099345 0 \\
0.061921128302120154 0 \\
0.10329066738480053 0 \\
0.17229921775233803 0 \\
0.28741241769182446 0 \\
0.47943280834969915 0 \\
0.7997421251594685 0 \\
1.334050268600028 0 \\
2.225329969703585 0 \\
3.7120741179099337 0 \\
6.192112830212015 0 \\
10.329066738480051 0 \\
17.2299217752338 0 \\
28.741241769182444 0 \\
47.94328083496991 0 \\
79.97421251594686 0 \\
   }; 
\addlegendentry{K1,A2,GB3}

\addplot [color=green!50!black,line width=1.5pt, mark options={solid, violet!50!magenta}, mark=*, mark repeat=11, mark phase = 9, mark size=1pt]
  table[row sep=crcr]{%
1.3340502686000278e-20 0 \\
2.225329969703585e-20 0 \\
3.7120741179099525e-20 0 \\
6.192112830212035e-20 0 \\
1.0329066738480053e-19 0 \\
1.7229921775233804e-19 0 \\
2.8741241769182593e-19 0 \\
4.794328083497031e-19 0 \\
7.997421251594712e-19 0 \\
1.334050268600028e-18 0 \\
2.225329969703585e-18 0 \\
3.7120741179099526e-18 0 \\
6.192112830212035e-18 0 \\
1.0329066738480054e-17 0 \\
1.7229921775233803e-17 0 \\
2.874124176918259e-17 0 \\
4.79432808349703e-17 1 \\
7.99742125159471e-17 0 \\
1.3340502686000278e-16 8 \\
2.225329969703591e-16 27 \\
3.7120741179099494e-16 69 \\
6.192112830212026e-16 89 \\
1.0329066738480054e-15 155 \\
1.7229921775233803e-15 183 \\
2.874124176918252e-15 226 \\
4.794328083497023e-15 280 \\
7.99742125159471e-15 277 \\
1.3340502686000279e-14 292 \\
2.225329969703585e-14 264 \\
3.7120741179099436e-14 250 \\
6.192112830212025e-14 233 \\
1.0329066738480053e-13 260 \\
1.7229921775233802e-13 255 \\
2.874124176918252e-13 259 \\
4.794328083497024e-13 247 \\
7.99742125159471e-13 285 \\
1.3340502686000278e-12 255 \\
2.2253299697035906e-12 291 \\
3.712074117909949e-12 287 \\
6.1921128302120254e-12 317 \\
1.0329066738480053e-11 316 \\
1.72299217752338e-11 357 \\
2.8741241769182516e-11 349 \\
4.7943280834970106e-11 399 \\
7.997421251594699e-11 349 \\
1.334050268600028e-10 346 \\
2.225329969703591e-10 388 \\
3.7120741179099496e-10 389 \\
6.19211283021201e-10 398 \\
1.0329066738480036e-09 366 \\
1.7229921775233802e-09 327 \\
2.8741241769182518e-09 305 \\
4.794328083497011e-09 262 \\
7.997421251594698e-09 186 \\
1.3340502686000278e-08 158 \\
2.225329969703585e-08 101 \\
3.712074117909944e-08 50 \\
6.192112830212009e-08 41 \\
1.0329066738480036e-07 30 \\
1.7229921775233804e-07 20 \\
2.8741241769182515e-07 14 \\
4.794328083497011e-07 9 \\
7.997421251594698e-07 3 \\
1.3340502686000278e-06 3 \\
2.2253299697035852e-06 2 \\
3.7120741179099434e-06 0 \\
6.1921128302120095e-06 3 \\
1.0329066738480037e-05 1 \\
1.7229921775233803e-05 0 \\
2.8741241769182516e-05 0 \\
4.794328083497011e-05 0 \\
7.997421251594698e-05 0 \\
0.0001334050268600028 0 \\
0.00022253299697035849 0 \\
0.00037120741179099337 0 \\
0.0006192112830212016 0 \\
0.0010329066738480053 0 \\
0.0017229921775233801 0 \\
0.0028741241769182444 0 \\
0.004794328083497016 0 \\
0.007997421251594711 0 \\
0.013340502686000278 1 \\
0.02225329969703585 0 \\
0.037120741179099345 1 \\
0.061921128302120154 1 \\
0.10329066738480053 1 \\
0.17229921775233803 2 \\
0.28741241769182446 2 \\
0.47943280834969915 4 \\
0.7997421251594685 2 \\
1.334050268600028 3 \\
2.225329969703585 1 \\
3.7120741179099337 0 \\
6.192112830212015 0 \\
10.329066738480051 0 \\
17.2299217752338 0 \\
28.741241769182444 0 \\
47.94328083496991 0 \\
79.97421251594686 0 \\
   }; 
\addlegendentry{K1,A1,HC}


\addplot [color=green!50!black,line width=1.5pt, mark options={solid,violet, draw=black,fill=violet}, mark=triangle*, mark repeat=11, mark phase=6, mark size=0.4pt, mark phase=3]
  table[row sep=crcr]{%
1.3340502686000278e-20 0 \\
2.225329969703585e-20 0 \\
3.7120741179099525e-20 0 \\
6.192112830212035e-20 0 \\
1.0329066738480053e-19 0 \\
1.7229921775233804e-19 0 \\
2.8741241769182593e-19 0 \\
4.794328083497031e-19 0 \\
7.997421251594712e-19 0 \\
1.334050268600028e-18 0 \\
2.225329969703585e-18 0 \\
3.7120741179099526e-18 0 \\
6.192112830212035e-18 0 \\
1.0329066738480054e-17 0 \\
1.7229921775233803e-17 0 \\
2.874124176918259e-17 0 \\
4.79432808349703e-17 2 \\
7.99742125159471e-17 7 \\
1.3340502686000278e-16 12 \\
2.225329969703591e-16 46 \\
3.7120741179099494e-16 80 \\
6.192112830212026e-16 107 \\
1.0329066738480054e-15 173 \\
1.7229921775233803e-15 233 \\
2.874124176918252e-15 266 \\
4.794328083497023e-15 231 \\
7.99742125159471e-15 249 \\
1.3340502686000279e-14 270 \\
2.225329969703585e-14 281 \\
3.7120741179099436e-14 237 \\
6.192112830212025e-14 249 \\
1.0329066738480053e-13 260 \\
1.7229921775233802e-13 256 \\
2.874124176918252e-13 266 \\
4.794328083497024e-13 245 \\
7.99742125159471e-13 267 \\
1.3340502686000278e-12 297 \\
2.2253299697035906e-12 315 \\
3.712074117909949e-12 280 \\
6.1921128302120254e-12 322 \\
1.0329066738480053e-11 317 \\
1.72299217752338e-11 317 \\
2.8741241769182516e-11 321 \\
4.7943280834970106e-11 360 \\
7.997421251594699e-11 354 \\
1.334050268600028e-10 389 \\
2.225329969703591e-10 347 \\
3.7120741179099496e-10 374 \\
6.19211283021201e-10 430 \\
1.0329066738480036e-09 402 \\
1.7229921775233802e-09 366 \\
2.8741241769182518e-09 297 \\
4.794328083497011e-09 202 \\
7.997421251594698e-09 173 \\
1.3340502686000278e-08 123 \\
2.225329969703585e-08 92 \\
3.712074117909944e-08 53 \\
6.192112830212009e-08 29 \\
1.0329066738480036e-07 25 \\
1.7229921775233804e-07 13 \\
2.8741241769182515e-07 12 \\
4.794328083497011e-07 9 \\
7.997421251594698e-07 6 \\
1.3340502686000278e-06 1 \\
2.2253299697035852e-06 3 \\
3.7120741179099434e-06 2 \\
6.1921128302120095e-06 1 \\
1.0329066738480037e-05 1 \\
1.7229921775233803e-05 0 \\
2.8741241769182516e-05 0 \\
4.794328083497011e-05 0 \\
7.997421251594698e-05 0 \\
0.0001334050268600028 0 \\
0.00022253299697035849 0 \\
0.00037120741179099337 0 \\
0.0006192112830212016 0 \\
0.0010329066738480053 1 \\
0.0017229921775233801 0 \\
0.0028741241769182444 0 \\
0.004794328083497016 0 \\
0.007997421251594711 1 \\
0.013340502686000278 0 \\
0.02225329969703585 2 \\
0.037120741179099345 1 \\
0.061921128302120154 1 \\
0.10329066738480053 4 \\
0.17229921775233803 0 \\
0.28741241769182446 6 \\
0.47943280834969915 4 \\
0.7997421251594685 6 \\
1.334050268600028 4 \\
2.225329969703585 0 \\
3.7120741179099337 0 \\
6.192112830212015 0 \\
10.329066738480051 0 \\
17.2299217752338 0 \\
28.741241769182444 0 \\
47.94328083496991 0 \\
79.97421251594686 0 \\
   }; 
\addlegendentry{K2,A2,HC}




%\legend{}

\end{axis}

==> plot/rotation_stability_3v.tex <==
\begin{axis}[%
xmode=log,
width=0.35\columnwidth,
height=0.22\columnwidth,
at={(0in,0.389in)},
scale only axis,
xmin=1e-18,
xmax=1e+2,
xlabel style={font=\color{white!15!black},yshift=0.05in},
xlabel={rotation error (rad)},
label style={font=\small},
title={Rotation stability},
ymin=0,
ymax=1000,
ymode=normal,
yminorticks=true,
axis lines = left,
axis background/.style={fill=white},
title style={font=\bfseries, yshift=0.03in},
ylabel style={yshift=-0.10in},
ylabel={Frequency},
grid=both,
legend style={at={(1.1,1.4)}, anchor=south, legend cell align=left, align=left, draw=white!15!black, font=\footnotesize,nodes={scale=1.0, transform shape}},
legend columns=4,
scaled y ticks=base 10:-3,
yticklabel style={/pgf/number format/fixed}
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\addplot [color=orange!50!black,line width=1.5pt, mark options={solid, orange}, mark options={solid, cyan}, mark=*, mark repeat=11, mark phase=3, mark size=1pt]
  table[row sep=crcr]{%
1.3340502686000278e-20 0 \\
2.225329969703585e-20 0 \\
3.7120741179099525e-20 0 \\
6.192112830212035e-20 0 \\
1.0329066738480053e-19 0 \\
1.7229921775233804e-19 0 \\
2.8741241769182593e-19 0 \\
4.794328083497031e-19 0 \\
7.997421251594712e-19 0 \\
1.334050268600028e-18 0 \\
2.225329969703585e-18 0 \\
3.7120741179099526e-18 0 \\
6.192112830212035e-18 0 \\
1.0329066738480054e-17 0 \\
1.7229921775233803e-17 0 \\
2.874124176918259e-17 0 \\
4.79432808349703e-17 1 \\
7.99742125159471e-17 2 \\
1.3340502686000278e-16 3 \\
2.225329969703591e-16 14 \\
3.7120741179099494e-16 40 \\
6.192112830212026e-16 62 \\
1.0329066738480054e-15 83 \\
1.7229921775233803e-15 123 \\
2.874124176918252e-15 150 \\
4.794328083497023e-15 188 \\
7.99742125159471e-15 173 \\
1.3340502686000279e-14 189 \\
2.225329969703585e-14 194 \\
3.7120741179099436e-14 222 \\
6.192112830212025e-14 216 \\
1.0329066738480053e-13 236 \\
1.7229921775233802e-13 223 \\
2.874124176918252e-13 240 \\
4.794328083497024e-13 240 \\
7.99742125159471e-13 227 \\
1.3340502686000278e-12 271 \\
2.2253299697035906e-12 271 \\
3.712074117909949e-12 272 \\
6.1921128302120254e-12 304 \\
1.0329066738480053e-11 316 \\
1.72299217752338e-11 325 \\
2.8741241769182516e-11 318 \\
4.7943280834970106e-11 341 \\
7.997421251594699e-11 368 \\
1.334050268600028e-10 357 \\
2.225329969703591e-10 396 \\
3.7120741179099496e-10 410 \\
6.19211283021201e-10 402 \\
1.0329066738480036e-09 464 \\
1.7229921775233802e-09 441 \\
2.8741241769182518e-09 421 \\
4.794328083497011e-09 379 \\
7.997421251594698e-09 336 \\
1.3340502686000278e-08 263 \\
2.225329969703585e-08 185 \\
3.712074117909944e-08 118 \\
6.192112830212009e-08 71 \\
1.0329066738480036e-07 41 \\
1.7229921775233804e-07 25 \\
2.8741241769182515e-07 18 \\
4.794328083497011e-07 14 \\
7.997421251594698e-07 7 \\
1.3340502686000278e-06 15 \\
2.2253299697035852e-06 5 \\
3.7120741179099434e-06 2 \\
6.1921128302120095e-06 3 \\
1.0329066738480037e-05 0 \\
1.7229921775233803e-05 0 \\
2.8741241769182516e-05 0 \\
4.794328083497011e-05 0 \\
7.997421251594698e-05 0 \\
0.0001334050268600028 0 \\
0.00022253299697035849 0 \\
0.00037120741179099337 0 \\
0.0006192112830212016 0 \\
0.0010329066738480053 0 \\
0.0017229921775233801 0 \\
0.0028741241769182444 0 \\
0.004794328083497016 0 \\
0.007997421251594711 0 \\
0.013340502686000278 1 \\
0.02225329969703585 0 \\
0.037120741179099345 0 \\
0.061921128302120154 1 \\
0.10329066738480053 2 \\
0.17229921775233803 0 \\
0.28741241769182446 0 \\
0.47943280834969915 4 \\
0.7997421251594685 0 \\
1.334050268600028 4 \\
2.225329969703585 3 \\
3.7120741179099337 0 \\
6.192112830212015 0 \\
10.329066738480051 0 \\
17.2299217752338 0 \\
28.741241769182444 0 \\
47.94328083496991 0 \\
79.97421251594686 0 \\
  };
\addlegendentry{K1,A1,HC}


\addplot [color=orange,line width=1.5pt, mark options={solid, orange}, mark options={solid, violet}, mark=*, mark repeat=11, mark phase=6, mark size=1pt]
  table[row sep=crcr]{%
1.3340502686000278e-20 0 \\
2.225329969703585e-20 0 \\
3.7120741179099525e-20 0 \\
6.192112830212035e-20 0 \\
1.0329066738480053e-19 0 \\
1.7229921775233804e-19 0 \\
2.8741241769182593e-19 0 \\
4.794328083497031e-19 0 \\
7.997421251594712e-19 0 \\
1.334050268600028e-18 0 \\
2.225329969703585e-18 0 \\
3.7120741179099526e-18 0 \\
6.192112830212035e-18 0 \\
1.0329066738480054e-17 0 \\
1.7229921775233803e-17 0 \\
2.874124176918259e-17 0 \\
4.79432808349703e-17 0 \\
7.99742125159471e-17 0 \\
1.3340502686000278e-16 0 \\
2.225329969703591e-16 0 \\
3.7120741179099494e-16 0 \\
6.192112830212026e-16 0 \\
1.0329066738480054e-15 0 \\
1.7229921775233803e-15 0 \\
2.874124176918252e-15 0 \\
4.794328083497023e-15 0 \\
7.99742125159471e-15 0 \\
1.3340502686000279e-14 0 \\
2.225329969703585e-14 0 \\
3.7120741179099436e-14 0 \\
6.192112830212025e-14 0 \\
1.0329066738480053e-13 0 \\
1.7229921775233802e-13 2 \\
2.874124176918252e-13 2 \\
4.794328083497024e-13 3 \\
7.99742125159471e-13 3 \\
1.3340502686000278e-12 8 \\
2.2253299697035906e-12 16 \\
3.712074117909949e-12 11 \\
6.1921128302120254e-12 28 \\
1.0329066738480053e-11 34 \\
1.72299217752338e-11 33 \\
2.8741241769182516e-11 44 \\
4.7943280834970106e-11 53 \\
7.997421251594699e-11 84 \\
1.334050268600028e-10 101 \\
2.225329969703591e-10 127 \\
3.7120741179099496e-10 153 \\
6.19211283021201e-10 141 \\
1.0329066738480036e-09 190 \\
1.7229921775233802e-09 214 \\
2.8741241769182518e-09 212 \\
4.794328083497011e-09 249 \\
7.997421251594698e-09 258 \\
1.3340502686000278e-08 300 \\
2.225329969703585e-08 322 \\
3.712074117909944e-08 282 \\
6.192112830212009e-08 290 \\
1.0329066738480036e-07 375 \\
1.7229921775233804e-07 349 \\
2.8741241769182515e-07 337 \\
4.794328083497011e-07 326 \\
7.997421251594698e-07 343 \\
1.3340502686000278e-06 311 \\
2.2253299697035852e-06 324 \\
3.7120741179099434e-06 327 \\
6.1921128302120095e-06 323 \\
1.0329066738480037e-05 297 \\
1.7229921775233803e-05 307 \\
2.8741241769182516e-05 276 \\
4.794328083497011e-05 286 \\
7.997421251594698e-05 249 \\
0.0001334050268600028 237 \\
0.00022253299697035849 220 \\
0.00037120741179099337 230 \\
0.0006192112830212016 202 \\
0.0010329066738480053 190 \\
0.0017229921775233801 169 \\
0.0028741241769182444 139 \\
0.004794328083497016 151 \\
0.007997421251594711 122 \\
0.013340502686000278 116 \\
0.02225329969703585 84 \\
0.037120741179099345 80 \\
0.061921128302120154 88 \\
0.10329066738480053 65 \\
0.17229921775233803 63 \\
0.28741241769182446 65 \\
0.47943280834969915 66 \\
0.7997421251594685 71 \\
1.334050268600028 39 \\
2.225329969703585 13 \\
3.7120741179099337 0 \\
6.192112830212015 0 \\
10.329066738480051 0 \\
17.2299217752338 0 \\
28.741241769182444 0 \\
47.94328083496991 0 \\
79.97421251594686 0 \\
  };
\addlegendentry{K1,A1,GB}


\addplot [color=orange!50!black,line width=1.5pt, mark options={solid, orange}, mark options={solid, cyan}, mark=triangle*, mark repeat=11, mark phase=9, mark size=1pt]
  table[row sep=crcr]{%
1.3340502686000278e-20 0 \\
2.225329969703585e-20 0 \\
3.7120741179099525e-20 0 \\
6.192112830212035e-20 0 \\
1.0329066738480053e-19 0 \\
1.7229921775233804e-19 0 \\
2.8741241769182593e-19 0 \\
4.794328083497031e-19 0 \\
7.997421251594712e-19 0 \\
1.334050268600028e-18 0 \\
2.225329969703585e-18 0 \\
3.7120741179099526e-18 0 \\
6.192112830212035e-18 0 \\
1.0329066738480054e-17 0 \\
1.7229921775233803e-17 0 \\
2.874124176918259e-17 0 \\
4.79432808349703e-17 0 \\
7.99742125159471e-17 1 \\
1.3340502686000278e-16 3 \\
2.225329969703591e-16 12 \\
3.7120741179099494e-16 36 \\
6.192112830212026e-16 53 \\
1.0329066738480054e-15 76 \\
1.7229921775233803e-15 112 \\
2.874124176918252e-15 159 \\
4.794328083497023e-15 193 \\
7.99742125159471e-15 224 \\
1.3340502686000279e-14 221 \\
2.225329969703585e-14 205 \\
3.7120741179099436e-14 222 \\
6.192112830212025e-14 213 \\
1.0329066738480053e-13 217 \\
1.7229921775233802e-13 225 \\
2.874124176918252e-13 239 \\
4.794328083497024e-13 241 \\
7.99742125159471e-13 239 \\
1.3340502686000278e-12 264 \\
2.2253299697035906e-12 250 \\
3.712074117909949e-12 303 \\
6.1921128302120254e-12 263 \\
1.0329066738480053e-11 268 \\
1.72299217752338e-11 331 \\
2.8741241769182516e-11 313 \\
4.7943280834970106e-11 371 \\
7.997421251594699e-11 364 \\
1.334050268600028e-10 413 \\
2.225329969703591e-10 391 \\
3.7120741179099496e-10 414 \\
6.19211283021201e-10 409 \\
1.0329066738480036e-09 445 \\
1.7229921775233802e-09 439 \\
2.8741241769182518e-09 403 \\
4.794328083497011e-09 334 \\
7.997421251594698e-09 321 \\
1.3340502686000278e-08 251 \\
2.225329969703585e-08 183 \\
3.712074117909944e-08 126 \\
6.192112830212009e-08 80 \\
1.0329066738480036e-07 57 \\
1.7229921775233804e-07 34 \\
2.8741241769182515e-07 26 \\
4.794328083497011e-07 18 \\
7.997421251594698e-07 5 \\
1.3340502686000278e-06 5 \\
2.2253299697035852e-06 6 \\
3.7120741179099434e-06 2 \\
6.1921128302120095e-06 4 \\
1.0329066738480037e-05 3 \\
1.7229921775233803e-05 0 \\
2.8741241769182516e-05 0 \\
4.794328083497011e-05 0 \\
7.997421251594698e-05 0 \\
0.0001334050268600028 0 \\
0.00022253299697035849 0 \\
0.00037120741179099337 0 \\
0.0006192112830212016 0 \\
0.0010329066738480053 0 \\
0.0017229921775233801 0 \\
0.0028741241769182444 0 \\
0.004794328083497016 0 \\
0.007997421251594711 0 \\
0.013340502686000278 0 \\
0.02225329969703585 0 \\
0.037120741179099345 0 \\
0.061921128302120154 0 \\
0.10329066738480053 0 \\
0.17229921775233803 0 \\
0.28741241769182446 1 \\
0.47943280834969915 0 \\
0.7997421251594685 1 \\
1.334050268600028 5 \\
2.225329969703585 6 \\
3.7120741179099337 0 \\
6.192112830212015 0 \\
10.329066738480051 0 \\
17.2299217752338 0 \\
28.741241769182444 0 \\
47.94328083496991 0 \\
79.97421251594686 0 \\
  };
\addlegendentry{K1,A2,HC}


\addplot [color=orange,line width=1.5pt, mark options={solid, orange}, mark options={solid, violet}, mark=triangle*, mark repeat=11, mark size=1pt]
  table[row sep=crcr]{%
1.3340502686000278e-20 0 \\
2.225329969703585e-20 0 \\
3.7120741179099525e-20 0 \\
6.192112830212035e-20 0 \\
1.0329066738480053e-19 0 \\
1.7229921775233804e-19 0 \\
2.8741241769182593e-19 0 \\
4.794328083497031e-19 0 \\
7.997421251594712e-19 0 \\
1.334050268600028e-18 0 \\
2.225329969703585e-18 0 \\
3.7120741179099526e-18 0 \\
6.192112830212035e-18 0 \\
1.0329066738480054e-17 0 \\
1.7229921775233803e-17 0 \\
2.874124176918259e-17 0 \\
4.79432808349703e-17 0 \\
7.99742125159471e-17 0 \\
1.3340502686000278e-16 0 \\
2.225329969703591e-16 0 \\
3.7120741179099494e-16 0 \\
6.192112830212026e-16 0 \\
1.0329066738480054e-15 0 \\
1.7229921775233803e-15 0 \\
2.874124176918252e-15 0 \\
4.794328083497023e-15 0 \\
7.99742125159471e-15 0 \\
1.3340502686000279e-14 0 \\
2.225329969703585e-14 0 \\
3.7120741179099436e-14 0 \\
6.192112830212025e-14 0 \\
1.0329066738480053e-13 0 \\
1.7229921775233802e-13 1 \\
2.874124176918252e-13 1 \\
4.794328083497024e-13 2 \\
7.99742125159471e-13 1 \\
1.3340502686000278e-12 3 \\
2.2253299697035906e-12 6 \\
3.712074117909949e-12 2 \\
6.1921128302120254e-12 8 \\
1.0329066738480053e-11 15 \\
1.72299217752338e-11 25 \\
2.8741241769182516e-11 43 \\
4.7943280834970106e-11 58 \\
7.997421251594699e-11 53 \\
1.334050268600028e-10 71 \\
2.225329969703591e-10 89 \\
3.7120741179099496e-10 130 \\
6.19211283021201e-10 136 \\
1.0329066738480036e-09 162 \\
1.7229921775233802e-09 198 \\
2.8741241769182518e-09 229 \\
4.794328083497011e-09 255 \\
7.997421251594698e-09 257 \\
1.3340502686000278e-08 287 \\
2.225329969703585e-08 309 \\
3.712074117909944e-08 321 \\
6.192112830212009e-08 298 \\
1.0329066738480036e-07 309 \\
1.7229921775233804e-07 326 \\
2.8741241769182515e-07 348 \\
4.794328083497011e-07 343 \\
7.997421251594698e-07 337 \\
1.3340502686000278e-06 363 \\
2.2253299697035852e-06 342 \\
3.7120741179099434e-06 329 \\
6.1921128302120095e-06 299 \\
1.0329066738480037e-05 304 \\
1.7229921775233803e-05 308 \\
2.8741241769182516e-05 283 \\
4.794328083497011e-05 258 \\
7.997421251594698e-05 261 \\
0.0001334050268600028 242 \\
0.00022253299697035849 224 \\
0.00037120741179099337 219 \\
0.0006192112830212016 210 \\
0.0010329066738480053 170 \\
0.0017229921775233801 176 \\
0.0028741241769182444 144 \\
0.004794328083497016 133 \\
0.007997421251594711 114 \\
0.013340502686000278 109 \\
0.02225329969703585 114 \\
0.037120741179099345 108 \\
0.061921128302120154 96 \\
0.10329066738480053 90 \\
0.17229921775233803 99 \\
0.28741241769182446 89 \\
0.47943280834969915 106 \\
0.7997421251594685 95 \\
1.334050268600028 73 \\
2.225329969703585 19 \\
3.7120741179099337 0 \\
6.192112830212015 0 \\
10.329066738480051 0 \\
17.2299217752338 0 \\
28.741241769182444 0 \\
47.94328083496991 0 \\
79.97421251594686 0 \\
  };
\addlegendentry{K1,A2,GB}




\addplot [color=orange!50!black,line width=1.5pt, mark options={solid, orange}, mark options={solid, black}, mark=*, mark repeat=11, mark size=1pt]
  table[row sep=crcr]{%
1.3340502686000278e-20 0 \\
2.225329969703585e-20 0 \\
3.7120741179099525e-20 0 \\
6.192112830212035e-20 0 \\
1.0329066738480053e-19 0 \\
1.7229921775233804e-19 0 \\
2.8741241769182593e-19 0 \\
4.794328083497031e-19 0 \\
7.997421251594712e-19 0 \\
1.334050268600028e-18 0 \\
2.225329969703585e-18 0 \\
3.7120741179099526e-18 0 \\
6.192112830212035e-18 0 \\
1.0329066738480054e-17 0 \\
1.7229921775233803e-17 0 \\
2.874124176918259e-17 0 \\
4.79432808349703e-17 0 \\
7.99742125159471e-17 3 \\
1.3340502686000278e-16 1 \\
2.225329969703591e-16 14 \\
3.7120741179099494e-16 30 \\
6.192112830212026e-16 74 \\
1.0329066738480054e-15 84 \\
1.7229921775233803e-15 122 \\
2.874124176918252e-15 163 \\
4.794328083497023e-15 212 \\
7.99742125159471e-15 218 \\
1.3340502686000279e-14 221 \\
2.225329969703585e-14 243 \\
3.7120741179099436e-14 221 \\
6.192112830212025e-14 256 \\
1.0329066738480053e-13 229 \\
1.7229921775233802e-13 246 \\
2.874124176918252e-13 212 \\
4.794328083497024e-13 303 \\
7.99742125159471e-13 252 \\
1.3340502686000278e-12 250 \\
2.2253299697035906e-12 292 \\
3.712074117909949e-12 271 \\
6.1921128302120254e-12 315 \\
1.0329066738480053e-11 270 \\
1.72299217752338e-11 320 \\
2.8741241769182516e-11 336 \\
4.7943280834970106e-11 349 \\
7.997421251594699e-11 332 \\
1.334050268600028e-10 410 \\
2.225329969703591e-10 414 \\
3.7120741179099496e-10 354 \\
6.19211283021201e-10 399 \\
1.0329066738480036e-09 437 \\
1.7229921775233802e-09 407 \\
2.8741241769182518e-09 412 \\
4.794328083497011e-09 388 \\
7.997421251594698e-09 306 \\
1.3340502686000278e-08 186 \\
2.225329969703585e-08 166 \\
3.712074117909944e-08 94 \\
6.192112830212009e-08 60 \\
1.0329066738480036e-07 48 \\
1.7229921775233804e-07 26 \\
2.8741241769182515e-07 15 \\
4.794328083497011e-07 7 \\
7.997421251594698e-07 6 \\
1.3340502686000278e-06 3 \\
2.2253299697035852e-06 6 \\
3.7120741179099434e-06 4 \\
6.1921128302120095e-06 2 \\
1.0329066738480037e-05 1 \\
1.7229921775233803e-05 0 \\
2.8741241769182516e-05 0 \\
4.794328083497011e-05 0 \\
7.997421251594698e-05 0 \\
0.0001334050268600028 0 \\
0.00022253299697035849 0 \\
0.00037120741179099337 0 \\
0.0006192112830212016 0 \\
0.0010329066738480053 0 \\
0.0017229921775233801 0 \\
0.0028741241769182444 0 \\
0.004794328083497016 0 \\
0.007997421251594711 0 \\
0.013340502686000278 0 \\
0.02225329969703585 0 \\
0.037120741179099345 0 \\
0.061921128302120154 0 \\
0.10329066738480053 2 \\
0.17229921775233803 0 \\
0.28741241769182446 1 \\
0.47943280834969915 5 \\
0.7997421251594685 1 \\
1.334050268600028 1 \\
2.225329969703585 0 \\
3.7120741179099337 0 \\
6.192112830212015 0 \\
10.329066738480051 0 \\
17.2299217752338 0 \\
28.741241769182444 0 \\
47.94328083496991 0 \\
79.97421251594686 0 \\
  };
\addlegendentry{K2,A1,HC}

\addplot [color=orange!50!black,line width=1.5pt, mark options={solid, orange}, mark options={solid, black}, mark=triangle*, mark repeat=11, mark size=1pt]
  table[row sep=crcr]{%
1.3340502686000278e-20 0 \\
2.225329969703585e-20 0 \\
3.7120741179099525e-20 0 \\
6.192112830212035e-20 0 \\
1.0329066738480053e-19 0 \\
1.7229921775233804e-19 0 \\
2.8741241769182593e-19 0 \\
4.794328083497031e-19 0 \\
7.997421251594712e-19 0 \\
1.334050268600028e-18 0 \\
2.225329969703585e-18 0 \\
3.7120741179099526e-18 0 \\
6.192112830212035e-18 0 \\
1.0329066738480054e-17 0 \\
1.7229921775233803e-17 0 \\
2.874124176918259e-17 0 \\
4.79432808349703e-17 1 \\
7.99742125159471e-17 0 \\
1.3340502686000278e-16 4 \\
2.225329969703591e-16 26 \\
3.7120741179099494e-16 41 \\
6.192112830212026e-16 88 \\
1.0329066738480054e-15 101 \\
1.7229921775233803e-15 113 \\
2.874124176918252e-15 162 \\
4.794328083497023e-15 183 \\
7.99742125159471e-15 187 \\
1.3340502686000279e-14 201 \\
2.225329969703585e-14 233 \\
3.7120741179099436e-14 252 \\
6.192112830212025e-14 210 \\
1.0329066738480053e-13 212 \\
1.7229921775233802e-13 222 \\
2.874124176918252e-13 260 \\
4.794328083497024e-13 238 \\
7.99742125159471e-13 267 \\
1.3340502686000278e-12 283 \\
2.2253299697035906e-12 264 \\
3.712074117909949e-12 232 \\
6.1921128302120254e-12 283 \\
1.0329066738480053e-11 316 \\
1.72299217752338e-11 344 \\
2.8741241769182516e-11 319 \\
4.7943280834970106e-11 354 \\
7.997421251594699e-11 390 \\
1.334050268600028e-10 406 \\
2.225329969703591e-10 392 \\
3.7120741179099496e-10 360 \\
6.19211283021201e-10 410 \\
1.0329066738480036e-09 378 \\
1.7229921775233802e-09 385 \\
2.8741241769182518e-09 371 \\
4.794328083497011e-09 375 \\
7.997421251594698e-09 296 \\
1.3340502686000278e-08 267 \\
2.225329969703585e-08 184 \\
3.712074117909944e-08 114 \\
6.192112830212009e-08 91 \\
1.0329066738480036e-07 65 \\
1.7229921775233804e-07 32 \\
2.8741241769182515e-07 29 \\
4.794328083497011e-07 22 \\
7.997421251594698e-07 13 \\
1.3340502686000278e-06 7 \\
2.2253299697035852e-06 3 \\
3.7120741179099434e-06 3 \\
6.1921128302120095e-06 4 \\
1.0329066738480037e-05 2 \\
1.7229921775233803e-05 1 \\
2.8741241769182516e-05 1 \\
4.794328083497011e-05 0 \\
7.997421251594698e-05 1 \\
0.0001334050268600028 0 \\
0.00022253299697035849 0 \\
0.00037120741179099337 0 \\
0.0006192112830212016 0 \\
0.0010329066738480053 0 \\
0.0017229921775233801 0 \\
0.0028741241769182444 0 \\
0.004794328083497016 0 \\
0.007997421251594711 0 \\
0.013340502686000278 0 \\
0.02225329969703585 0 \\
0.037120741179099345 0 \\
0.061921128302120154 1 \\
0.10329066738480053 1 \\
0.17229921775233803 0 \\
0.28741241769182446 0 \\
0.47943280834969915 0 \\
0.7997421251594685 0 \\
1.334050268600028 0 \\
2.225329969703585 0 \\
3.7120741179099337 0 \\
6.192112830212015 0 \\
10.329066738480051 0 \\
17.2299217752338 0 \\
28.741241769182444 0 \\
47.94328083496991 0 \\
79.97421251594686 0 \\
  };
\addlegendentry{K2,A2,HC}







%\legend{}

\end{axis}

==> plot/rotation_stability_4v.tex <==
\begin{axis}[%
xmode=log,
width=0.35\columnwidth,
height=0.22\columnwidth,
at={(0in,0.389in)},
scale only axis,
xmin=1e-18,
xmax=1e+2,
xlabel style={font=\color{white!15!black},yshift=0.05in},
xlabel={rotation error (rad)},
label style={font=\small},
title={Rotation stability},
ymin=0,
ymax=1000,
ymode=normal,
yminorticks=true,
axis lines = left,
axis background/.style={fill=white},
title style={font=\bfseries, yshift=0.03in},
ylabel style={yshift=-0.10in},
ylabel={Frequency},
grid=both,
legend style={at={(1.1,1.4)}, anchor=south, legend cell align=left, align=left, draw=white!15!black, font=\footnotesize,nodes={scale=1.0, transform shape}},
legend columns=4,
scaled y ticks=base 10:-3,
yticklabel style={/pgf/number format/fixed}
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\addplot [color=cyan!50!black,line width=1.5pt, mark options={solid, orange}, mark options={solid, violet!50!magenta}, mark=*, mark repeat=11, mark phase=9, mark size=1pt]
  table[row sep=crcr]{%
1.3340502686000278e-20 0 \\
2.225329969703585e-20 0 \\
3.7120741179099525e-20 0 \\
6.192112830212035e-20 0 \\
1.0329066738480053e-19 0 \\
1.7229921775233804e-19 0 \\
2.8741241769182593e-19 0 \\
4.794328083497031e-19 0 \\
7.997421251594712e-19 0 \\
1.334050268600028e-18 0 \\
2.225329969703585e-18 0 \\
3.7120741179099526e-18 0 \\
6.192112830212035e-18 0 \\
1.0329066738480054e-17 0 \\
1.7229921775233803e-17 0 \\
2.874124176918259e-17 0 \\
4.79432808349703e-17 0 \\
7.99742125159471e-17 0 \\
1.3340502686000278e-16 0 \\
2.225329969703591e-16 0 \\
3.7120741179099494e-16 1 \\
6.192112830212026e-16 0 \\
1.0329066738480054e-15 9 \\
1.7229921775233803e-15 17 \\
2.874124176918252e-15 31 \\
4.794328083497023e-15 38 \\
7.99742125159471e-15 64 \\
1.3340502686000279e-14 90 \\
2.225329969703585e-14 124 \\
3.7120741179099436e-14 176 \\
6.192112830212025e-14 219 \\
1.0329066738480053e-13 231 \\
1.7229921775233802e-13 288 \\
2.874124176918252e-13 280 \\
4.794328083497024e-13 316 \\
7.99742125159471e-13 343 \\
1.3340502686000278e-12 331 \\
2.2253299697035906e-12 334 \\
3.712074117909949e-12 369 \\
6.1921128302120254e-12 348 \\
1.0329066738480053e-11 383 \\
1.72299217752338e-11 392 \\
2.8741241769182516e-11 384 \\
4.7943280834970106e-11 371 \\
7.997421251594699e-11 340 \\
1.334050268600028e-10 428 \\
2.225329969703591e-10 381 \\
3.7120741179099496e-10 382 \\
6.19211283021201e-10 365 \\
1.0329066738480036e-09 395 \\
1.7229921775233802e-09 430 \\
2.8741241769182518e-09 415 \\
4.794328083497011e-09 395 \\
7.997421251594698e-09 372 \\
1.3340502686000278e-08 276 \\
2.225329969703585e-08 208 \\
3.712074117909944e-08 169 \\
6.192112830212009e-08 114 \\
1.0329066738480036e-07 64 \\
1.7229921775233804e-07 42 \\
2.8741241769182515e-07 28 \\
4.794328083497011e-07 15 \\
7.997421251594698e-07 6 \\
1.3340502686000278e-06 4 \\
2.2253299697035852e-06 3 \\
3.7120741179099434e-06 6 \\
6.1921128302120095e-06 0 \\
1.0329066738480037e-05 2 \\
1.7229921775233803e-05 0 \\
2.8741241769182516e-05 2 \\
4.794328083497011e-05 0 \\
7.997421251594698e-05 0 \\
0.0001334050268600028 0 \\
0.00022253299697035849 0 \\
0.00037120741179099337 0 \\
0.0006192112830212016 0 \\
0.0010329066738480053 0 \\
0.0017229921775233801 0 \\
0.0028741241769182444 0 \\
0.004794328083497016 0 \\
0.007997421251594711 0 \\
0.013340502686000278 0 \\
0.02225329969703585 0 \\
0.037120741179099345 0 \\
0.061921128302120154 0 \\
0.10329066738480053 0 \\
0.17229921775233803 2 \\
0.28741241769182446 1 \\
0.47943280834969915 3 \\
0.7997421251594685 1 \\
1.334050268600028 5 \\
2.225329969703585 3 \\
3.7120741179099337 0 \\
6.192112830212015 0 \\
10.329066738480051 0 \\
17.2299217752338 0 \\
28.741241769182444 0 \\
47.94328083496991 0 \\
79.97421251594686 0 \\
  };
\addlegendentry{K1,A1,HC}


\addplot [color=cyan,line width=1.5pt, mark options={solid, orange}, mark options={solid, violet}, mark=*, mark repeat=11, mark phase=6, mark size=1pt]
  table[row sep=crcr]{%
1.3340502686000278e-20 0 \\
2.225329969703585e-20 0 \\
3.7120741179099525e-20 0 \\
6.192112830212035e-20 0 \\
1.0329066738480053e-19 0 \\
1.7229921775233804e-19 0 \\
2.8741241769182593e-19 0 \\
4.794328083497031e-19 0 \\
7.997421251594712e-19 0 \\
1.334050268600028e-18 0 \\
2.225329969703585e-18 0 \\
3.7120741179099526e-18 0 \\
6.192112830212035e-18 0 \\
1.0329066738480054e-17 0 \\
1.7229921775233803e-17 0 \\
2.874124176918259e-17 0 \\
4.79432808349703e-17 0 \\
7.99742125159471e-17 0 \\
1.3340502686000278e-16 0 \\
2.225329969703591e-16 0 \\
3.7120741179099494e-16 0 \\
6.192112830212026e-16 0 \\
1.0329066738480054e-15 0 \\
1.7229921775233803e-15 0 \\
2.874124176918252e-15 1 \\
4.794328083497023e-15 0 \\
7.99742125159471e-15 0 \\
1.3340502686000279e-14 0 \\
2.225329969703585e-14 1 \\
3.7120741179099436e-14 2 \\
6.192112830212025e-14 7 \\
1.0329066738480053e-13 11 \\
1.7229921775233802e-13 10 \\
2.874124176918252e-13 14 \\
4.794328083497024e-13 43 \\
7.99742125159471e-13 61 \\
1.3340502686000278e-12 73 \\
2.2253299697035906e-12 88 \\
3.712074117909949e-12 111 \\
6.1921128302120254e-12 142 \\
1.0329066738480053e-11 146 \\
1.72299217752338e-11 189 \\
2.8741241769182516e-11 189 \\
4.7943280834970106e-11 226 \\
7.997421251594699e-11 223 \\
1.334050268600028e-10 228 \\
2.225329969703591e-10 264 \\
3.7120741179099496e-10 283 \\
6.19211283021201e-10 292 \\
1.0329066738480036e-09 296 \\
1.7229921775233802e-09 344 \\
2.8741241769182518e-09 301 \\
4.794328083497011e-09 316 \\
7.997421251594698e-09 356 \\
1.3340502686000278e-08 306 \\
2.225329969703585e-08 325 \\
3.712074117909944e-08 307 \\
6.192112830212009e-08 298 \\
1.0329066738480036e-07 310 \\
1.7229921775233804e-07 292 \\
2.8741241769182515e-07 273 \\
4.794328083497011e-07 254 \\
7.997421251594698e-07 263 \\
1.3340502686000278e-06 252 \\
2.2253299697035852e-06 214 \\
3.7120741179099434e-06 214 \\
6.1921128302120095e-06 222 \\
1.0329066738480037e-05 182 \\
1.7229921775233803e-05 182 \\
2.8741241769182516e-05 162 \\
4.794328083497011e-05 136 \\
7.997421251594698e-05 162 \\
0.0001334050268600028 135 \\
0.00022253299697035849 148 \\
0.00037120741179099337 126 \\
0.0006192112830212016 98 \\
0.0010329066738480053 111 \\
0.0017229921775233801 82 \\
0.0028741241769182444 72 \\
0.004794328083497016 59 \\
0.007997421251594711 59 \\
0.013340502686000278 55 \\
0.02225329969703585 65 \\
0.037120741179099345 48 \\
0.061921128302120154 62 \\
0.10329066738480053 55 \\
0.17229921775233803 69 \\
0.28741241769182446 54 \\
0.47943280834969915 60 \\
0.7997421251594685 31 \\
1.334050268600028 26 \\
2.225329969703585 13 \\
3.7120741179099337 0 \\
6.192112830212015 0 \\
10.329066738480051 0 \\
17.2299217752338 0 \\
28.741241769182444 0 \\
47.94328083496991 0 \\
79.97421251594686 0 \\
  };
\addlegendentry{K1,A1,GB}


\addplot [color=cyan!50!black,line width=1.5pt, mark options={solid, orange}, mark options={solid, violet!50!magenta}, mark=triangle*, mark repeat=11, mark phase=3, mark size=1pt]
  table[row sep=crcr]{%
1.3340502686000278e-20 0 \\
2.225329969703585e-20 0 \\
3.7120741179099525e-20 0 \\
6.192112830212035e-20 0 \\
1.0329066738480053e-19 0 \\
1.7229921775233804e-19 0 \\
2.8741241769182593e-19 0 \\
4.794328083497031e-19 0 \\
7.997421251594712e-19 0 \\
1.334050268600028e-18 0 \\
2.225329969703585e-18 0 \\
3.7120741179099526e-18 0 \\
6.192112830212035e-18 0 \\
1.0329066738480054e-17 0 \\
1.7229921775233803e-17 0 \\
2.874124176918259e-17 0 \\
4.79432808349703e-17 0 \\
7.99742125159471e-17 1 \\
1.3340502686000278e-16 3 \\
2.225329969703591e-16 5 \\
3.7120741179099494e-16 16 \\
6.192112830212026e-16 23 \\
1.0329066738480054e-15 46 \\
1.7229921775233803e-15 82 \\
2.874124176918252e-15 105 \\
4.794328083497023e-15 140 \\
7.99742125159471e-15 185 \\
1.3340502686000279e-14 227 \\
2.225329969703585e-14 259 \\
3.7120741179099436e-14 277 \\
6.192112830212025e-14 306 \\
1.0329066738480053e-13 300 \\
1.7229921775233802e-13 333 \\
2.874124176918252e-13 301 \\
4.794328083497024e-13 295 \\
7.99742125159471e-13 282 \\
1.3340502686000278e-12 283 \\
2.2253299697035906e-12 315 \\
3.712074117909949e-12 304 \\
6.1921128302120254e-12 349 \\
1.0329066738480053e-11 325 \\
1.72299217752338e-11 313 \\
2.8741241769182516e-11 335 \\
4.7943280834970106e-11 330 \\
7.997421251594699e-11 378 \\
1.334050268600028e-10 371 \\
2.225329969703591e-10 368 \\
3.7120741179099496e-10 382 \\
6.19211283021201e-10 377 \\
1.0329066738480036e-09 371 \\
1.7229921775233802e-09 336 \\
2.8741241769182518e-09 324 \\
4.794328083497011e-09 306 \\
7.997421251594698e-09 240 \\
1.3340502686000278e-08 199 \\
2.225329969703585e-08 152 \\
3.712074117909944e-08 90 \\
6.192112830212009e-08 76 \\
1.0329066738480036e-07 53 \\
1.7229921775233804e-07 47 \\
2.8741241769182515e-07 23 \\
4.794328083497011e-07 16 \\
7.997421251594698e-07 8 \\
1.3340502686000278e-06 10 \\
2.2253299697035852e-06 6 \\
3.7120741179099434e-06 2 \\
6.1921128302120095e-06 3 \\
1.0329066738480037e-05 1 \\
1.7229921775233803e-05 0 \\
2.8741241769182516e-05 0 \\
4.794328083497011e-05 0 \\
7.997421251594698e-05 0 \\
0.0001334050268600028 0 \\
0.00022253299697035849 0 \\
0.00037120741179099337 1 \\
0.0006192112830212016 0 \\
0.0010329066738480053 0 \\
0.0017229921775233801 0 \\
0.0028741241769182444 0 \\
0.004794328083497016 1 \\
0.007997421251594711 0 \\
0.013340502686000278 0 \\
0.02225329969703585 3 \\
0.037120741179099345 3 \\
0.061921128302120154 4 \\
0.10329066738480053 1 \\
0.17229921775233803 8 \\
0.28741241769182446 4 \\
0.47943280834969915 14 \\
0.7997421251594685 17 \\
1.334050268600028 27 \\
2.225329969703585 38 \\
3.7120741179099337 0 \\
6.192112830212015 0 \\
10.329066738480051 0 \\
17.2299217752338 0 \\
28.741241769182444 0 \\
47.94328083496991 0 \\
79.97421251594686 0 \\
  };
\addlegendentry{K1,A2,HC}


\addplot [color=cyan,line width=1.5pt, mark options={solid, orange}, mark options={solid, violet}, mark=triangle*, mark repeat=11, mark size=1pt]
  table[row sep=crcr]{%
1.3340502686000278e-20 0 \\
2.225329969703585e-20 0 \\
3.7120741179099525e-20 0 \\
6.192112830212035e-20 0 \\
1.0329066738480053e-19 0 \\
1.7229921775233804e-19 0 \\
2.8741241769182593e-19 0 \\
4.794328083497031e-19 0 \\
7.997421251594712e-19 0 \\
1.334050268600028e-18 0 \\
2.225329969703585e-18 0 \\
3.7120741179099526e-18 0 \\
6.192112830212035e-18 0 \\
1.0329066738480054e-17 0 \\
1.7229921775233803e-17 0 \\
2.874124176918259e-17 0 \\
4.79432808349703e-17 0 \\
7.99742125159471e-17 0 \\
1.3340502686000278e-16 0 \\
2.225329969703591e-16 0 \\
3.7120741179099494e-16 0 \\
6.192112830212026e-16 0 \\
1.0329066738480054e-15 0 \\
1.7229921775233803e-15 0 \\
2.874124176918252e-15 0 \\
4.794328083497023e-15 0 \\
7.99742125159471e-15 0 \\
1.3340502686000279e-14 0 \\
2.225329969703585e-14 3 \\
3.7120741179099436e-14 3 \\
6.192112830212025e-14 4 \\
1.0329066738480053e-13 11 \\
1.7229921775233802e-13 22 \\
2.874124176918252e-13 27 \\
4.794328083497024e-13 37 \\
7.99742125159471e-13 39 \\
1.3340502686000278e-12 41 \\
2.2253299697035906e-12 60 \\
3.712074117909949e-12 72 \\
6.1921128302120254e-12 101 \\
1.0329066738480053e-11 120 \\
1.72299217752338e-11 137 \\
2.8741241769182516e-11 148 \\
4.7943280834970106e-11 170 \\
7.997421251594699e-11 168 \\
1.334050268600028e-10 210 \\
2.225329969703591e-10 228 \\
3.7120741179099496e-10 244 \\
6.19211283021201e-10 231 \\
1.0329066738480036e-09 250 \\
1.7229921775233802e-09 264 \\
2.8741241769182518e-09 284 \\
4.794328083497011e-09 283 \\
7.997421251594698e-09 295 \\
1.3340502686000278e-08 278 \\
2.225329969703585e-08 313 \\
3.712074117909944e-08 278 \\
6.192112830212009e-08 268 \\
1.0329066738480036e-07 332 \\
1.7229921775233804e-07 260 \\
2.8741241769182515e-07 287 \\
4.794328083497011e-07 282 \\
7.997421251594698e-07 257 \\
1.3340502686000278e-06 264 \\
2.2253299697035852e-06 239 \\
3.7120741179099434e-06 231 \\
6.1921128302120095e-06 242 \\
1.0329066738480037e-05 231 \\
1.7229921775233803e-05 222 \\
2.8741241769182516e-05 201 \\
4.794328083497011e-05 206 \\
7.997421251594698e-05 228 \\
0.0001334050268600028 193 \\
0.00022253299697035849 174 \\
0.00037120741179099337 163 \\
0.0006192112830212016 157 \\
0.0010329066738480053 159 \\
0.0017229921775233801 145 \\
0.0028741241769182444 144 \\
0.004794328083497016 107 \\
0.007997421251594711 93 \\
0.013340502686000278 99 \\
0.02225329969703585 85 \\
0.037120741179099345 50 \\
0.061921128302120154 72 \\
0.10329066738480053 48 \\
0.17229921775233803 49 \\
0.28741241769182446 49 \\
0.47943280834969915 42 \\
0.7997421251594685 36 \\
1.334050268600028 23 \\
2.225329969703585 41 \\
3.7120741179099337 0 \\
6.192112830212015 0 \\
10.329066738480051 0 \\
17.2299217752338 0 \\
28.741241769182444 0 \\
47.94328083496991 0 \\
79.97421251594686 0 \\
  };
\addlegendentry{K1,A2,GB}




\addplot [color=cyan!50!black,line width=1.5pt, mark options={solid, orange}, mark options={solid, black}, mark=*, mark repeat=11, mark size=1pt]
  table[row sep=crcr]{%
1.3340502686000278e-20 0 \\
2.225329969703585e-20 0 \\
3.7120741179099525e-20 0 \\
6.192112830212035e-20 0 \\
1.0329066738480053e-19 0 \\
1.7229921775233804e-19 0 \\
2.8741241769182593e-19 0 \\
4.794328083497031e-19 0 \\
7.997421251594712e-19 0 \\
1.334050268600028e-18 0 \\
2.225329969703585e-18 0 \\
3.7120741179099526e-18 0 \\
6.192112830212035e-18 0 \\
1.0329066738480054e-17 0 \\
1.7229921775233803e-17 0 \\
2.874124176918259e-17 0 \\
4.79432808349703e-17 0 \\
7.99742125159471e-17 0 \\
1.3340502686000278e-16 0 \\
2.225329969703591e-16 2 \\
3.7120741179099494e-16 10 \\
6.192112830212026e-16 10 \\
1.0329066738480054e-15 27 \\
1.7229921775233803e-15 42 \\
2.874124176918252e-15 70 \\
4.794328083497023e-15 97 \\
7.99742125159471e-15 101 \\
1.3340502686000279e-14 137 \\
2.225329969703585e-14 160 \\
3.7120741179099436e-14 229 \\
6.192112830212025e-14 208 \\
1.0329066738480053e-13 229 \\
1.7229921775233802e-13 228 \\
2.874124176918252e-13 213 \\
4.794328083497024e-13 247 \\
7.99742125159471e-13 259 \\
1.3340502686000278e-12 261 \\
2.2253299697035906e-12 264 \\
3.712074117909949e-12 269 \\
6.1921128302120254e-12 269 \\
1.0329066738480053e-11 280 \\
1.72299217752338e-11 319 \\
2.8741241769182516e-11 343 \\
4.7943280834970106e-11 351 \\
7.997421251594699e-11 358 \\
1.334050268600028e-10 371 \\
2.225329969703591e-10 372 \\
3.7120741179099496e-10 438 \\
6.19211283021201e-10 465 \\
1.0329066738480036e-09 425 \\
1.7229921775233802e-09 446 \\
2.8741241769182518e-09 442 \\
4.794328083497011e-09 415 \\
7.997421251594698e-09 379 \\
1.3340502686000278e-08 343 \\
2.225329969703585e-08 243 \\
3.712074117909944e-08 222 \\
6.192112830212009e-08 132 \\
1.0329066738480036e-07 100 \\
1.7229921775233804e-07 63 \\
2.8741241769182515e-07 41 \\
4.794328083497011e-07 27 \\
7.997421251594698e-07 13 \\
1.3340502686000278e-06 15 \\
2.2253299697035852e-06 5 \\
3.7120741179099434e-06 2 \\
6.1921128302120095e-06 1 \\
1.0329066738480037e-05 1 \\
1.7229921775233803e-05 1 \\
2.8741241769182516e-05 1 \\
4.794328083497011e-05 0 \\
7.997421251594698e-05 0 \\
0.0001334050268600028 0 \\
0.00022253299697035849 0 \\
0.00037120741179099337 0 \\
0.0006192112830212016 0 \\
0.0010329066738480053 0 \\
0.0017229921775233801 0 \\
0.0028741241769182444 0 \\
0.004794328083497016 0 \\
0.007997421251594711 0 \\
0.013340502686000278 0 \\
0.02225329969703585 1 \\
0.037120741179099345 1 \\
0.061921128302120154 2 \\
0.10329066738480053 3 \\
0.17229921775233803 8 \\
0.28741241769182446 10 \\
0.47943280834969915 12 \\
0.7997421251594685 8 \\
1.334050268600028 8 \\
2.225329969703585 1 \\
3.7120741179099337 0 \\
6.192112830212015 0 \\
10.329066738480051 0 \\
17.2299217752338 0 \\
28.741241769182444 0 \\
47.94328083496991 0 \\
79.97421251594686 0 \\
  };
\addlegendentry{K2,A1,HC}

\addplot [color=cyan!50!black,line width=1.5pt, mark options={solid, orange}, mark options={solid, black}, mark=triangle*, mark repeat=11, mark phase=6, mark size=1pt]
  table[row sep=crcr]{%
1.3340502686000278e-20 0 \\
2.225329969703585e-20 0 \\
3.7120741179099525e-20 0 \\
6.192112830212035e-20 0 \\
1.0329066738480053e-19 0 \\
1.7229921775233804e-19 0 \\
2.8741241769182593e-19 0 \\
4.794328083497031e-19 0 \\
7.997421251594712e-19 0 \\
1.334050268600028e-18 0 \\
2.225329969703585e-18 0 \\
3.7120741179099526e-18 0 \\
6.192112830212035e-18 0 \\
1.0329066738480054e-17 0 \\
1.7229921775233803e-17 0 \\
2.874124176918259e-17 0 \\
4.79432808349703e-17 0 \\
7.99742125159471e-17 0 \\
1.3340502686000278e-16 1 \\
2.225329969703591e-16 2 \\
3.7120741179099494e-16 8 \\
6.192112830212026e-16 8 \\
1.0329066738480054e-15 10 \\
1.7229921775233803e-15 36 \\
2.874124176918252e-15 48 \\
4.794328083497023e-15 69 \\
7.99742125159471e-15 101 \\
1.3340502686000279e-14 123 \\
2.225329969703585e-14 148 \\
3.7120741179099436e-14 149 \\
6.192112830212025e-14 182 \\
1.0329066738480053e-13 215 \\
1.7229921775233802e-13 213 \\
2.874124176918252e-13 243 \\
4.794328083497024e-13 229 \\
7.99742125159471e-13 279 \\
1.3340502686000278e-12 236 \\
2.2253299697035906e-12 287 \\
3.712074117909949e-12 281 \\
6.1921128302120254e-12 303 \\
1.0329066738480053e-11 297 \\
1.72299217752338e-11 326 \\
2.8741241769182516e-11 346 \\
4.7943280834970106e-11 351 \\
7.997421251594699e-11 346 \\
1.334050268600028e-10 358 \\
2.225329969703591e-10 357 \\
3.7120741179099496e-10 424 \\
6.19211283021201e-10 420 \\
1.0329066738480036e-09 448 \\
1.7229921775233802e-09 460 \\
2.8741241769182518e-09 476 \\
4.794328083497011e-09 448 \\
7.997421251594698e-09 415 \\
1.3340502686000278e-08 317 \\
2.225329969703585e-08 302 \\
3.712074117909944e-08 214 \\
6.192112830212009e-08 146 \\
1.0329066738480036e-07 123 \\
1.7229921775233804e-07 95 \\
2.8741241769182515e-07 49 \\
4.794328083497011e-07 46 \\
7.997421251594698e-07 16 \\
1.3340502686000278e-06 13 \\
2.2253299697035852e-06 7 \\
3.7120741179099434e-06 3 \\
6.1921128302120095e-06 2 \\
1.0329066738480037e-05 1 \\
1.7229921775233803e-05 2 \\
2.8741241769182516e-05 3 \\
4.794328083497011e-05 0 \\
7.997421251594698e-05 0 \\
0.0001334050268600028 1 \\
0.00022253299697035849 0 \\
0.00037120741179099337 0 \\
0.0006192112830212016 0 \\
0.0010329066738480053 0 \\
0.0017229921775233801 0 \\
0.0028741241769182444 0 \\
0.004794328083497016 1 \\
0.007997421251594711 0 \\
0.013340502686000278 1 \\
0.02225329969703585 1 \\
0.037120741179099345 1 \\
0.061921128302120154 0 \\
0.10329066738480053 0 \\
0.17229921775233803 2 \\
0.28741241769182446 1 \\
0.47943280834969915 2 \\
0.7997421251594685 3 \\
1.334050268600028 3 \\
2.225329969703585 2 \\
3.7120741179099337 0 \\
6.192112830212015 0 \\
10.329066738480051 0 \\
17.2299217752338 0 \\
28.741241769182444 0 \\
47.94328083496991 0 \\
79.97421251594686 0 \\
  };
\addlegendentry{K2,A2,HC}

\addplot [color=cyan,line width=1.5pt, mark options={solid, orange}, mark options={solid, yellow}, mark=triangle*, mark repeat=11, mark phase=3, mark size=1pt]
  table[row sep=crcr]{%
1.3340502686000278e-20 0 \\
2.225329969703585e-20 0 \\
3.7120741179099525e-20 0 \\
6.192112830212035e-20 0 \\
1.0329066738480053e-19 0 \\
1.7229921775233804e-19 0 \\
2.8741241769182593e-19 0 \\
4.794328083497031e-19 0 \\
7.997421251594712e-19 0 \\
1.334050268600028e-18 0 \\
2.225329969703585e-18 0 \\
3.7120741179099526e-18 0 \\
6.192112830212035e-18 0 \\
1.0329066738480054e-17 0 \\
1.7229921775233803e-17 0 \\
2.874124176918259e-17 0 \\
4.79432808349703e-17 0 \\
7.99742125159471e-17 0 \\
1.3340502686000278e-16 0 \\
2.225329969703591e-16 0 \\
3.7120741179099494e-16 0 \\
6.192112830212026e-16 0 \\
1.0329066738480054e-15 0 \\
1.7229921775233803e-15 0 \\
2.874124176918252e-15 0 \\
4.794328083497023e-15 0 \\
7.99742125159471e-15 0 \\
1.3340502686000279e-14 0 \\
2.225329969703585e-14 0 \\
3.7120741179099436e-14 0 \\
6.192112830212025e-14 0 \\
1.0329066738480053e-13 0 \\
1.7229921775233802e-13 0 \\
2.874124176918252e-13 0 \\
4.794328083497024e-13 0 \\
7.99742125159471e-13 0 \\
1.3340502686000278e-12 0 \\
2.2253299697035906e-12 1 \\
3.712074117909949e-12 2 \\
6.1921128302120254e-12 1 \\
1.0329066738480053e-11 0 \\
1.72299217752338e-11 2 \\
2.8741241769182516e-11 5 \\
4.7943280834970106e-11 12 \\
7.997421251594699e-11 24 \\
1.334050268600028e-10 31 \\
2.225329969703591e-10 60 \\
3.7120741179099496e-10 71 \\
6.19211283021201e-10 123 \\
1.0329066738480036e-09 165 \\
1.7229921775233802e-09 209 \\
2.8741241769182518e-09 272 \\
4.794328083497011e-09 324 \\
7.997421251594698e-09 347 \\
1.3340502686000278e-08 445 \\
2.225329969703585e-08 492 \\
3.712074117909944e-08 482 \\
6.192112830212009e-08 546 \\
1.0329066738480036e-07 527 \\
1.7229921775233804e-07 522 \\
2.8741241769182515e-07 586 \\
4.794328083497011e-07 528 \\
7.997421251594698e-07 522 \\
1.3340502686000278e-06 465 \\
2.2253299697035852e-06 413 \\
3.7120741179099434e-06 366 \\
6.1921128302120095e-06 339 \\
1.0329066738480037e-05 291 \\
1.7229921775233803e-05 278 \\
2.8741241769182516e-05 253 \\
4.794328083497011e-05 210 \\
7.997421251594698e-05 174 \\
0.0001334050268600028 169 \\
0.00022253299697035849 116 \\
0.00037120741179099337 98 \\
0.0006192112830212016 96 \\
0.0010329066738480053 63 \\
0.0017229921775233801 60 \\
0.0028741241769182444 56 \\
0.004794328083497016 52 \\
0.007997421251594711 37 \\
0.013340502686000278 29 \\
0.02225329969703585 27 \\
0.037120741179099345 24 \\
0.061921128302120154 18 \\
0.10329066738480053 17 \\
0.17229921775233803 10 \\
0.28741241769182446 11 \\
0.47943280834969915 13 \\
0.7997421251594685 11 \\
1.334050268600028 4 \\
2.225329969703585 1 \\
3.7120741179099337 0 \\
6.192112830212015 0 \\
10.329066738480051 0 \\
17.2299217752338 0 \\
28.741241769182444 0 \\
47.94328083496991 0 \\
79.97421251594686 0 \\
  };
\addlegendentry{K2,A2,GB}


%\legend{}

\end{axis}

==> plot/translation_stability.tex <==
\begin{axis}[%
xmode=log,
width=0.35\columnwidth,
height=0.22\columnwidth,
at={(1.5in,0.389in)},
scale only axis,
xmin=1e-12,
xmax=1e+2,
xlabel style={font=\color{white!15!black},yshift=0.05in},
xlabel={translation error (rad)},
label style={font=\small},
title={Translation stability},
ymin=0,
ymax=5000,
ymode=normal,
yminorticks=true,
axis lines = left,
axis background/.style={fill=white},
title style={font=\bfseries},
title style={font=\bfseries, yshift=0.03in},
%ylabel style={yshift=-0.15in},
%ylabel={Frequency},
grid=both,
legend style={at={(1.73,1.3)}, anchor=south, legend cell align=left, align=left, draw=white!15!black, font=\normalsize,nodes={scale=1.0, transform shape}},
legend columns=6,
%yticklabel style={/pgf/number format/sci},
scaled y ticks=base 10:-3,
yticklabel style={/pgf/number format/fixed}
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addplot [color=green!50!black,line width=1.5pt, mark options={solid, violet!50!magenta}, mark=triangle*, mark repeat=11, mark phase=7, mark size=0.5pt]
  table[row sep=crcr]{%
1.334050268600027769e-20 0.000000000000000000e+00 \\
2.225329969703585113e-20 0.000000000000000000e+00 \\
3.712074117909952463e-20 0.000000000000000000e+00 \\
6.192112830212035034e-20 0.000000000000000000e+00 \\
1.032906673848005283e-19 0.000000000000000000e+00 \\
1.722992177523380382e-19 0.000000000000000000e+00 \\
2.874124176918259319e-19 0.000000000000000000e+00 \\
4.794328083497031032e-19 0.000000000000000000e+00 \\
7.997421251594711528e-19 0.000000000000000000e+00 \\
1.334050268600027926e-18 0.000000000000000000e+00 \\
2.225329969703585089e-18 0.000000000000000000e+00 \\
3.712074117909952560e-18 0.000000000000000000e+00 \\
6.192112830212034649e-18 0.000000000000000000e+00 \\
1.032906673848005355e-17 0.000000000000000000e+00 \\
1.722992177523380305e-17 0.000000000000000000e+00 \\
2.874124176918259049e-17 0.000000000000000000e+00 \\
4.794328083497030300e-17 0.000000000000000000e+00 \\
7.997421251594709602e-17 0.000000000000000000e+00 \\
1.334050268600027833e-16 0.000000000000000000e+00 \\
2.225329969703590759e-16 0.000000000000000000e+00 \\
3.712074117909949355e-16 0.000000000000000000e+00 \\
6.192112830212025928e-16 0.000000000000000000e+00 \\
1.032906673848005379e-15 0.000000000000000000e+00 \\
1.722992177523380280e-15 0.000000000000000000e+00 \\
2.874124176918252048e-15 0.000000000000000000e+00 \\
4.794328083497023053e-15 0.000000000000000000e+00 \\
7.997421251594710194e-15 0.000000000000000000e+00 \\
1.334050268600027883e-14 0.000000000000000000e+00 \\
2.225329969703585099e-14 0.000000000000000000e+00 \\
3.712074117909943596e-14 0.000000000000000000e+00 \\
6.192112830212024824e-14 0.000000000000000000e+00 \\
1.032906673848005253e-13 0.000000000000000000e+00 \\
1.722992177523380249e-13 0.000000000000000000e+00 \\
2.874124176918251795e-13 0.000000000000000000e+00 \\
4.794328083497023747e-13 0.000000000000000000e+00 \\
7.997421251594709689e-13 0.000000000000000000e+00 \\
1.334050268600027782e-12 0.000000000000000000e+00 \\
2.225329969703590564e-12 0.000000000000000000e+00 \\
3.712074117909949327e-12 0.000000000000000000e+00 \\
6.192112830212025429e-12 0.000000000000000000e+00 \\
1.032906673848005339e-11 0.000000000000000000e+00 \\
1.722992177523380047e-11 0.000000000000000000e+00 \\
2.874124176918251573e-11 0.000000000000000000e+00 \\
4.794328083497010580e-11 1.000000000000000000e+00 \\
7.997421251594699026e-11 0.000000000000000000e+00 \\
1.334050268600027960e-10 1.000000000000000000e+00 \\
2.225329969703590920e-10 1.000000000000000000e+00 \\
3.712074117909949650e-10 1.200000000000000000e+01 \\
6.192112830212009726e-10 2.300000000000000000e+01 \\
1.032906673848003633e-09 7.300000000000000000e+01 \\
1.722992177523380150e-09 2.380000000000000000e+02 \\
2.874124176918251780e-09 6.110000000000000000e+02 \\
4.794328083497010735e-09 1.834000000000000000e+03 \\
7.997421251594698199e-09 4.028000000000000000e+03 \\
1.334050268600027794e-08 3.019000000000000000e+03 \\
2.225329969703584995e-08 5.000000000000000000e+01 \\
3.712074117909943777e-08 2.200000000000000000e+01 \\
6.192112830212008568e-08 1.400000000000000000e+01 \\
1.032906673848003625e-07 9.000000000000000000e+00 \\
1.722992177523380448e-07 1.100000000000000000e+01 \\
2.874124176918251548e-07 5.000000000000000000e+00 \\
4.794328083497010669e-07 2.000000000000000000e+00 \\
7.997421251594698001e-07 2.000000000000000000e+00 \\
1.334050268600027847e-06 4.000000000000000000e+00 \\
2.225329969703585246e-06 0.000000000000000000e+00 \\
3.712074117909943380e-06 0.000000000000000000e+00 \\
6.192112830212009521e-06 0.000000000000000000e+00 \\
1.032906673848003662e-05 1.000000000000000000e+00 \\
1.722992177523380300e-05 0.000000000000000000e+00 \\
2.874124176918251570e-05 0.000000000000000000e+00 \\
4.794328083497011135e-05 0.000000000000000000e+00 \\
7.997421251594698255e-05 0.000000000000000000e+00 \\
1.334050268600027889e-04 0.000000000000000000e+00 \\
2.225329969703584857e-04 0.000000000000000000e+00 \\
3.712074117909933656e-04 0.000000000000000000e+00 \\
6.192112830212015721e-04 0.000000000000000000e+00 \\
1.032906673848005275e-03 0.000000000000000000e+00 \\
1.722992177523380124e-03 0.000000000000000000e+00 \\
2.874124176918244414e-03 0.000000000000000000e+00 \\
4.794328083497016203e-03 0.000000000000000000e+00 \\
7.997421251594711428e-03 1.000000000000000000e+00 \\
1.334050268600027803e-02 1.000000000000000000e+00 \\
2.225329969703584987e-02 0.000000000000000000e+00 \\
3.712074117909934523e-02 2.000000000000000000e+00 \\
6.192112830212015417e-02 3.000000000000000000e+00 \\
1.032906673848005275e-01 7.000000000000000000e+00 \\
1.722992177523380297e-01 5.000000000000000000e+00 \\
2.874124176918244622e-01 1.000000000000000000e+01 \\
4.794328083496991466e-01 9.000000000000000000e+00 \\
7.997421251594685199e-01 1.000000000000000000e+00 \\
1.334050268600027955e+00 0.000000000000000000e+00 \\
2.225329969703584876e+00 0.000000000000000000e+00 \\
3.712074117909933690e+00 0.000000000000000000e+00 \\
6.192112830212015417e+00 0.000000000000000000e+00 \\
1.032906673848005141e+01 0.000000000000000000e+00 \\
1.722992177523380164e+01 0.000000000000000000e+00 \\
2.874124176918244444e+01 0.000000000000000000e+00 \\
4.794328083496991155e+01 0.000000000000000000e+00 \\
7.997421251594685998e+01 0.000000000000000000e+00 \\
};
\addlegendentry{P2L1 our}

\addplot [color=green!90!black,line width=1.5pt, mark options={solid, violet}, mark=triangle*, mark repeat=9, mark phase = 5, mark size=1pt]
  table[row sep=crcr]{%
  1.3340502686000278e-20 0 \\
2.225329969703585e-20 0 \\
3.7120741179099525e-20 0 \\
6.192112830212035e-20 0 \\
1.0329066738480053e-19 0 \\
1.7229921775233804e-19 0 \\
2.8741241769182593e-19 0 \\
4.794328083497031e-19 0 \\
7.997421251594712e-19 0 \\
1.334050268600028e-18 0 \\
2.225329969703585e-18 0 \\
3.7120741179099526e-18 0 \\
6.192112830212035e-18 0 \\
1.0329066738480054e-17 0 \\
1.7229921775233803e-17 0 \\
2.874124176918259e-17 0 \\
4.79432808349703e-17 0 \\
7.99742125159471e-17 0 \\
1.3340502686000278e-16 0 \\
2.225329969703591e-16 0 \\
3.7120741179099494e-16 0 \\
6.192112830212026e-16 0 \\
1.0329066738480054e-15 0 \\
1.7229921775233803e-15 0 \\
2.874124176918252e-15 0 \\
4.794328083497023e-15 0 \\
7.99742125159471e-15 0 \\
1.3340502686000279e-14 0 \\
2.225329969703585e-14 0 \\
3.7120741179099436e-14 0 \\
6.192112830212025e-14 0 \\
1.0329066738480053e-13 0 \\
1.7229921775233802e-13 0 \\
2.874124176918252e-13 0 \\
4.794328083497024e-13 0 \\
7.99742125159471e-13 0 \\
1.3340502686000278e-12 0 \\
2.2253299697035906e-12 0 \\
3.712074117909949e-12 0 \\
6.1921128302120254e-12 0 \\
1.0329066738480053e-11 1 \\
1.72299217752338e-11 0 \\
2.8741241769182516e-11 0 \\
4.7943280834970106e-11 0 \\
7.997421251594699e-11 0 \\
1.334050268600028e-10 0 \\
2.225329969703591e-10 4 \\
3.7120741179099496e-10 12 \\
6.19211283021201e-10 24 \\
1.0329066738480036e-09 101 \\
1.7229921775233802e-09 206 \\
2.8741241769182518e-09 594 \\
4.794328083497011e-09 1685 \\
7.997421251594698e-09 3738 \\
1.3340502686000278e-08 2689 \\
2.225329969703585e-08 142 \\
3.712074117909944e-08 98 \\
6.192112830212009e-08 103 \\
1.0329066738480036e-07 89 \\
1.7229921775233804e-07 89 \\
2.8741241769182515e-07 76 \\
4.794328083497011e-07 41 \\
7.997421251594698e-07 41 \\
1.3340502686000278e-06 36 \\
2.2253299697035852e-06 47 \\
3.7120741179099434e-06 28 \\
6.1921128302120095e-06 19 \\
1.0329066738480037e-05 21 \\
1.7229921775233803e-05 11 \\
2.8741241769182516e-05 12 \\
4.794328083497011e-05 12 \\
7.997421251594698e-05 11 \\
0.0001334050268600028 11 \\
0.00022253299697035849 8 \\
0.00037120741179099337 10 \\
0.0006192112830212016 8 \\
0.0010329066738480053 5 \\
0.0017229921775233801 3 \\
0.0028741241769182444 3 \\
0.004794328083497016 2 \\
0.007997421251594711 4 \\
0.013340502686000278 1 \\
0.02225329969703585 1 \\
0.037120741179099345 1 \\
0.061921128302120154 2 \\
0.10329066738480053 2 \\
0.17229921775233803 1 \\
0.28741241769182446 5 \\
0.47943280834969915 2 \\
0.7997421251594685 1 \\
1.334050268600028 0 \\
2.225329969703585 0 \\
3.7120741179099337 0 \\
6.192112830212015 0 \\
10.329066738480051 0 \\
17.2299217752338 0 \\
28.741241769182444 0 \\
47.94328083496991 0 \\
79.97421251594686 0 \\
   }; 
\addlegendentry{m=2,n=5,K=1,A2,GB5}


\addplot [color=green!20!yellow,line width=1.5pt, mark options={solid, red}]
  table[row sep=crcr]{%
  1.3340502686000278e-20 0 \\
2.225329969703585e-20 0 \\
3.7120741179099525e-20 0 \\
6.192112830212035e-20 0 \\
1.0329066738480053e-19 0 \\
1.7229921775233804e-19 0 \\
2.8741241769182593e-19 0 \\
4.794328083497031e-19 0 \\
7.997421251594712e-19 0 \\
1.334050268600028e-18 0 \\
2.225329969703585e-18 0 \\
3.7120741179099526e-18 0 \\
6.192112830212035e-18 0 \\
1.0329066738480054e-17 0 \\
1.7229921775233803e-17 0 \\
2.874124176918259e-17 0 \\
4.79432808349703e-17 0 \\
7.99742125159471e-17 0 \\
1.3340502686000278e-16 0 \\
2.225329969703591e-16 0 \\
3.7120741179099494e-16 0 \\
6.192112830212026e-16 0 \\
1.0329066738480054e-15 0 \\
1.7229921775233803e-15 0 \\
2.874124176918252e-15 0 \\
4.794328083497023e-15 0 \\
7.99742125159471e-15 0 \\
1.3340502686000279e-14 0 \\
2.225329969703585e-14 0 \\
3.7120741179099436e-14 0 \\
6.192112830212025e-14 0 \\
1.0329066738480053e-13 0 \\
1.7229921775233802e-13 0 \\
2.874124176918252e-13 0 \\
4.794328083497024e-13 0 \\
7.99742125159471e-13 0 \\
1.3340502686000278e-12 0 \\
2.2253299697035906e-12 0 \\
3.712074117909949e-12 0 \\
6.1921128302120254e-12 0 \\
1.0329066738480053e-11 0 \\
1.72299217752338e-11 0 \\
2.8741241769182516e-11 0 \\
4.7943280834970106e-11 0 \\
7.997421251594699e-11 0 \\
1.334050268600028e-10 2 \\
2.225329969703591e-10 3 \\
3.7120741179099496e-10 10 \\
6.19211283021201e-10 31 \\
1.0329066738480036e-09 103 \\
1.7229921775233802e-09 281 \\
2.8741241769182518e-09 705 \\
4.794328083497011e-09 1838 \\
7.997421251594698e-09 4280 \\
1.3340502686000278e-08 2727 \\
2.225329969703585e-08 18 \\
3.712074117909944e-08 0 \\
6.192112830212009e-08 1 \\
1.0329066738480036e-07 1 \\
1.7229921775233804e-07 0 \\
2.8741241769182515e-07 0 \\
4.794328083497011e-07 0 \\
7.997421251594698e-07 0 \\
1.3340502686000278e-06 0 \\
2.2253299697035852e-06 0 \\
3.7120741179099434e-06 0 \\
6.1921128302120095e-06 0 \\
1.0329066738480037e-05 0 \\
1.7229921775233803e-05 0 \\
2.8741241769182516e-05 0 \\
4.794328083497011e-05 0 \\
7.997421251594698e-05 0 \\
0.0001334050268600028 0 \\
0.00022253299697035849 0 \\
0.00037120741179099337 0 \\
0.0006192112830212016 0 \\
0.0010329066738480053 0 \\
0.0017229921775233801 0 \\
0.0028741241769182444 0 \\
0.004794328083497016 0 \\
0.007997421251594711 0 \\
0.013340502686000278 0 \\
0.02225329969703585 0 \\
0.037120741179099345 0 \\
0.061921128302120154 0 \\
0.10329066738480053 0 \\
0.17229921775233803 0 \\
0.28741241769182446 0 \\
0.47943280834969915 0 \\
0.7997421251594685 0 \\
1.334050268600028 0 \\
2.225329969703585 0 \\
3.7120741179099337 0 \\
6.192112830212015 0 \\
10.329066738480051 0 \\
17.2299217752338 0 \\
28.741241769182444 0 \\
47.94328083496991 0 \\
79.97421251594686 0 \\
   }; 
\addlegendentry{m=2,n=5,K=1,A2,GB5}

\addplot [color=green!50!black,line width=1.5pt, mark options={solid, violet!50!magenta}, mark=*, mark repeat=11, mark size=1pt]
  table[row sep=crcr]{%
1.3340502686000278e-20 0 \\
2.225329969703585e-20 0 \\
3.7120741179099525e-20 0 \\
6.192112830212035e-20 0 \\
1.0329066738480053e-19 0 \\
1.7229921775233804e-19 0 \\
2.8741241769182593e-19 0 \\
4.794328083497031e-19 0 \\
7.997421251594712e-19 0 \\
1.334050268600028e-18 0 \\
2.225329969703585e-18 0 \\
3.7120741179099526e-18 0 \\
6.192112830212035e-18 0 \\
1.0329066738480054e-17 0 \\
1.7229921775233803e-17 0 \\
2.874124176918259e-17 0 \\
4.79432808349703e-17 0 \\
7.99742125159471e-17 0 \\
1.3340502686000278e-16 0 \\
2.225329969703591e-16 0 \\
3.7120741179099494e-16 0 \\
6.192112830212026e-16 0 \\
1.0329066738480054e-15 0 \\
1.7229921775233803e-15 0 \\
2.874124176918252e-15 0 \\
4.794328083497023e-15 0 \\
7.99742125159471e-15 0 \\
1.3340502686000279e-14 0 \\
2.225329969703585e-14 0 \\
3.7120741179099436e-14 0 \\
6.192112830212025e-14 0 \\
1.0329066738480053e-13 0 \\
1.7229921775233802e-13 0 \\
2.874124176918252e-13 0 \\
4.794328083497024e-13 0 \\
7.99742125159471e-13 0 \\
1.3340502686000278e-12 0 \\
2.2253299697035906e-12 0 \\
3.712074117909949e-12 0 \\
6.1921128302120254e-12 0 \\
1.0329066738480053e-11 0 \\
1.72299217752338e-11 0 \\
2.8741241769182516e-11 0 \\
4.7943280834970106e-11 0 \\
7.997421251594699e-11 0 \\
1.334050268600028e-10 1 \\
2.225329969703591e-10 3 \\
3.7120741179099496e-10 15 \\
6.19211283021201e-10 23 \\
1.0329066738480036e-09 81 \\
1.7229921775233802e-09 256 \\
2.8741241769182518e-09 642 \\
4.794328083497011e-09 1814 \\
7.997421251594698e-09 4038 \\
1.3340502686000278e-08 2947 \\
2.225329969703585e-08 67 \\
3.712074117909944e-08 38 \\
6.192112830212009e-08 20 \\
1.0329066738480036e-07 11 \\
1.7229921775233804e-07 6 \\
2.8741241769182515e-07 7 \\
4.794328083497011e-07 5 \\
7.997421251594698e-07 3 \\
1.3340502686000278e-06 0 \\
2.2253299697035852e-06 0 \\
3.7120741179099434e-06 2 \\
6.1921128302120095e-06 0 \\
1.0329066738480037e-05 1 \\
1.7229921775233803e-05 1 \\
2.8741241769182516e-05 0 \\
4.794328083497011e-05 0 \\
7.997421251594698e-05 0 \\
0.0001334050268600028 0 \\
0.00022253299697035849 0 \\
0.00037120741179099337 0 \\
0.0006192112830212016 0 \\
0.0010329066738480053 0 \\
0.0017229921775233801 0 \\
0.0028741241769182444 0 \\
0.004794328083497016 0 \\
0.007997421251594711 1 \\
0.013340502686000278 2 \\
0.02225329969703585 0 \\
0.037120741179099345 0 \\
0.061921128302120154 5 \\
0.10329066738480053 3 \\
0.17229921775233803 5 \\
0.28741241769182446 1 \\
0.47943280834969915 1 \\
0.7997421251594685 0 \\
1.334050268600028 0 \\
2.225329969703585 0 \\
3.7120741179099337 0 \\
6.192112830212015 0 \\
10.329066738480051 0 \\
17.2299217752338 0 \\
28.741241769182444 0 \\
47.94328083496991 0 \\
79.97421251594686 0 \\
   }; 
\addlegendentry{m=2,n=5,K=1,A1,HC}

\addplot [color=green!50!black,line width=1.5pt, mark options={solid,violet, draw=black,fill=violet}, mark=triangle*, mark repeat=11, mark size=0.4pt, mark phase=3]
  table[row sep=crcr]{%
1.3340502686000278e-20 0 \\
2.225329969703585e-20 0 \\
3.7120741179099525e-20 0 \\
6.192112830212035e-20 0 \\
1.0329066738480053e-19 0 \\
1.7229921775233804e-19 0 \\
2.8741241769182593e-19 0 \\
4.794328083497031e-19 0 \\
7.997421251594712e-19 0 \\
1.334050268600028e-18 0 \\
2.225329969703585e-18 0 \\
3.7120741179099526e-18 0 \\
6.192112830212035e-18 0 \\
1.0329066738480054e-17 0 \\
1.7229921775233803e-17 0 \\
2.874124176918259e-17 0 \\
4.79432808349703e-17 0 \\
7.99742125159471e-17 0 \\
1.3340502686000278e-16 0 \\
2.225329969703591e-16 0 \\
3.7120741179099494e-16 0 \\
6.192112830212026e-16 0 \\
1.0329066738480054e-15 0 \\
1.7229921775233803e-15 0 \\
2.874124176918252e-15 0 \\
4.794328083497023e-15 0 \\
7.99742125159471e-15 0 \\
1.3340502686000279e-14 0 \\
2.225329969703585e-14 0 \\
3.7120741179099436e-14 0 \\
6.192112830212025e-14 0 \\
1.0329066738480053e-13 0 \\
1.7229921775233802e-13 0 \\
2.874124176918252e-13 0 \\
4.794328083497024e-13 0 \\
7.99742125159471e-13 0 \\
1.3340502686000278e-12 0 \\
2.2253299697035906e-12 0 \\
3.712074117909949e-12 0 \\
6.1921128302120254e-12 0 \\
1.0329066738480053e-11 0 \\
1.72299217752338e-11 0 \\
2.8741241769182516e-11 0 \\
4.7943280834970106e-11 0 \\
7.997421251594699e-11 1 \\
1.334050268600028e-10 1 \\
2.225329969703591e-10 4 \\
3.7120741179099496e-10 8 \\
6.19211283021201e-10 25 \\
1.0329066738480036e-09 79 \\
1.7229921775233802e-09 228 \\
2.8741241769182518e-09 661 \\
4.794328083497011e-09 1846 \\
7.997421251594698e-09 4056 \\
1.3340502686000278e-08 2919 \\
2.225329969703585e-08 54 \\
3.712074117909944e-08 31 \\
6.192112830212009e-08 18 \\
1.0329066738480036e-07 9 \\
1.7229921775233804e-07 9 \\
2.8741241769182515e-07 11 \\
4.794328083497011e-07 1 \\
7.997421251594698e-07 3 \\
1.3340502686000278e-06 3 \\
2.2253299697035852e-06 1 \\
3.7120741179099434e-06 1 \\
6.1921128302120095e-06 0 \\
1.0329066738480037e-05 0 \\
1.7229921775233803e-05 0 \\
2.8741241769182516e-05 0 \\
4.794328083497011e-05 0 \\
7.997421251594698e-05 0 \\
0.0001334050268600028 0 \\
0.00022253299697035849 0 \\
0.00037120741179099337 0 \\
0.0006192112830212016 0 \\
0.0010329066738480053 1 \\
0.0017229921775233801 0 \\
0.0028741241769182444 0 \\
0.004794328083497016 1 \\
0.007997421251594711 0 \\
0.013340502686000278 0 \\
0.02225329969703585 2 \\
0.037120741179099345 0 \\
0.061921128302120154 7 \\
0.10329066738480053 4 \\
0.17229921775233803 11 \\
0.28741241769182446 3 \\
0.47943280834969915 1 \\
0.7997421251594685 0 \\
1.334050268600028 0 \\
2.225329969703585 0 \\
3.7120741179099337 0 \\
6.192112830212015 0 \\
10.329066738480051 0 \\
17.2299217752338 0 \\
28.741241769182444 0 \\
47.94328083496991 0 \\
79.97421251594686 0 \\
   }; 
\addlegendentry{m=2,n=5,K=2,A2,HC}

%


\legend{}

\end{axis}

==> plot/translation_stability_3v.tex <==
\begin{axis}[%
xmode=log,
width=0.35\columnwidth,
height=0.22\columnwidth,
at={(1.5in,0.389in)},
scale only axis,
xmin=1e-12,
xmax=1e+2,
xlabel style={font=\color{white!15!black},yshift=0.05in},
xlabel={translation error (rad)},
label style={font=\small},
title={Translation stability},
ymin=0,
ymax=5000,
ymode=normal,
yminorticks=true,
axis lines = left,
axis background/.style={fill=white},
title style={font=\bfseries},
title style={font=\bfseries, yshift=0.03in},
%ylabel style={yshift=-0.15in},
%ylabel={Frequency},
grid=both,
legend style={at={(1.73,1.3)}, anchor=south, legend cell align=left, align=left, draw=white!15!black, font=\normalsize,nodes={scale=1.0, transform shape}},
legend columns=6,
%yticklabel style={/pgf/number format/sci},
scaled y ticks=base 10:-3,
yticklabel style={/pgf/number format/fixed}
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\addplot [color=orange!50!black,line width=1.5pt, mark options={solid, orange}, mark options={solid, cyan}, mark=*, mark repeat=11, mark phase=3, mark size=1pt]
  table[row sep=crcr]{%
1.3340502686000278e-20 0 \\
2.225329969703585e-20 0 \\
3.7120741179099525e-20 0 \\
6.192112830212035e-20 0 \\
1.0329066738480053e-19 0 \\
1.7229921775233804e-19 0 \\
2.8741241769182593e-19 0 \\
4.794328083497031e-19 0 \\
7.997421251594712e-19 0 \\
1.334050268600028e-18 0 \\
2.225329969703585e-18 0 \\
3.7120741179099526e-18 0 \\
6.192112830212035e-18 0 \\
1.0329066738480054e-17 0 \\
1.7229921775233803e-17 0 \\
2.874124176918259e-17 0 \\
4.79432808349703e-17 0 \\
7.99742125159471e-17 0 \\
1.3340502686000278e-16 0 \\
2.225329969703591e-16 0 \\
3.7120741179099494e-16 0 \\
6.192112830212026e-16 0 \\
1.0329066738480054e-15 0 \\
1.7229921775233803e-15 0 \\
2.874124176918252e-15 0 \\
4.794328083497023e-15 0 \\
7.99742125159471e-15 0 \\
1.3340502686000279e-14 0 \\
2.225329969703585e-14 0 \\
3.7120741179099436e-14 0 \\
6.192112830212025e-14 0 \\
1.0329066738480053e-13 0 \\
1.7229921775233802e-13 0 \\
2.874124176918252e-13 0 \\
4.794328083497024e-13 0 \\
7.99742125159471e-13 0 \\
1.3340502686000278e-12 0 \\
2.2253299697035906e-12 0 \\
3.712074117909949e-12 0 \\
6.1921128302120254e-12 0 \\
1.0329066738480053e-11 0 \\
1.72299217752338e-11 0 \\
2.8741241769182516e-11 0 \\
4.7943280834970106e-11 0 \\
7.997421251594699e-11 1 \\
1.334050268600028e-10 1 \\
2.225329969703591e-10 6 \\
3.7120741179099496e-10 10 \\
6.19211283021201e-10 32 \\
1.0329066738480036e-09 80 \\
1.7229921775233802e-09 227 \\
2.8741241769182518e-09 616 \\
4.794328083497011e-09 1773 \\
7.997421251594698e-09 3973 \\
1.3340502686000278e-08 2904 \\
2.225329969703585e-08 119 \\
3.712074117909944e-08 74 \\
6.192112830212009e-08 52 \\
1.0329066738480036e-07 38 \\
1.7229921775233804e-07 25 \\
2.8741241769182515e-07 14 \\
4.794328083497011e-07 13 \\
7.997421251594698e-07 9 \\
1.3340502686000278e-06 10 \\
2.2253299697035852e-06 4 \\
3.7120741179099434e-06 3 \\
6.1921128302120095e-06 0 \\
1.0329066738480037e-05 1 \\
1.7229921775233803e-05 0 \\
2.8741241769182516e-05 0 \\
4.794328083497011e-05 0 \\
7.997421251594698e-05 0 \\
0.0001334050268600028 0 \\
0.00022253299697035849 0 \\
0.00037120741179099337 0 \\
0.0006192112830212016 0 \\
0.0010329066738480053 0 \\
0.0017229921775233801 0 \\
0.0028741241769182444 0 \\
0.004794328083497016 0 \\
0.007997421251594711 0 \\
0.013340502686000278 1 \\
0.02225329969703585 1 \\
0.037120741179099345 0 \\
0.061921128302120154 2 \\
0.10329066738480053 2 \\
0.17229921775233803 1 \\
0.28741241769182446 2 \\
0.47943280834969915 3 \\
0.7997421251594685 3 \\
1.334050268600028 0 \\
2.225329969703585 0 \\
3.7120741179099337 0 \\
6.192112830212015 0 \\
10.329066738480051 0 \\
17.2299217752338 0 \\
28.741241769182444 0 \\
47.94328083496991 0 \\
79.97421251594686 0 \\
  };
\addlegendentry{m=3,n=2,K=1+A1,HC}


\addplot [color=orange,line width=1.5pt, mark options={solid, orange}, mark options={solid, violet}, mark=*, mark repeat=11, mark phase=6, mark size=1pt]
  table[row sep=crcr]{%
1.3340502686000278e-20 0 \\
2.225329969703585e-20 0 \\
3.7120741179099525e-20 0 \\
6.192112830212035e-20 0 \\
1.0329066738480053e-19 0 \\
1.7229921775233804e-19 0 \\
2.8741241769182593e-19 0 \\
4.794328083497031e-19 0 \\
7.997421251594712e-19 0 \\
1.334050268600028e-18 0 \\
2.225329969703585e-18 0 \\
3.7120741179099526e-18 0 \\
6.192112830212035e-18 0 \\
1.0329066738480054e-17 0 \\
1.7229921775233803e-17 0 \\
2.874124176918259e-17 0 \\
4.79432808349703e-17 0 \\
7.99742125159471e-17 0 \\
1.3340502686000278e-16 0 \\
2.225329969703591e-16 0 \\
3.7120741179099494e-16 0 \\
6.192112830212026e-16 0 \\
1.0329066738480054e-15 0 \\
1.7229921775233803e-15 0 \\
2.874124176918252e-15 0 \\
4.794328083497023e-15 0 \\
7.99742125159471e-15 0 \\
1.3340502686000279e-14 0 \\
2.225329969703585e-14 0 \\
3.7120741179099436e-14 0 \\
6.192112830212025e-14 0 \\
1.0329066738480053e-13 0 \\
1.7229921775233802e-13 0 \\
2.874124176918252e-13 0 \\
4.794328083497024e-13 0 \\
7.99742125159471e-13 0 \\
1.3340502686000278e-12 0 \\
2.2253299697035906e-12 0 \\
3.712074117909949e-12 0 \\
6.1921128302120254e-12 0 \\
1.0329066738480053e-11 0 \\
1.72299217752338e-11 0 \\
2.8741241769182516e-11 0 \\
4.7943280834970106e-11 0 \\
7.997421251594699e-11 0 \\
1.334050268600028e-10 1 \\
2.225329969703591e-10 3 \\
3.7120741179099496e-10 3 \\
6.19211283021201e-10 10 \\
1.0329066738480036e-09 26 \\
1.7229921775233802e-09 66 \\
2.8741241769182518e-09 174 \\
4.794328083497011e-09 506 \\
7.997421251594698e-09 1265 \\
1.3340502686000278e-08 1034 \\
2.225329969703585e-08 359 \\
3.712074117909944e-08 361 \\
6.192112830212009e-08 345 \\
1.0329066738480036e-07 333 \\
1.7229921775233804e-07 316 \\
2.8741241769182515e-07 343 \\
4.794328083497011e-07 313 \\
7.997421251594698e-07 290 \\
1.3340502686000278e-06 293 \\
2.2253299697035852e-06 281 \\
3.7120741179099434e-06 315 \\
6.1921128302120095e-06 311 \\
1.0329066738480037e-05 299 \\
1.7229921775233803e-05 244 \\
2.8741241769182516e-05 252 \\
4.794328083497011e-05 237 \\
7.997421251594698e-05 212 \\
0.0001334050268600028 211 \\
0.00022253299697035849 201 \\
0.00037120741179099337 162 \\
0.0006192112830212016 142 \\
0.0010329066738480053 154 \\
0.0017229921775233801 141 \\
0.0028741241769182444 103 \\
0.004794328083497016 113 \\
0.007997421251594711 100 \\
0.013340502686000278 89 \\
0.02225329969703585 66 \\
0.037120741179099345 55 \\
0.061921128302120154 56 \\
0.10329066738480053 54 \\
0.17229921775233803 59 \\
0.28741241769182446 58 \\
0.47943280834969915 36 \\
0.7997421251594685 8 \\
1.334050268600028 0 \\
2.225329969703585 0 \\
3.7120741179099337 0 \\
6.192112830212015 0 \\
10.329066738480051 0 \\
17.2299217752338 0 \\
28.741241769182444 0 \\
47.94328083496991 0 \\
79.97421251594686 0 \\
  };
\addlegendentry{m=3,n=2,K=1+A1,GB}


\addplot [color=orange!50!black,line width=1.5pt, mark options={solid, orange}, mark options={solid, cyan}, mark=triangle*, mark repeat=11, mark phase=9, mark size=1pt]
  table[row sep=crcr]{%
1.3340502686000278e-20 0 \\
2.225329969703585e-20 0 \\
3.7120741179099525e-20 0 \\
6.192112830212035e-20 0 \\
1.0329066738480053e-19 0 \\
1.7229921775233804e-19 0 \\
2.8741241769182593e-19 0 \\
4.794328083497031e-19 0 \\
7.997421251594712e-19 0 \\
1.334050268600028e-18 0 \\
2.225329969703585e-18 0 \\
3.7120741179099526e-18 0 \\
6.192112830212035e-18 0 \\
1.0329066738480054e-17 0 \\
1.7229921775233803e-17 0 \\
2.874124176918259e-17 0 \\
4.79432808349703e-17 0 \\
7.99742125159471e-17 0 \\
1.3340502686000278e-16 0 \\
2.225329969703591e-16 0 \\
3.7120741179099494e-16 0 \\
6.192112830212026e-16 0 \\
1.0329066738480054e-15 0 \\
1.7229921775233803e-15 0 \\
2.874124176918252e-15 0 \\
4.794328083497023e-15 0 \\
7.99742125159471e-15 0 \\
1.3340502686000279e-14 0 \\
2.225329969703585e-14 0 \\
3.7120741179099436e-14 0 \\
6.192112830212025e-14 0 \\
1.0329066738480053e-13 0 \\
1.7229921775233802e-13 0 \\
2.874124176918252e-13 0 \\
4.794328083497024e-13 0 \\
7.99742125159471e-13 0 \\
1.3340502686000278e-12 0 \\
2.2253299697035906e-12 0 \\
3.712074117909949e-12 0 \\
6.1921128302120254e-12 0 \\
1.0329066738480053e-11 0 \\
1.72299217752338e-11 0 \\
2.8741241769182516e-11 0 \\
4.7943280834970106e-11 0 \\
7.997421251594699e-11 2 \\
1.334050268600028e-10 1 \\
2.225329969703591e-10 4 \\
3.7120741179099496e-10 7 \\
6.19211283021201e-10 39 \\
1.0329066738480036e-09 91 \\
1.7229921775233802e-09 241 \\
2.8741241769182518e-09 624 \\
4.794328083497011e-09 1787 \\
7.997421251594698e-09 3872 \\
1.3340502686000278e-08 2898 \\
2.225329969703585e-08 155 \\
3.712074117909944e-08 87 \\
6.192112830212009e-08 68 \\
1.0329066738480036e-07 38 \\
1.7229921775233804e-07 28 \\
2.8741241769182515e-07 10 \\
4.794328083497011e-07 8 \\
7.997421251594698e-07 7 \\
1.3340502686000278e-06 7 \\
2.2253299697035852e-06 6 \\
3.7120741179099434e-06 2 \\
6.1921128302120095e-06 1 \\
1.0329066738480037e-05 3 \\
1.7229921775233803e-05 1 \\
2.8741241769182516e-05 0 \\
4.794328083497011e-05 0 \\
7.997421251594698e-05 0 \\
0.0001334050268600028 0 \\
0.00022253299697035849 0 \\
0.00037120741179099337 0 \\
0.0006192112830212016 0 \\
0.0010329066738480053 0 \\
0.0017229921775233801 0 \\
0.0028741241769182444 0 \\
0.004794328083497016 0 \\
0.007997421251594711 0 \\
0.013340502686000278 0 \\
0.02225329969703585 0 \\
0.037120741179099345 0 \\
0.061921128302120154 1 \\
0.10329066738480053 0 \\
0.17229921775233803 1 \\
0.28741241769182446 2 \\
0.47943280834969915 3 \\
0.7997421251594685 6 \\
1.334050268600028 0 \\
2.225329969703585 0 \\
3.7120741179099337 0 \\
6.192112830212015 0 \\
10.329066738480051 0 \\
17.2299217752338 0 \\
28.741241769182444 0 \\
47.94328083496991 0 \\
79.97421251594686 0 \\
  };
\addlegendentry{m=3,n=2,K=1+A2,HC}


\addplot [color=orange,line width=1.5pt, mark options={solid, orange}, mark options={solid, violet}, mark=triangle*, mark repeat=11, mark size=1pt]
  table[row sep=crcr]{%
1.3340502686000278e-20 0 \\
2.225329969703585e-20 0 \\
3.7120741179099525e-20 0 \\
6.192112830212035e-20 0 \\
1.0329066738480053e-19 0 \\
1.7229921775233804e-19 0 \\
2.8741241769182593e-19 0 \\
4.794328083497031e-19 0 \\
7.997421251594712e-19 0 \\
1.334050268600028e-18 0 \\
2.225329969703585e-18 0 \\
3.7120741179099526e-18 0 \\
6.192112830212035e-18 0 \\
1.0329066738480054e-17 0 \\
1.7229921775233803e-17 0 \\
2.874124176918259e-17 0 \\
4.79432808349703e-17 0 \\
7.99742125159471e-17 0 \\
1.3340502686000278e-16 0 \\
2.225329969703591e-16 0 \\
3.7120741179099494e-16 0 \\
6.192112830212026e-16 0 \\
1.0329066738480054e-15 0 \\
1.7229921775233803e-15 0 \\
2.874124176918252e-15 0 \\
4.794328083497023e-15 0 \\
7.99742125159471e-15 0 \\
1.3340502686000279e-14 0 \\
2.225329969703585e-14 0 \\
3.7120741179099436e-14 0 \\
6.192112830212025e-14 0 \\
1.0329066738480053e-13 0 \\
1.7229921775233802e-13 0 \\
2.874124176918252e-13 0 \\
4.794328083497024e-13 0 \\
7.99742125159471e-13 0 \\
1.3340502686000278e-12 0 \\
2.2253299697035906e-12 0 \\
3.712074117909949e-12 0 \\
6.1921128302120254e-12 0 \\
1.0329066738480053e-11 0 \\
1.72299217752338e-11 0 \\
2.8741241769182516e-11 0 \\
4.7943280834970106e-11 0 \\
7.997421251594699e-11 0 \\
1.334050268600028e-10 0 \\
2.225329969703591e-10 0 \\
3.7120741179099496e-10 3 \\
6.19211283021201e-10 2 \\
1.0329066738480036e-09 23 \\
1.7229921775233802e-09 50 \\
2.8741241769182518e-09 176 \\
4.794328083497011e-09 460 \\
7.997421251594698e-09 1045 \\
1.3340502686000278e-08 934 \\
2.225329969703585e-08 316 \\
3.712074117909944e-08 334 \\
6.192112830212009e-08 354 \\
1.0329066738480036e-07 334 \\
1.7229921775233804e-07 326 \\
2.8741241769182515e-07 338 \\
4.794328083497011e-07 353 \\
7.997421251594698e-07 344 \\
1.3340502686000278e-06 345 \\
2.2253299697035852e-06 298 \\
3.7120741179099434e-06 293 \\
6.1921128302120095e-06 313 \\
1.0329066738480037e-05 274 \\
1.7229921775233803e-05 247 \\
2.8741241769182516e-05 257 \\
4.794328083497011e-05 228 \\
7.997421251594698e-05 261 \\
0.0001334050268600028 204 \\
0.00022253299697035849 201 \\
0.00037120741179099337 183 \\
0.0006192112830212016 189 \\
0.0010329066738480053 130 \\
0.0017229921775233801 132 \\
0.0028741241769182444 136 \\
0.004794328083497016 95 \\
0.007997421251594711 105 \\
0.013340502686000278 86 \\
0.02225329969703585 78 \\
0.037120741179099345 97 \\
0.061921128302120154 66 \\
0.10329066738480053 80 \\
0.17229921775233803 95 \\
0.28741241769182446 98 \\
0.47943280834969915 87 \\
0.7997421251594685 30 \\
1.334050268600028 0 \\
2.225329969703585 0 \\
3.7120741179099337 0 \\
6.192112830212015 0 \\
10.329066738480051 0 \\
17.2299217752338 0 \\
28.741241769182444 0 \\
47.94328083496991 0 \\
79.97421251594686 0 \\
  };
\addlegendentry{m=3,n=2,K=1+A2,GB}




\addplot [color=orange!50!black,line width=1.5pt, mark options={solid, orange}, mark options={solid, black}, mark=*, mark repeat=11, mark size=1pt]
  table[row sep=crcr]{%
1.3340502686000278e-20 0 \\
2.225329969703585e-20 0 \\
3.7120741179099525e-20 0 \\
6.192112830212035e-20 0 \\
1.0329066738480053e-19 0 \\
1.7229921775233804e-19 0 \\
2.8741241769182593e-19 0 \\
4.794328083497031e-19 0 \\
7.997421251594712e-19 0 \\
1.334050268600028e-18 0 \\
2.225329969703585e-18 0 \\
3.7120741179099526e-18 0 \\
6.192112830212035e-18 0 \\
1.0329066738480054e-17 0 \\
1.7229921775233803e-17 0 \\
2.874124176918259e-17 0 \\
4.79432808349703e-17 0 \\
7.99742125159471e-17 0 \\
1.3340502686000278e-16 0 \\
2.225329969703591e-16 0 \\
3.7120741179099494e-16 0 \\
6.192112830212026e-16 0 \\
1.0329066738480054e-15 0 \\
1.7229921775233803e-15 0 \\
2.874124176918252e-15 0 \\
4.794328083497023e-15 0 \\
7.99742125159471e-15 0 \\
1.3340502686000279e-14 0 \\
2.225329969703585e-14 0 \\
3.7120741179099436e-14 0 \\
6.192112830212025e-14 0 \\
1.0329066738480053e-13 0 \\
1.7229921775233802e-13 0 \\
2.874124176918252e-13 0 \\
4.794328083497024e-13 0 \\
7.99742125159471e-13 0 \\
1.3340502686000278e-12 0 \\
2.2253299697035906e-12 0 \\
3.712074117909949e-12 0 \\
6.1921128302120254e-12 0 \\
1.0329066738480053e-11 0 \\
1.72299217752338e-11 0 \\
2.8741241769182516e-11 0 \\
4.7943280834970106e-11 0 \\
7.997421251594699e-11 0 \\
1.334050268600028e-10 2 \\
2.225329969703591e-10 5 \\
3.7120741179099496e-10 15 \\
6.19211283021201e-10 29 \\
1.0329066738480036e-09 80 \\
1.7229921775233802e-09 209 \\
2.8741241769182518e-09 632 \\
4.794328083497011e-09 1724 \\
7.997421251594698e-09 4030 \\
1.3340502686000278e-08 2903 \\
2.225329969703585e-08 138 \\
3.712074117909944e-08 73 \\
6.192112830212009e-08 59 \\
1.0329066738480036e-07 33 \\
1.7229921775233804e-07 23 \\
2.8741241769182515e-07 7 \\
4.794328083497011e-07 6 \\
7.997421251594698e-07 6 \\
1.3340502686000278e-06 7 \\
2.2253299697035852e-06 5 \\
3.7120741179099434e-06 2 \\
6.1921128302120095e-06 0 \\
1.0329066738480037e-05 1 \\
1.7229921775233803e-05 0 \\
2.8741241769182516e-05 0 \\
4.794328083497011e-05 0 \\
7.997421251594698e-05 0 \\
0.0001334050268600028 1 \\
0.00022253299697035849 0 \\
0.00037120741179099337 0 \\
0.0006192112830212016 0 \\
0.0010329066738480053 0 \\
0.0017229921775233801 0 \\
0.0028741241769182444 0 \\
0.004794328083497016 0 \\
0.007997421251594711 0 \\
0.013340502686000278 0 \\
0.02225329969703585 0 \\
0.037120741179099345 0 \\
0.061921128302120154 3 \\
0.10329066738480053 3 \\
0.17229921775233803 1 \\
0.28741241769182446 2 \\
0.47943280834969915 1 \\
0.7997421251594685 0 \\
1.334050268600028 0 \\
2.225329969703585 0 \\
3.7120741179099337 0 \\
6.192112830212015 0 \\
10.329066738480051 0 \\
17.2299217752338 0 \\
28.741241769182444 0 \\
47.94328083496991 0 \\
79.97421251594686 0 \\
  };
\addlegendentry{m=3,n=2,K=2+A1,HC}

\addplot [color=orange!50!black,line width=1.5pt, mark options={solid, orange}, mark options={solid, black}, mark=triangle*, mark repeat=11, mark size=1pt]
  table[row sep=crcr]{%
1.3340502686000278e-20 0 \\
2.225329969703585e-20 0 \\
3.7120741179099525e-20 0 \\
6.192112830212035e-20 0 \\
1.0329066738480053e-19 0 \\
1.7229921775233804e-19 0 \\
2.8741241769182593e-19 0 \\
4.794328083497031e-19 0 \\
7.997421251594712e-19 0 \\
1.334050268600028e-18 0 \\
2.225329969703585e-18 0 \\
3.7120741179099526e-18 0 \\
6.192112830212035e-18 0 \\
1.0329066738480054e-17 0 \\
1.7229921775233803e-17 0 \\
2.874124176918259e-17 0 \\
4.79432808349703e-17 0 \\
7.99742125159471e-17 0 \\
1.3340502686000278e-16 0 \\
2.225329969703591e-16 0 \\
3.7120741179099494e-16 0 \\
6.192112830212026e-16 0 \\
1.0329066738480054e-15 0 \\
1.7229921775233803e-15 0 \\
2.874124176918252e-15 0 \\
4.794328083497023e-15 0 \\
7.99742125159471e-15 0 \\
1.3340502686000279e-14 0 \\
2.225329969703585e-14 0 \\
3.7120741179099436e-14 0 \\
6.192112830212025e-14 0 \\
1.0329066738480053e-13 0 \\
1.7229921775233802e-13 0 \\
2.874124176918252e-13 0 \\
4.794328083497024e-13 0 \\
7.99742125159471e-13 0 \\
1.3340502686000278e-12 0 \\
2.2253299697035906e-12 0 \\
3.712074117909949e-12 0 \\
6.1921128302120254e-12 0 \\
1.0329066738480053e-11 0 \\
1.72299217752338e-11 0 \\
2.8741241769182516e-11 1 \\
4.7943280834970106e-11 0 \\
7.997421251594699e-11 1 \\
1.334050268600028e-10 4 \\
2.225329969703591e-10 7 \\
3.7120741179099496e-10 16 \\
6.19211283021201e-10 28 \\
1.0329066738480036e-09 71 \\
1.7229921775233802e-09 242 \\
2.8741241769182518e-09 646 \\
4.794328083497011e-09 1721 \\
7.997421251594698e-09 3866 \\
1.3340502686000278e-08 2961 \\
2.225329969703585e-08 150 \\
3.712074117909944e-08 90 \\
6.192112830212009e-08 48 \\
1.0329066738480036e-07 49 \\
1.7229921775233804e-07 28 \\
2.8741241769182515e-07 25 \\
4.794328083497011e-07 18 \\
7.997421251594698e-07 10 \\
1.3340502686000278e-06 5 \\
2.2253299697035852e-06 3 \\
3.7120741179099434e-06 1 \\
6.1921128302120095e-06 3 \\
1.0329066738480037e-05 2 \\
1.7229921775233803e-05 2 \\
2.8741241769182516e-05 0 \\
4.794328083497011e-05 0 \\
7.997421251594698e-05 0 \\
0.0001334050268600028 0 \\
0.00022253299697035849 0 \\
0.00037120741179099337 0 \\
0.0006192112830212016 0 \\
0.0010329066738480053 0 \\
0.0017229921775233801 0 \\
0.0028741241769182444 0 \\
0.004794328083497016 0 \\
0.007997421251594711 0 \\
0.013340502686000278 0 \\
0.02225329969703585 1 \\
0.037120741179099345 1 \\
0.061921128302120154 0 \\
0.10329066738480053 0 \\
0.17229921775233803 0 \\
0.28741241769182446 0 \\
0.47943280834969915 0 \\
0.7997421251594685 0 \\
1.334050268600028 0 \\
2.225329969703585 0 \\
3.7120741179099337 0 \\
6.192112830212015 0 \\
10.329066738480051 0 \\
17.2299217752338 0 \\
28.741241769182444 0 \\
47.94328083496991 0 \\
79.97421251594686 0 \\
  };
\addlegendentry{m=3,n=2,K=2+A2,GB}






\legend{}

\end{axis}

==> plot/translation_stability_4v.tex <==
\begin{axis}[%
xmode=log,
width=0.35\columnwidth,
height=0.22\columnwidth,
at={(1.5in,0.389in)},
scale only axis,
xmin=1e-12,
xmax=1e+2,
xlabel style={font=\color{white!15!black},yshift=0.05in},
xlabel={translation error (rad)},
label style={font=\small},
title={Translation stability},
ymin=0,
ymax=5000,
ymode=normal,
yminorticks=true,
axis lines = left,
axis background/.style={fill=white},
title style={font=\bfseries},
title style={font=\bfseries, yshift=0.03in},
%ylabel style={yshift=-0.15in},
%ylabel={Frequency},
grid=both,
legend style={at={(1.73,1.3)}, anchor=south, legend cell align=left, align=left, draw=white!15!black, font=\normalsize,nodes={scale=1.0, transform shape}},
legend columns=6,
%yticklabel style={/pgf/number format/sci},
scaled y ticks=base 10:-3,
yticklabel style={/pgf/number format/fixed}
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\addplot [color=cyan!50!black,line width=1.5pt, mark options={solid, red}, mark options={solid, violet!50!magenta}, mark=*, mark repeat=11, mark phase=3, mark size=1pt]
  table[row sep=crcr]{%
1.3340502686000278e-20 0 \\
2.225329969703585e-20 0 \\
3.7120741179099525e-20 0 \\
6.192112830212035e-20 0 \\
1.0329066738480053e-19 0 \\
1.7229921775233804e-19 0 \\
2.8741241769182593e-19 0 \\
4.794328083497031e-19 0 \\
7.997421251594712e-19 0 \\
1.334050268600028e-18 0 \\
2.225329969703585e-18 0 \\
3.7120741179099526e-18 0 \\
6.192112830212035e-18 0 \\
1.0329066738480054e-17 0 \\
1.7229921775233803e-17 0 \\
2.874124176918259e-17 0 \\
4.79432808349703e-17 0 \\
7.99742125159471e-17 0 \\
1.3340502686000278e-16 0 \\
2.225329969703591e-16 0 \\
3.7120741179099494e-16 0 \\
6.192112830212026e-16 0 \\
1.0329066738480054e-15 0 \\
1.7229921775233803e-15 0 \\
2.874124176918252e-15 0 \\
4.794328083497023e-15 0 \\
7.99742125159471e-15 0 \\
1.3340502686000279e-14 0 \\
2.225329969703585e-14 0 \\
3.7120741179099436e-14 0 \\
6.192112830212025e-14 0 \\
1.0329066738480053e-13 0 \\
1.7229921775233802e-13 0 \\
2.874124176918252e-13 0 \\
4.794328083497024e-13 0 \\
7.99742125159471e-13 0 \\
1.3340502686000278e-12 0 \\
2.2253299697035906e-12 0 \\
3.712074117909949e-12 0 \\
6.1921128302120254e-12 0 \\
1.0329066738480053e-11 0 \\
1.72299217752338e-11 0 \\
2.8741241769182516e-11 0 \\
4.7943280834970106e-11 0 \\
7.997421251594699e-11 0 \\
1.334050268600028e-10 0 \\
2.225329969703591e-10 4 \\
3.7120741179099496e-10 10 \\
6.19211283021201e-10 26 \\
1.0329066738480036e-09 84 \\
1.7229921775233802e-09 237 \\
2.8741241769182518e-09 638 \\
4.794328083497011e-09 1754 \\
7.997421251594698e-09 3952 \\
1.3340502686000278e-08 2936 \\
2.225329969703585e-08 119 \\
3.712074117909944e-08 91 \\
6.192112830212009e-08 51 \\
1.0329066738480036e-07 31 \\
1.7229921775233804e-07 14 \\
2.8741241769182515e-07 8 \\
4.794328083497011e-07 13 \\
7.997421251594698e-07 3 \\
1.3340502686000278e-06 3 \\
2.2253299697035852e-06 2 \\
3.7120741179099434e-06 1 \\
6.1921128302120095e-06 1 \\
1.0329066738480037e-05 1 \\
1.7229921775233803e-05 1 \\
2.8741241769182516e-05 1 \\
4.794328083497011e-05 0 \\
7.997421251594698e-05 0 \\
0.0001334050268600028 0 \\
0.00022253299697035849 0 \\
0.00037120741179099337 0 \\
0.0006192112830212016 0 \\
0.0010329066738480053 0 \\
0.0017229921775233801 0 \\
0.0028741241769182444 0 \\
0.004794328083497016 0 \\
0.007997421251594711 0 \\
0.013340502686000278 0 \\
0.02225329969703585 0 \\
0.037120741179099345 1 \\
0.061921128302120154 2 \\
0.10329066738480053 1 \\
0.17229921775233803 2 \\
0.28741241769182446 3 \\
0.47943280834969915 3 \\
0.7997421251594685 3 \\
1.334050268600028 0 \\
2.225329969703585 0 \\
3.7120741179099337 0 \\
6.192112830212015 0 \\
10.329066738480051 0 \\
17.2299217752338 0 \\
28.741241769182444 0 \\
47.94328083496991 0 \\
79.97421251594686 0 \\
  };
\addlegendentry{m=4,n=1,K=1+A1,HC}


\addplot [color=cyan,line width=1.5pt, mark options={solid, red}, mark options={solid, violet}, mark=*, mark repeat=11, mark phase=6, mark size=1pt]
  table[row sep=crcr]{%
1.3340502686000278e-20 0 \\
2.225329969703585e-20 0 \\
3.7120741179099525e-20 0 \\
6.192112830212035e-20 0 \\
1.0329066738480053e-19 0 \\
1.7229921775233804e-19 0 \\
2.8741241769182593e-19 0 \\
4.794328083497031e-19 0 \\
7.997421251594712e-19 0 \\
1.334050268600028e-18 0 \\
2.225329969703585e-18 0 \\
3.7120741179099526e-18 0 \\
6.192112830212035e-18 0 \\
1.0329066738480054e-17 0 \\
1.7229921775233803e-17 0 \\
2.874124176918259e-17 0 \\
4.79432808349703e-17 0 \\
7.99742125159471e-17 0 \\
1.3340502686000278e-16 0 \\
2.225329969703591e-16 0 \\
3.7120741179099494e-16 0 \\
6.192112830212026e-16 0 \\
1.0329066738480054e-15 0 \\
1.7229921775233803e-15 0 \\
2.874124176918252e-15 0 \\
4.794328083497023e-15 0 \\
7.99742125159471e-15 0 \\
1.3340502686000279e-14 0 \\
2.225329969703585e-14 0 \\
3.7120741179099436e-14 0 \\
6.192112830212025e-14 0 \\
1.0329066738480053e-13 0 \\
1.7229921775233802e-13 0 \\
2.874124176918252e-13 0 \\
4.794328083497024e-13 0 \\
7.99742125159471e-13 0 \\
1.3340502686000278e-12 0 \\
2.2253299697035906e-12 0 \\
3.712074117909949e-12 0 \\
6.1921128302120254e-12 0 \\
1.0329066738480053e-11 0 \\
1.72299217752338e-11 0 \\
2.8741241769182516e-11 0 \\
4.7943280834970106e-11 1 \\
7.997421251594699e-11 0 \\
1.334050268600028e-10 0 \\
2.225329969703591e-10 0 \\
3.7120741179099496e-10 4 \\
6.19211283021201e-10 18 \\
1.0329066738480036e-09 39 \\
1.7229921775233802e-09 106 \\
2.8741241769182518e-09 347 \\
4.794328083497011e-09 834 \\
7.997421251594698e-09 1900 \\
1.3340502686000278e-08 1548 \\
2.225329969703585e-08 315 \\
3.712074117909944e-08 328 \\
6.192112830212009e-08 275 \\
1.0329066738480036e-07 316 \\
1.7229921775233804e-07 278 \\
2.8741241769182515e-07 273 \\
4.794328083497011e-07 247 \\
7.997421251594698e-07 236 \\
1.3340502686000278e-06 230 \\
2.2253299697035852e-06 209 \\
3.7120741179099434e-06 217 \\
6.1921128302120095e-06 186 \\
1.0329066738480037e-05 172 \\
1.7229921775233803e-05 167 \\
2.8741241769182516e-05 139 \\
4.794328083497011e-05 159 \\
7.997421251594698e-05 149 \\
0.0001334050268600028 135 \\
0.00022253299697035849 119 \\
0.00037120741179099337 115 \\
0.0006192112830212016 85 \\
0.0010329066738480053 83 \\
0.0017229921775233801 93 \\
0.0028741241769182444 65 \\
0.004794328083497016 71 \\
0.007997421251594711 59 \\
0.013340502686000278 47 \\
0.02225329969703585 57 \\
0.037120741179099345 65 \\
0.061921128302120154 69 \\
0.10329066738480053 62 \\
0.17229921775233803 66 \\
0.28741241769182446 55 \\
0.47943280834969915 54 \\
0.7997421251594685 6 \\
1.334050268600028 0 \\
2.225329969703585 0 \\
3.7120741179099337 0 \\
6.192112830212015 0 \\
10.329066738480051 0 \\
17.2299217752338 0 \\
28.741241769182444 0 \\
47.94328083496991 0 \\
79.97421251594686 0 \\
  };
\addlegendentry{m=4,n=1,K=1+A1,GB}


\addplot [color=cyan!50!black,line width=1.5pt, mark options={solid, red}, mark options={solid, violet!50!magenta}, mark=triangle*, mark repeat=11, mark phase=9, mark size=1pt]
  table[row sep=crcr]{%
1.3340502686000278e-20 0 \\
2.225329969703585e-20 0 \\
3.7120741179099525e-20 0 \\
6.192112830212035e-20 0 \\
1.0329066738480053e-19 0 \\
1.7229921775233804e-19 0 \\
2.8741241769182593e-19 0 \\
4.794328083497031e-19 0 \\
7.997421251594712e-19 0 \\
1.334050268600028e-18 0 \\
2.225329969703585e-18 0 \\
3.7120741179099526e-18 0 \\
6.192112830212035e-18 0 \\
1.0329066738480054e-17 0 \\
1.7229921775233803e-17 0 \\
2.874124176918259e-17 0 \\
4.79432808349703e-17 0 \\
7.99742125159471e-17 0 \\
1.3340502686000278e-16 0 \\
2.225329969703591e-16 0 \\
3.7120741179099494e-16 0 \\
6.192112830212026e-16 0 \\
1.0329066738480054e-15 0 \\
1.7229921775233803e-15 0 \\
2.874124176918252e-15 0 \\
4.794328083497023e-15 0 \\
7.99742125159471e-15 0 \\
1.3340502686000279e-14 0 \\
2.225329969703585e-14 0 \\
3.7120741179099436e-14 0 \\
6.192112830212025e-14 0 \\
1.0329066738480053e-13 0 \\
1.7229921775233802e-13 0 \\
2.874124176918252e-13 0 \\
4.794328083497024e-13 0 \\
7.99742125159471e-13 0 \\
1.3340502686000278e-12 0 \\
2.2253299697035906e-12 0 \\
3.712074117909949e-12 0 \\
6.1921128302120254e-12 0 \\
1.0329066738480053e-11 0 \\
1.72299217752338e-11 0 \\
2.8741241769182516e-11 0 \\
4.7943280834970106e-11 0 \\
7.997421251594699e-11 1 \\
1.334050268600028e-10 0 \\
2.225329969703591e-10 2 \\
3.7120741179099496e-10 12 \\
6.19211283021201e-10 24 \\
1.0329066738480036e-09 84 \\
1.7229921775233802e-09 209 \\
2.8741241769182518e-09 590 \\
4.794328083497011e-09 1709 \\
7.997421251594698e-09 4042 \\
1.3340502686000278e-08 2863 \\
2.225329969703585e-08 115 \\
3.712074117909944e-08 68 \\
6.192112830212009e-08 50 \\
1.0329066738480036e-07 48 \\
1.7229921775233804e-07 18 \\
2.8741241769182515e-07 15 \\
4.794328083497011e-07 12 \\
7.997421251594698e-07 6 \\
1.3340502686000278e-06 5 \\
2.2253299697035852e-06 3 \\
3.7120741179099434e-06 1 \\
6.1921128302120095e-06 1 \\
1.0329066738480037e-05 0 \\
1.7229921775233803e-05 1 \\
2.8741241769182516e-05 0 \\
4.794328083497011e-05 0 \\
7.997421251594698e-05 0 \\
0.0001334050268600028 0 \\
0.00022253299697035849 1 \\
0.00037120741179099337 0 \\
0.0006192112830212016 0 \\
0.0010329066738480053 0 \\
0.0017229921775233801 0 \\
0.0028741241769182444 0 \\
0.004794328083497016 2 \\
0.007997421251594711 0 \\
0.013340502686000278 1 \\
0.02225329969703585 3 \\
0.037120741179099345 2 \\
0.061921128302120154 5 \\
0.10329066738480053 6 \\
0.17229921775233803 11 \\
0.28741241769182446 15 \\
0.47943280834969915 18 \\
0.7997421251594685 57 \\
1.334050268600028 0 \\
2.225329969703585 0 \\
3.7120741179099337 0 \\
6.192112830212015 0 \\
10.329066738480051 0 \\
17.2299217752338 0 \\
28.741241769182444 0 \\
47.94328083496991 0 \\
79.97421251594686 0 \\
  };
\addlegendentry{m=4,n=1,K=1+A2,HC}


\addplot [color=cyan,line width=1.5pt, mark options={solid, red}, mark options={solid, violet}, mark=triangle*, mark repeat=11, mark size=1pt]
  table[row sep=crcr]{%
1.3340502686000278e-20 0 \\
2.225329969703585e-20 0 \\
3.7120741179099525e-20 0 \\
6.192112830212035e-20 0 \\
1.0329066738480053e-19 0 \\
1.7229921775233804e-19 0 \\
2.8741241769182593e-19 0 \\
4.794328083497031e-19 0 \\
7.997421251594712e-19 0 \\
1.334050268600028e-18 0 \\
2.225329969703585e-18 0 \\
3.7120741179099526e-18 0 \\
6.192112830212035e-18 0 \\
1.0329066738480054e-17 0 \\
1.7229921775233803e-17 0 \\
2.874124176918259e-17 0 \\
4.79432808349703e-17 0 \\
7.99742125159471e-17 0 \\
1.3340502686000278e-16 0 \\
2.225329969703591e-16 0 \\
3.7120741179099494e-16 0 \\
6.192112830212026e-16 0 \\
1.0329066738480054e-15 0 \\
1.7229921775233803e-15 0 \\
2.874124176918252e-15 0 \\
4.794328083497023e-15 0 \\
7.99742125159471e-15 0 \\
1.3340502686000279e-14 0 \\
2.225329969703585e-14 0 \\
3.7120741179099436e-14 0 \\
6.192112830212025e-14 0 \\
1.0329066738480053e-13 0 \\
1.7229921775233802e-13 0 \\
2.874124176918252e-13 0 \\
4.794328083497024e-13 0 \\
7.99742125159471e-13 0 \\
1.3340502686000278e-12 0 \\
2.2253299697035906e-12 0 \\
3.712074117909949e-12 0 \\
6.1921128302120254e-12 0 \\
1.0329066738480053e-11 0 \\
1.72299217752338e-11 0 \\
2.8741241769182516e-11 0 \\
4.7943280834970106e-11 0 \\
7.997421251594699e-11 0 \\
1.334050268600028e-10 1 \\
2.225329969703591e-10 3 \\
3.7120741179099496e-10 4 \\
6.19211283021201e-10 8 \\
1.0329066738480036e-09 40 \\
1.7229921775233802e-09 112 \\
2.8741241769182518e-09 269 \\
4.794328083497011e-09 733 \\
7.997421251594698e-09 1628 \\
1.3340502686000278e-08 1351 \\
2.225329969703585e-08 362 \\
3.712074117909944e-08 302 \\
6.192112830212009e-08 283 \\
1.0329066738480036e-07 295 \\
1.7229921775233804e-07 296 \\
2.8741241769182515e-07 307 \\
4.794328083497011e-07 312 \\
7.997421251594698e-07 252 \\
1.3340502686000278e-06 246 \\
2.2253299697035852e-06 237 \\
3.7120741179099434e-06 271 \\
6.1921128302120095e-06 243 \\
1.0329066738480037e-05 217 \\
1.7229921775233803e-05 223 \\
2.8741241769182516e-05 214 \\
4.794328083497011e-05 222 \\
7.997421251594698e-05 200 \\
0.0001334050268600028 205 \\
0.00022253299697035849 164 \\
0.00037120741179099337 149 \\
0.0006192112830212016 147 \\
0.0010329066738480053 128 \\
0.0017229921775233801 101 \\
0.0028741241769182444 97 \\
0.004794328083497016 73 \\
0.007997421251594711 46 \\
0.013340502686000278 62 \\
0.02225329969703585 41 \\
0.037120741179099345 36 \\
0.061921128302120154 35 \\
0.10329066738480053 25 \\
0.17229921775233803 12 \\
0.28741241769182446 20 \\
0.47943280834969915 12 \\
0.7997421251594685 16 \\
1.334050268600028 0 \\
2.225329969703585 0 \\
3.7120741179099337 0 \\
6.192112830212015 0 \\
10.329066738480051 0 \\
17.2299217752338 0 \\
28.741241769182444 0 \\
47.94328083496991 0 \\
79.97421251594686 0 \\
  };
\addlegendentry{m=4,n=1,K=1+A2,GB}




\addplot [color=cyan!50!black,line width=1.5pt, mark options={solid, red}, mark options={solid, black}, mark=*, mark repeat=11, mark phase = 3, mark size=1pt]
  table[row sep=crcr]{%
1.3340502686000278e-20 0 \\
2.225329969703585e-20 0 \\
3.7120741179099525e-20 0 \\
6.192112830212035e-20 0 \\
1.0329066738480053e-19 0 \\
1.7229921775233804e-19 0 \\
2.8741241769182593e-19 0 \\
4.794328083497031e-19 0 \\
7.997421251594712e-19 0 \\
1.334050268600028e-18 0 \\
2.225329969703585e-18 0 \\
3.7120741179099526e-18 0 \\
6.192112830212035e-18 0 \\
1.0329066738480054e-17 0 \\
1.7229921775233803e-17 0 \\
2.874124176918259e-17 0 \\
4.79432808349703e-17 0 \\
7.99742125159471e-17 0 \\
1.3340502686000278e-16 0 \\
2.225329969703591e-16 0 \\
3.7120741179099494e-16 0 \\
6.192112830212026e-16 0 \\
1.0329066738480054e-15 0 \\
1.7229921775233803e-15 0 \\
2.874124176918252e-15 0 \\
4.794328083497023e-15 0 \\
7.99742125159471e-15 0 \\
1.3340502686000279e-14 0 \\
2.225329969703585e-14 0 \\
3.7120741179099436e-14 0 \\
6.192112830212025e-14 0 \\
1.0329066738480053e-13 0 \\
1.7229921775233802e-13 0 \\
2.874124176918252e-13 0 \\
4.794328083497024e-13 0 \\
7.99742125159471e-13 0 \\
1.3340502686000278e-12 0 \\
2.2253299697035906e-12 0 \\
3.712074117909949e-12 0 \\
6.1921128302120254e-12 0 \\
1.0329066738480053e-11 0 \\
1.72299217752338e-11 0 \\
2.8741241769182516e-11 0 \\
4.7943280834970106e-11 0 \\
7.997421251594699e-11 0 \\
1.334050268600028e-10 1 \\
2.225329969703591e-10 3 \\
3.7120741179099496e-10 7 \\
6.19211283021201e-10 29 \\
1.0329066738480036e-09 73 \\
1.7229921775233802e-09 235 \\
2.8741241769182518e-09 629 \\
4.794328083497011e-09 1680 \\
7.997421251594698e-09 3825 \\
1.3340502686000278e-08 2874 \\
2.225329969703585e-08 208 \\
3.712074117909944e-08 116 \\
6.192112830212009e-08 112 \\
1.0329066738480036e-07 51 \\
1.7229921775233804e-07 40 \\
2.8741241769182515e-07 24 \\
4.794328083497011e-07 19 \\
7.997421251594698e-07 7 \\
1.3340502686000278e-06 5 \\
2.2253299697035852e-06 4 \\
3.7120741179099434e-06 0 \\
6.1921128302120095e-06 1 \\
1.0329066738480037e-05 1 \\
1.7229921775233803e-05 1 \\
2.8741241769182516e-05 0 \\
4.794328083497011e-05 0 \\
7.997421251594698e-05 1 \\
0.0001334050268600028 0 \\
0.00022253299697035849 0 \\
0.00037120741179099337 0 \\
0.0006192112830212016 0 \\
0.0010329066738480053 0 \\
0.0017229921775233801 0 \\
0.0028741241769182444 0 \\
0.004794328083497016 0 \\
0.007997421251594711 0 \\
0.013340502686000278 0 \\
0.02225329969703585 5 \\
0.037120741179099345 1 \\
0.061921128302120154 2 \\
0.10329066738480053 8 \\
0.17229921775233803 12 \\
0.28741241769182446 12 \\
0.47943280834969915 8 \\
0.7997421251594685 6 \\
1.334050268600028 0 \\
2.225329969703585 0 \\
3.7120741179099337 0 \\
6.192112830212015 0 \\
10.329066738480051 0 \\
17.2299217752338 0 \\
28.741241769182444 0 \\
47.94328083496991 0 \\
79.97421251594686 0 \\
  };
\addlegendentry{m=4,n=1,K=2+A1,HC}

\addplot [color=cyan!50!black,line width=1.5pt, mark options={solid, red}, mark options={solid, black}, mark=triangle*, mark repeat=11, mark phase = 6, mark size=1pt]
  table[row sep=crcr]{%
1.3340502686000278e-20 0 \\
2.225329969703585e-20 0 \\
3.7120741179099525e-20 0 \\
6.192112830212035e-20 0 \\
1.0329066738480053e-19 0 \\
1.7229921775233804e-19 0 \\
2.8741241769182593e-19 0 \\
4.794328083497031e-19 0 \\
7.997421251594712e-19 0 \\
1.334050268600028e-18 0 \\
2.225329969703585e-18 0 \\
3.7120741179099526e-18 0 \\
6.192112830212035e-18 0 \\
1.0329066738480054e-17 0 \\
1.7229921775233803e-17 0 \\
2.874124176918259e-17 0 \\
4.79432808349703e-17 0 \\
7.99742125159471e-17 0 \\
1.3340502686000278e-16 0 \\
2.225329969703591e-16 0 \\
3.7120741179099494e-16 0 \\
6.192112830212026e-16 0 \\
1.0329066738480054e-15 0 \\
1.7229921775233803e-15 0 \\
2.874124176918252e-15 0 \\
4.794328083497023e-15 0 \\
7.99742125159471e-15 0 \\
1.3340502686000279e-14 0 \\
2.225329969703585e-14 0 \\
3.7120741179099436e-14 0 \\
6.192112830212025e-14 0 \\
1.0329066738480053e-13 0 \\
1.7229921775233802e-13 0 \\
2.874124176918252e-13 0 \\
4.794328083497024e-13 0 \\
7.99742125159471e-13 0 \\
1.3340502686000278e-12 0 \\
2.2253299697035906e-12 0 \\
3.712074117909949e-12 0 \\
6.1921128302120254e-12 0 \\
1.0329066738480053e-11 0 \\
1.72299217752338e-11 0 \\
2.8741241769182516e-11 0 \\
4.7943280834970106e-11 0 \\
7.997421251594699e-11 0 \\
1.334050268600028e-10 1 \\
2.225329969703591e-10 2 \\
3.7120741179099496e-10 6 \\
6.19211283021201e-10 38 \\
1.0329066738480036e-09 90 \\
1.7229921775233802e-09 226 \\
2.8741241769182518e-09 595 \\
4.794328083497011e-09 1712 \\
7.997421251594698e-09 3819 \\
1.3340502686000278e-08 2821 \\
2.225329969703585e-08 217 \\
3.712074117909944e-08 138 \\
6.192112830212009e-08 98 \\
1.0329066738480036e-07 85 \\
1.7229921775233804e-07 52 \\
2.8741241769182515e-07 32 \\
4.794328083497011e-07 18 \\
7.997421251594698e-07 11 \\
1.3340502686000278e-06 10 \\
2.2253299697035852e-06 3 \\
3.7120741179099434e-06 4 \\
6.1921128302120095e-06 1 \\
1.0329066738480037e-05 1 \\
1.7229921775233803e-05 2 \\
2.8741241769182516e-05 1 \\
4.794328083497011e-05 0 \\
7.997421251594698e-05 0 \\
0.0001334050268600028 0 \\
0.00022253299697035849 0 \\
0.00037120741179099337 0 \\
0.0006192112830212016 0 \\
0.0010329066738480053 0 \\
0.0017229921775233801 0 \\
0.0028741241769182444 1 \\
0.004794328083497016 0 \\
0.007997421251594711 0 \\
0.013340502686000278 3 \\
0.02225329969703585 0 \\
0.037120741179099345 2 \\
0.061921128302120154 3 \\
0.10329066738480053 2 \\
0.17229921775233803 1 \\
0.28741241769182446 3 \\
0.47943280834969915 1 \\
0.7997421251594685 1 \\
1.334050268600028 0 \\
2.225329969703585 0 \\
3.7120741179099337 0 \\
6.192112830212015 0 \\
10.329066738480051 0 \\
17.2299217752338 0 \\
28.741241769182444 0 \\
47.94328083496991 0 \\
79.97421251594686 0 \\
  };
\addlegendentry{m=4,n=1,K=2+A2,HC}

\addplot [color=cyan,line width=1.5pt, mark options={solid, red}, mark options={solid, yellow}, mark=triangle*, mark repeat=11, mark size=1pt]
  table[row sep=crcr]{%
1.3340502686000278e-20 0 \\
2.225329969703585e-20 0 \\
3.7120741179099525e-20 0 \\
6.192112830212035e-20 0 \\
1.0329066738480053e-19 0 \\
1.7229921775233804e-19 0 \\
2.8741241769182593e-19 0 \\
4.794328083497031e-19 0 \\
7.997421251594712e-19 0 \\
1.334050268600028e-18 0 \\
2.225329969703585e-18 0 \\
3.7120741179099526e-18 0 \\
6.192112830212035e-18 0 \\
1.0329066738480054e-17 0 \\
1.7229921775233803e-17 0 \\
2.874124176918259e-17 0 \\
4.79432808349703e-17 0 \\
7.99742125159471e-17 0 \\
1.3340502686000278e-16 0 \\
2.225329969703591e-16 0 \\
3.7120741179099494e-16 0 \\
6.192112830212026e-16 0 \\
1.0329066738480054e-15 0 \\
1.7229921775233803e-15 0 \\
2.874124176918252e-15 0 \\
4.794328083497023e-15 0 \\
7.99742125159471e-15 0 \\
1.3340502686000279e-14 0 \\
2.225329969703585e-14 0 \\
3.7120741179099436e-14 0 \\
6.192112830212025e-14 0 \\
1.0329066738480053e-13 0 \\
1.7229921775233802e-13 0 \\
2.874124176918252e-13 0 \\
4.794328083497024e-13 0 \\
7.99742125159471e-13 0 \\
1.3340502686000278e-12 0 \\
2.2253299697035906e-12 0 \\
3.712074117909949e-12 0 \\
6.1921128302120254e-12 0 \\
1.0329066738480053e-11 0 \\
1.72299217752338e-11 0 \\
2.8741241769182516e-11 0 \\
4.7943280834970106e-11 0 \\
7.997421251594699e-11 1 \\
1.334050268600028e-10 2 \\
2.225329969703591e-10 2 \\
3.7120741179099496e-10 2 \\
6.19211283021201e-10 10 \\
1.0329066738480036e-09 25 \\
1.7229921775233802e-09 69 \\
2.8741241769182518e-09 212 \\
4.794328083497011e-09 505 \\
7.997421251594698e-09 1220 \\
1.3340502686000278e-08 1192 \\
2.225329969703585e-08 572 \\
3.712074117909944e-08 542 \\
6.192112830212009e-08 542 \\
1.0329066738480036e-07 527 \\
1.7229921775233804e-07 543 \\
2.8741241769182515e-07 473 \\
4.794328083497011e-07 461 \\
7.997421251594698e-07 419 \\
1.3340502686000278e-06 408 \\
2.2253299697035852e-06 308 \\
3.7120741179099434e-06 337 \\
6.1921128302120095e-06 290 \\
1.0329066738480037e-05 220 \\
1.7229921775233803e-05 214 \\
2.8741241769182516e-05 184 \\
4.794328083497011e-05 137 \\
7.997421251594698e-05 94 \\
0.0001334050268600028 95 \\
0.00022253299697035849 72 \\
0.00037120741179099337 66 \\
0.0006192112830212016 47 \\
0.0010329066738480053 46 \\
0.0017229921775233801 31 \\
0.0028741241769182444 25 \\
0.004794328083497016 27 \\
0.007997421251594711 17 \\
0.013340502686000278 10 \\
0.02225329969703585 11 \\
0.037120741179099345 8 \\
0.061921128302120154 11 \\
0.10329066738480053 4 \\
0.17229921775233803 9 \\
0.28741241769182446 6 \\
0.47943280834969915 2 \\
0.7997421251594685 2 \\
1.334050268600028 0 \\
2.225329969703585 0 \\
3.7120741179099337 0 \\
6.192112830212015 0 \\
10.329066738480051 0 \\
17.2299217752338 0 \\
28.741241769182444 0 \\
47.94328083496991 0 \\
79.97421251594686 0 \\
  };
\addlegendentry{m=4,n=1,K=2+A2,GB}


\legend{}

\end{axis}
